Meaningfulness and Genericity in a Subsuming Framework

This paper studies the notion of meaningfulness for a unifying framework called dBang-calculus, which subsumes both call-by-name (dCbN) and call-by-value (dCbV). We first characterize meaningfulness in dBang by means of typability and inhabitation in an associated non-idempotent intersection type system previously proposed in the literature. We validate the proposed notion of meaningfulness by showing two properties (1) consistency of the theory $\mathcal{H}$ equating meaningless terms and (2) genericity, stating that meaningless subterms have no bearing on the significance of meaningful terms. The theory $\mathcal{H}$ is also shown to have a unique consistent and maximal extension. Last but not least, we show that the notions of meaningfulness and genericity in the literature for dCbN and dCbV are subsumed by the respectively ones proposed here for the dBang-calculus.

==> 2_Proofs/Bang_Full_dB_U_d__and_s__strongly_commute.tex <==
\begin{proof}
  Let $t, u_1, u_2 \in \bangSetTerms$ such that $t
\bangArr_{S_\indexOmega}<R> u_1$ and $t \bangArr_{S_\indexOmega}<s!>
u_2$ for some $\rel \in \{\bangSymbBeta, \bangSymbBang\}$. Let us show
that there exists $s \in \bangSetTerms$ such that $u_1
\bangArr_{S_\indexOmega}<s!> s$ and $u_2 \bangArr*_{S_\indexOmega}<R>
s$.

By induction on $t$:
\begin{itemize}
\item[\bltI] $t = x$: Impossible since it contradicts the hypothesis
    $t \bangArr_{S_\indexOmega}<s!> u_2$.

\item[\bltI] $t = \abs{x}{t'}$: Since by hypothesis $t
    \bangArr_{S_\indexOmega}<R> u_1$ and $t
    \bangArr_{S_\indexOmega}<s!> u_2$, then necessarily $u_1 =
    \abs{x}{u'_1}$ and $u_2 = \abs{x}{u'_2}$ for some $u'_1, u'_2 \in
    \bangSetTerms$ such that $t' \bangArr_{S_\indexOmega}<R> u'_1$ and
    $t' \bangArr_{S_\indexOmega}<s!> u'_2$. By \ih on $t'$, there
    exists $s' \in \bangSetTerms$ such that $u'_1
    \bangArr_{S_\indexOmega}<s!> s'$ and $u'_2
    \bangArr*_{S_\indexOmega}<R> s'$. We set $s := \abs{x}{s'}$ since
    by contextual closure $u_1 = \abs{x}{u'_1}
    \bangArr_{S_\indexOmega}<s!> \abs{x}{s'} = s'$ and $u_2 =
    \abs{x}{u'_2} \bangArr*_{S_\indexOmega}<R> \abs{x}{s'} = s'$.
    Graphically,
    \begin{equation*}
        \begin{array}{lll}
            \abs{x}{t'}                         &\bangArr_{S_\indexOmega}<R>    &  \abs{x}{u'_1}
        \\[0.2cm]
           \;\;\bangDownArr_{S_\indexOmega}<s!> &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
        \\[0.2cm]
           \abs{x}{u'_2}                        &\bangArr*_{S_\indexOmega}<R>   & \abs{x}{s'}
       \end{array}
    \end{equation*}
\item[\bltI] $t = \app{t_1}{t_2}$: We distinguish two cases:
    \begin{itemize}
    \item[\bltII] $t$ is the $\bangSymbBeta$-redex reduced in the step
        $t \bangArr_{S_\indexOmega}<R> u_1$: Then $t_1 =
        \bangLCtxt<\abs{x}{t'_1}>$ and $u_1 =
        \bangLCtxt<t'_1\esub{x}{t_2}>$. By hypothesis
        $\app{\bangLCtxt<\abs{x}{t'_1}>}{t_2}
        \bangArr_{S_\indexOmega}<s!> u_2$ so that four different cases
        can be distinguished:
        \begin{itemize}
        \item[\bltIII] $u_2 = \app{\bangLCtxt<\abs{x}{u'_1}>}{t_2}$
            for some $u'_1 \in \bangSetTerms$ such that $t'_1
            \bangArr_{S_\indexOmega}<s!> u'_1$: We set $s :=
            \bangLCtxt<u'_1\esub{x}{t_2}>$ which concludes this case
            since by contextual closure $u_1 =
            \bangLCtxt<t'_1\esub{x}{t_2}> \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt<u'_1\esub{x}{t_2}> = s$ and $u_2 =
            \app{\bangLCtxt<\abs{x}{u'_1}>}{t_2}
            \bangArr_{S_\indexOmega}<dB> \bangLCtxt<u'_1\esub{x}{t_2}>
            = s$. Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{\bangLCtxt<\abs{x}{t'_1}>}{t_2}        &\bangArr_{S_\indexOmega}<dB>   &\bangLCtxt<t'_1\esub{x}{t_2}>
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>        &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \app{\bangLCtxt<\abs{x}{u'_1}>}{t_2}        &\bangArr_{S_\indexOmega}<dB>   &\bangLCtxt<u'_1\esub{x}{t_2}>
                \end{array}
            \end{equation*}

        \item[\bltIII] $u_2 = \app{\bangLCtxt<\abs{x}{t'_1}>}{u'_2}$
            for some $u'_2 \in \bangSetTerms$ such that $t_2
            \bangArr_{S_\indexOmega}<s!> u'_2$: We set $s :=
            \bangLCtxt<t'_1\esub{x}{u'_2}>$ which concludes this case
            since by contextual closure $u_1 =
            \bangLCtxt<t'_1\esub{x}{t_2}> \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt<t'_1\esub{x}{u'_2}> = s$ and $u_2 =
            \app{\bangLCtxt<\abs{x}{t'_1}>}{u'_2}
            \bangArr_{S_\indexOmega}<dB>
            \bangLCtxt<t'_1\esub{x}{u'_2}> = s$. Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{\bangLCtxt<\abs{x}{t'_1}>}{t_2}        &\bangArr_{S_\indexOmega}<dB>   &  \bangLCtxt<t'_1\esub{x}{t_2}>
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>        &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                        \app{\bangLCtxt<\abs{x}{t'_1}>}{u'_2}   &\bangArr_{S_\indexOmega}<dB>  & \bangLCtxt<t'_1\esub{x}{u'_2}>
                \end{array}
            \end{equation*}

        \item[\bltIII] $u_2 = \app{\bangLCtxt'<\abs{x}{t'_1}>}{t_2}$
            for some context $\bangLCtxt'$ such that $\bangLCtxt
            \bangArr_{S_\indexOmega}<s!> \bangLCtxt'$: We set $s :=
            \bangLCtxt'<t'_1\esub{x}{t_2}>$ which concludes this case
            since by
            \Cref{lem:Bang_Full_dB_d!_Context_Reduction_Lifted_to_Terms},
            $u_1 = \bangLCtxt<t'_1\esub{x}{t_2}>
            \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt'<t'_1\esub{x}{t_2}> = s$ and $u_2 =
            \app{\bangLCtxt'<\abs{x}{t'_1}>}{t_2}
            \bangArr_{S_\indexOmega}<dB>
            \bangLCtxt'<t'_1\esub{x}{t_2}> = s$. Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{\bangLCtxt<\abs{x}{t'_1}>}{t_2}    &\bangArr_{S_\indexOmega}<dB>   &  \bangLCtxt<t'_1\esub{x}{t_2}>
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \app{\bangLCtxt'<\abs{x}{t'_1}>}{t_2}   &\bangArr_{S_\indexOmega}<dB>   & \bangLCtxt'<t'_1\esub{x}{t_2}>
                \end{array}
            \end{equation*}

        \item[\bltIII] $\bangLCtxt =
            \bangLCtxt_1<\bangLCtxt_3\esub{y}{\bangLCtxt_2<\oc
            t''_1>}>$, $u_2 =
            \app{\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{y}{t''_1}\bangCtxtPlug{\abs{x}{t'_1\isub{y}{t''_1}}}>>}{t_2}$
            for some contexts $\bangLCtxt_1, \bangLCtxt_2,
            \bangLCtxt_3$ and some term $t''_1 \in \bangSetTerms$: We
            set $s :=
            \bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{y}{t''_1}\bangCtxtPlug{t'_1\isub{y}{t''_1}\esub{x}{t_2}}>>$
            which concludes this case since by $\alpha$-conversion $y
            \notin \freeVar{t_2}$ thus $t_2\isub{x}{t''_1} = t_2$ and
            therefore: Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{\bangLCtxt_1<\bangLCtxt_3<\abs{x}{t'_1}>\esub{y}{\bangLCtxt_2<\oc t''_1>}>}{t_2}                           &\bangArr_{S_\indexOmega}<dB>   &\bangLCtxt_1<\bangLCtxt_3<t'_1\esub{x}{t_2}>\esub{y}{\bangLCtxt_2<\oc t''_1>}>
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>                                                                            &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \app{\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{y}{t''_1}\bangCtxtPlug{\abs{x}{t'_1\isub{y}{t''_1}}}>>}{t_2}   &\bangArr*_{S_\indexOmega}<dB>  &\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{y}{t''_1}\bangCtxtPlug{t'_1\isub{y}{t''_1}\esub{x}{t_2}}>>
                \end{array}
            \end{equation*}
        \end{itemize}

    \item[\bltII] Otherwise:  By hypothesis $t
        \bangArr_{S_\indexOmega}<R> u_1$ and $t
        \bangArr_{S_\indexOmega}<s!> u_2$, and four cases can thus be
        distinguished:
        \begin{itemize}
        \item[\bltIII] $u_1 = \app{u'_1}{t_2}$ and $u_2 =
            \app{u'_2}{t_2}$ with $t_1 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_1 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: By \ih on $t_1$, there
            exists $s' \in \bangSetTerms$ such that $u'_1
            \bangArr_{S_\indexOmega}<s!> s'$ and $u'_2
            \bangArr*_{S_\indexOmega}<R> s'$. We set $s :=
            \app{s'}{t_2}$ since by contextual closure $u_1 =
            \app{u'_1}{t_2} \bangArr_{S_\indexOmega}<s!> \app{s'}{t_2}
            = s'$ and $u_2 = \app{u'_2}{t_2}
            \bangArr*_{S_\indexOmega}<R> \app{s'}{t_2} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{t_1}{t_2}                          &\bangArr_{S_\indexOmega}<R>    &\app{u'_1}{t_2}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \app{u'_2}{t_2}                         &\bangArr*_{S_\indexOmega}<R>   &\app{s'}{t_2}
                \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = \app{u'_1}{t_2}$ and $u_2 =
            \app{t_1}{u'_2}$ with $t_1 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_2 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: We set $s' :=
            \app{u'_1}{u'_2}$ since by contextual closure $u_1 =
            \app{u'_1}{t_2} \bangArr_{S_\indexOmega}<s!>
            \app{u'_1}{u'_2} = s'$ and $u_2 = \app{t_1}{u'_2}
            \bangArr_{S_\indexOmega}<R> \app{u'_1}{u'_2} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{t_1}{t_2}                          &\bangArr_{S_\indexOmega}<R>    &\app{u'_1}{t_2}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \app{t_1}{u'_2}                         &\bangArr_{S_\indexOmega}<R>    &\app{u'_1}{u'_2}
                \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = \app{t_1}{u'_1}$ and $u_2 =
            \app{u'_2}{t_2}$ with $t_2 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_1 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: We set $s' :=
            \app{u'_2}{u'_1}$ since by contextual closure $u_1 =
            \app{t_1}{u'_1} \bangArr_{S_\indexOmega}<s!>
            \app{u'_2}{u'_1} = s'$ and $u_2 = \app{u'_2}{t_2}
            \bangArr_{S_\indexOmega}<R> \app{u'_2}{u'_1} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{t_1}{t_2}                          &\bangArr_{S_\indexOmega}<R>    &  \app{t_1}{u'_1}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                     \app{u'_2}{t_2}                        &\bangArr_{S_\indexOmega}<R>    &\app{u'_2}{u'_1}   
                 \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = \app{t_1}{u'_1}$ and $u_2 =
            \app{t_1}{u'_2}$ with $t_2 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_2 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: By \ih on $t_2$, there
            exists $s' \in \bangSetTerms$ such that $u'_1
            \bangArr_{S_\indexOmega}<s!> s'$ and $u'_2
            \bangArr*_{S_\indexOmega}<R> s'$. We set $s :=
            \app{t_1}{s'}$ since by contextual closure $u_1 =
            \app{t_1}{u'_1} \bangArr_{S_\indexOmega}<s!> \app{t_1}{s'}
            = s'$ and $u_2 = \app{t_1}{u'_2}
            \bangArr*_{S_\indexOmega}<R> \app{t_1}{s'} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \app{t_1}{t_2}                              &\bangArr_{S_\indexOmega}<R>    &  \app{t_1}{u'_1}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>   &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \app{t_1}{u'_2}                                   &\bangArr*_{S_\indexOmega}<R>  & \app{t_1}{s'} 
                 \end{array}
            \end{equation*}

        \end{itemize}
    \end{itemize}

\item[\bltI] $t = t_1\esub{x}{t_2}$: We distinguish two cases:
    \begin{itemize}
    \item[\bltII] $t$ is the $\bangSymbSubs$-redex reduced in the step
        $t \bangArr_{S_\indexOmega}<s!> u_2$: Then $t_2 =
        \bangLCtxt<\oc t'_2>$ and $u_2 =
        \bangLCtxt<t_1\isub{x}{t'_2}>$ for some context $\bangLCtxt$
        and some term $t'_2 \in \bangSetTerms$. Since
        $t_1\esub{x}{\bangLCtxt<\oc t'_2>} \bangArr_{S_\indexOmega}<R>
        u_1$ then three cases can be distinguished:
        \begin{itemize}
        \item[\bltIII] $t_1 \bangArr_{S_\indexOmega}<R> t'_1$ and $u_1
            = t'_1\esub{x}{t_2}$ for some term $t'_1 \in
            \bangSetTerms$: We set $s :=
            \bangLCtxt<t'_1\isub{x}{t'_2}>$ which concludes this case
            since by induction on $t_1$, one has that
            $t_1\isub{x}{t'_2} \bangArr_{S_\indexOmega}<R>
            t'_1\isub{x}{t'_2}$ thus by contextual closure $u_1 =
            t'_1\esub{x}{\bangLCtxt<\oc t'_2>}
            \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt<t'_1\isub{x}{t'_2}> = s$ and $u_2 =
            \bangLCtxt<t_1\isub{x}{t'_2}> \bangArr_{S_\indexOmega}<R>
            \bangLCtxt<t'_1\isub{x}{t'_2}> = s$ Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{\bangLCtxt<\oc t'_2>}       &\bangArr_{S_\indexOmega}<R>    &t'_1\esub{x}{\bangLCtxt<\oc t'_2>}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \bangLCtxt<t_1\isub{x}{t'_2}>           &\bangArr_{S_\indexOmega}<R>    &\bangLCtxt<t'_1\isub{x}{t'_2}>
            \end{array}
            \end{equation*}

        \item[\bltIII] $t'_2 \bangArr_{S_\indexOmega}<R> t''_2$ and
            $u_1 = t_1\esub{x}{\bangLCtxt<\oc t''_2>}$ for some term
            $t'_2 \in \bangSetTerms$: We set $s :=
            \bangLCtxt<t_1\isub{x}{t''_2}>$ which concludes this case
            since by induction on $t_1$, one has that
            $t_1\isub{x}{t'_2} \bangArr*_{S_\indexOmega}<R>
            t_1\isub{x}{t''_2}$ thus by contextual closure $u_1 =
            t_1\esub{x}{\bangLCtxt<\oc t''_2>}
            \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt<t_1\isub{x}{t''_2}> = s$ and $u_2 =
            \bangLCtxt<t_1\isub{x}{t'_2}> \bangArr*_{S_\indexOmega}<R>
            \bangLCtxt<t_1\isub{x}{t''_2}> = s$. Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{\bangLCtxt<\oc t'_2>}       &\bangArr_{S_\indexOmega}<R>    &t_1\esub{x}{\bangLCtxt<\oc t''_2>}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                   \bangLCtxt<t_1\isub{x}{t'_2}>            &\bangArr^*_{S_\indexOmega}<R>  &\bangLCtxt<t_1\isub{x}{t''_2}>
            \end{array}
            \end{equation*}

        \item[\bltIII] $\bangLCtxt \bangArr_{S_\indexOmega}<R>
            \bangLCtxt'$ and $u_1 = t_1\esub{x}{\bangLCtxt'<\oc
            t'_2>}$ for some context $\bangLCtxt'$: We set $s :=
            \bangLCtxt'<t_1\isub{x}{t'_2}>$ which concludes this case
            since by
            \Cref{lem:Bang_Full_dB_d!_Context_Reduction_Lifted_to_Terms},
            $u_1 = t_1\esub{x}{\bangLCtxt'<\oc t'_2>}
            \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt'<t_1\isub{x}{t'_2}> = s$ and $u_2 =
            \bangLCtxt<t_1\isub{x}{t'_2}> \bangArr_{S_\indexOmega}<R>
            \bangLCtxt'<t_1\isub{x}{t'_2}> = s$. Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{\bangLCtxt<\oc t'_2>}       &\bangArr_{S_\indexOmega}<R>    &   t_1\esub{x}{\bangLCtxt'<\oc t'_2>}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                   \bangLCtxt<t_1\isub{x}{t'_2}>            &\bangArr_{S_\indexOmega}<R>    & \bangLCtxt'<t_1\isub{x}{t'_2}>
            \end{array}
            \end{equation*}
        \end{itemize}

    \item[\bltII] Otherwise: By hypothesis $t
        \bangArr_{S_\indexOmega}<R> u_1$ and $t
        \bangArr_{S_\indexOmega}<s!> u_2$, and four cases can thus be
        distinguished:
        \begin{itemize}
        \item[\bltIII] $u_1 = u'_1\esub{x}{t_2}$ and $u_2 =
            u'_2\esub{x}{t_2}$ with $t_1 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_1 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: By \ih on $t_1$, there
            exists $s' \in \bangSetTerms$ such that $u'_1
            \bangArr_{S_\indexOmega}<s!> s'$ and $u'_2
            \bangArr*_{S_\indexOmega}<R> s'$. We set $s :=
            s'\esub{x}{t_2}$ since by contextual closure $u_1 =
            u'_1\esub{x}{t_2} \bangArr_{S_\indexOmega}<s!>
            s'\esub{x}{t_2} = s'$ and $u_2 = u'_2\esub{x}{t_2}
            \bangArr*_{S_\indexOmega}<R> u'_2\esub{x}{t_2} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                        &\bangArr_{S_\indexOmega}<R>    &  u'_1\esub{x}{t_2}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    u'_2\esub{x}{t_2}                       &\bangArr*_{S_\indexOmega}<R>   & s'\esub{x}{t_2}   
              \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = u'_1\esub{x}{t_2}$ and $u_2 =
            t_1\esub{x}{u'_2}$ with $t_1 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_2 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: We set $s' :=
            u'_1\esub{x}{u'_2}$ since by contextual closure $u_1 =
            u'_1\esub{x}{t_2} \bangArr_{S_\indexOmega}<s!>
            u'_1\esub{x}{u'_2} = s'$ and $u_2 = u'_1\esub{x}{u'_2}
            \bangArr_{S_\indexOmega}<R> u'_1\esub{x}{u'_2} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                        &\bangArr_{S_\indexOmega}<R>    &u'_1\esub{x}{t_2}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
              \\[0.2cm]
                    t_1\esub{x}{u'_2}                       &\bangArr_{S_\indexOmega}<R>    &u'_1\esub{x}{u'_2}   
              \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = t_1\esub{x}{u'_1}$ and $u_2 =
            u'_2\esub{x}{t_2}$ with $t_2 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_1 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: We set $s' :=
            u'_2\esub{x}{u'_1}$ since by contextual closure $u_1 =
            t_1\esub{x}{u'_1} \bangArr_{S_\indexOmega}<s!>
            u'_2\esub{x}{u'_1} = s'$ and $u_2 = u'_2\esub{x}{t_2}
            \bangArr_{S_\indexOmega}<R> u'_2\esub{x}{u'_1} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                        &\bangArr_{S_\indexOmega}<R>    &  t_1\esub{x}{u'_1}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    u'_2\esub{x}{t_2}                       &\bangArr_{S_\indexOmega}<R>    & u'_2\esub{x}{u'_1}
              \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = t_1\esub{x}{u'_1}$ and $u_2 =
            t_1\esub{x}{u'_2}$ with $t_2 \bangArr_{S_\indexOmega}<R>
            u'_1$ and $t_2 \bangArr_{S_\indexOmega}<s!> u'_2$ for some
            $u'_1, u'_2 \in \bangSetTerms$: By \ih on $t_2$, there
            exists $s' \in \bangSetTerms$ such that $u'_1
            \bangArr_{S_\indexOmega}<s!> s'$ and $u'_2
            \bangArr*_{S_\indexOmega}<R> s'$. We set $s :=
            t_1\esub{x}{s'}$ since by contextual closure $u_1 =
            t_1\esub{x}{u'_1} \bangArr_{S_\indexOmega}<s!>
            t_1\esub{x}{s'} = s'$ and $u_2 = t_1\esub{x}{u'_2}
            \bangArr*_{S_\indexOmega}<R> t_1\esub{x}{s'} = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                        &\bangArr_{S_\indexOmega}<R>    &t_1\esub{x}{u'_1}
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    t_1\esub{x}{u'_2}                       &\bangArr^*_{S_\indexOmega}<R>  &t_1\esub{x}{s'}
              \end{array}
            \end{equation*}
        \end{itemize}
    \end{itemize}

\item[\bltI] $t = \der{t'_0}$:  We distinguish two cases:
    \begin{itemize}
    \item[\bltII] $t$ is the $\bangSymbBang$-redex reduced in the step
        $t \bangArr_{S_\indexOmega}<d!> u_1$: Then $t =
        \der{\bangLCtxt<\oc t'>}$ and $u_1 = \bangLCtxt<t'>$ for some
        context $\bangLCtxt$ and some term $t' \in \bangSetTerms$. By
        hypothesis $\der{\bangLCtxt<\oc t'>}
        \bangArr_{S_\indexOmega}<s!> u_2$ so that three different
        cases can be distinguished:
        \begin{itemize}
        \item[\bltIII] $t' \bangArr_{S_\indexOmega}<s!> t''$ and $u_2
            = \der{\bangLCtxt<\oc t''>}$ for some $t'' \in
            \bangSetTerms$: We set $s := \bangLCtxt<t''>$ which
            concludes this case since by contextual closure $u_1 =
            \bangLCtxt<t'> \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt<t''> = s'$ and $u_2 = \der{\bangLCtxt<\oc t''>}
            \bangArr_{S_\indexOmega}<d!> \bangLCtxt<t''> = s'$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \der{\bangLCtxt<\oc t'>}                &\bangArr_{S_\indexOmega}<d!>   &\bangLCtxt<t'>
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \der{\bangLCtxt<\oc t''>}               &\bangArr_{S_\indexOmega}<d!>   &\bangLCtxt<t''>
                \end{array}
            \end{equation*}

        \item[\bltIII] $\bangLCtxt \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt'$ and $u_2 = \der{\bangLCtxt'<\oc t'>}$ for
            some context $\bangLCtxt'$: We set $s := \bangLCtxt'<t'>$
            which concludes this case since by
            \Cref{lem:Bang_Full_dB_d!_Context_Reduction_Lifted_to_Terms}
            $u_1 = \bangLCtxt<t'> \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt'<t'> = s$ and $u_2 = \der{\bangLCtxt'<\oc t'>}
            \bangArr_{S_\indexOmega}<d!> \bangLCtxt'<t'> = s$.
            Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \der{\bangLCtxt<\oc t'>}                &\bangArr_{S_\indexOmega}<d!>   &\bangLCtxt<t'>
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \der{\bangLCtxt'<\oc t'>}               &\bangArr_{S_\indexOmega}<d!>   &\bangLCtxt'<t'>
                \end{array}
            \end{equation*}

        \item[\bltIII] $\bangLCtxt =
            \bangLCtxt_1<\bangLCtxt_3\esub{x}{\bangLCtxt_2<\oc t''>}>$
            and $u_2 =
            \der{\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t''}\bangCtxtPlug{\oc
            t'\isub{x}{t''}}>>}$ for some context $\bangLCtxt_1,
            \bangLCtxt_2, \bangLCtxt_3$ and some term $t'' \in
            \bangSetTerms$: We set $s =
            \bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t''}\bangCtxtPlug{t'}>>$
            which concludes this case since by contextual closure $u_1
            = \bangLCtxt_1<\bangLCtxt_3<t'>\esub{x}{\bangLCtxt_2<\oc
            t''>}> \bangArr_{S_\indexOmega}<s!>
            \bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t''}\bangCtxtPlug{t'\isub{x}{t''}}>>
            = s$ and $u_2 =
            \der{\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t''}\bangCtxtPlug{\oc
            t'\isub{x}{t''}}>>} \bangArr_{S_\indexOmega}<d!>
            \bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t''}\bangCtxtPlug{t'\isub{x}{t''}}>>
            = s$. Graphically,
            \begin{equation*}
                \begin{array}{lll}
                    \der{\bangLCtxt_1<\bangLCtxt_3<\oc t'>\esub{x}{\bangLCtxt_2<\oc t''>}>}                         &\bangArr_{S_\indexOmega}<R>    &\bangLCtxt_1<\bangLCtxt_3<t'>\esub{x}{\bangLCtxt_2<\oc t''>}>
                \\[0.2cm]
                    \;\;\bangDownArr_{S_\indexOmega}<s!>                                                            &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                    \der{\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t''}\bangCtxtPlug{\oc t'\isub{x}{t''}}>>}   &\bangArr_{S_\indexOmega}<R>    &\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t''}\bangCtxtPlug{t'\isub{x}{t''}}>>   
                \end{array}
            \end{equation*}
        \end{itemize}

    \item[\bltII] Otherwise: Since by hypothesis $t
        \bangArr_{S_\indexOmega}<R> u_1$ and $t
        \bangArr_{S_\indexOmega}<s!> u_2$, then necessarily $u_1 =
        \der{u'_1}$ and $u_2 = \der{u'_2}$ for some $u'_1, u'_2 \in
        \bangSetTerms$ such that $t'_0 \bangArr_{S_\indexOmega}<R>
        u'_1$ and $t'_0 \bangArr_{S_\indexOmega}<s!> u'_2$. By \ih on
        $t'$, there exists $s' \in \bangSetTerms$ such that $u'_1
        \bangArr_{S_\indexOmega}<s!> s'$ and $u'_2
        \bangArr*_{S_\indexOmega}<R> s'$. We set $s := \der{s'}$ since
        by contextual closure $u_1 = \der{u'_1}
        \bangArr_{S_\indexOmega}<s!> \der{s'} = s'$ and $u_2 =
        \der{u'_2} \bangArr*_{S_\indexOmega}<R> \der{s'} = s'$.
        Graphically,
        \begin{equation*}
            \begin{array}{lll}
                \der{t'_0}                              &\bangArr_{S_\indexOmega}<R>    &\der{u'_1}
            \\[0.2cm]
                \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
            \\[0.2cm]
                \der{u'_1}                              &\bangArr_{S_\indexOmega}<R>    &\der{s'}
            \end{array}
        \end{equation*}
    \end{itemize}

\item[\bltI] $t = \oc t'$: Since by hypothesis $t
    \bangArr_{S_\indexOmega}<R> u_1$ and $t
    \bangArr_{S_\indexOmega}<s!> u_2$, then necessarily $u_1 = \oc
    u'_1$ and $u_2 = \oc u'_2$ for some $u'_1, u'_2 \in \bangSetTerms$
    such that $t \bangArr_{S_\indexOmega}<R> u'_1$ and $t
    \bangArr_{S_\indexOmega}<s!> u'_2$. By \ih on $t'$, there exists
    $s' \in \bangSetTerms$ such that $u'_1
    \bangArr_{S_\indexOmega}<s!> s'$ and $u'_2
    \bangArr*_{S_\indexOmega}<R> s'$. We set $s := \oc s'$ since by
    contextual closure $u_1 = \oc u'_1 \bangArr_{S_\indexOmega}<s!>
    \oc s' = s'$ and $u_2 = \oc u'_2 \bangArr*_{S_\indexOmega}<R> \oc
    s' = s'$. Graphically,
    \begin{equation*}
        \begin{array}{lll}
            \oc t'                                  &\bangArr_{S_\indexOmega}<R>    &\oc u'_1
        \\[0.2cm]
            \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
        \\[0.2cm]
          \oc u'_2                                  &\bangArr*_{S_\indexOmega}<R>   &\oc s'
        \end{array}
    \end{equation*}
\end{itemize}
\end{proof}


==> 2_Proofs/Bang_Full_dB_d__Context_Reduction_Lifted_to_Terms.tex <==
\begin{proof}
We distinguish two cases:
\begin{itemize}
\item[\bltI] $\rel = \bangSymbBeta$: By definition, there exist three
    contexts $\bangStratCtxt_\indexOmega,
    \bangStratCtxt_\indexOmega^{1'}$ and
    $\bangStratCtxt_\indexOmega^{2'}$ such that
    $\bangStratCtxt_\indexOmega^1 =
    \bangStratCtxt_\indexOmega<\bangStratCtxt_\indexOmega^{1'}>$,
    $\bangStratCtxt_\indexOmega^2 =
    \bangStratCtxt_\indexOmega<\bangStratCtxt_\indexOmega^{2'}>$ and
    $\bangStratCtxt_\indexOmega^{1'} \mapstoR[\rel']
    \bangStratCtxt_\indexOmega^{2'}$ for some $\rel' \in
    \{\bangSymbBeta_1, \bangSymbBeta_2, \bangSymbBeta_3\}$. We
    distinguish three cases:
    \begin{itemize}
    \item[\bltII] $\rel' = \bangSymbBeta_1$: Then
        $\bangStratCtxt_\indexOmega^{1'} =
        \app{\bangLCtxt<\abs{x}{\bangStratCtxt'_\indexOmega}>}{u}$ and
        $\bangStratCtxt_\indexOmega^{2'} =
        \bangLCtxt<\bangStratCtxt'_\indexOmega\esub{x}{u}>$. Thus
        $\bangStratCtxt_\indexOmega^{1'}<t> =
        \app{\bangLCtxt<\abs{x}{\bangStratCtxt'_\indexOmega<t>}>}{u}$
        and $\bangStratCtxt_\indexOmega^{2'}<t> =
        \bangLCtxt<\bangStratCtxt'_\indexOmega<t>\esub{x}{u}>$.
        Therefore $\bangStratCtxt_\indexOmega^{1'}<t>
        \mapstoR[\bangSymbBeta] \bangStratCtxt_\indexOmega^{2'}<t>$
        hence $\bangStratCtxt_\indexOmega^1<t>
        \bangArr_{S_\indexOmega}<dB> \bangStratCtxt_\indexOmega^2<t>$.

    \item[\bltII] $\rel' = \bangSymbBeta_2$: Then
        $\bangStratCtxt_\indexOmega^{1'} =
        \app{\bangLCtxt<\abs{x}{t}>}{\bangStratCtxt'_\indexOmega}$ and
        $\bangStratCtxt_\indexOmega^{2'} =
        \bangLCtxt<t\esub{x}{\bangStratCtxt'_\indexOmega}>$. Thus
        $\bangStratCtxt_\indexOmega^{1'}<t> =
        \app{\bangLCtxt<\abs{x}{t}>}{\bangStratCtxt'_\indexOmega<t>}$
        and $\bangStratCtxt_\indexOmega^{2'}<t> =
        \bangLCtxt<t\esub{x}{\bangStratCtxt'_\indexOmega<t>}>$.
        Therefore $\bangStratCtxt_\indexOmega^{1'}<t>
        \mapstoR[\bangSymbBeta] \bangStratCtxt_\indexOmega^{2'}<t>$
        hence $\bangStratCtxt_\indexOmega^1<t>
        \bangArr_{S_\indexOmega}<dB> \bangStratCtxt_\indexOmega^2<t>$.

    \item[\bltII] $\rel' = \bangSymbBeta_3$: Then
        $\bangStratCtxt_\indexOmega^{1'} =
        \app{\bangLCtxt_1<\bangLCtxt_2<\abs{x}{t}>\esub{y}{\bangStratCtxt'_\indexOmega}>}{u}$
        and $\bangStratCtxt_\indexOmega^{2'} =
        \bangLCtxt_1<\bangLCtxt_2<t\esub{x}{u}>\esub{y}{\bangStratCtxt'_\indexOmega}>$.
        Thus $\bangStratCtxt_\indexOmega^{1'}<t> =
        \app{\bangLCtxt_1<\bangLCtxt_2<\abs{x}{t}>\esub{y}{\bangStratCtxt'_\indexOmega<t>}>}{u}$
        and $\bangStratCtxt_\indexOmega^{2'}<t> =
        \bangLCtxt_1<\bangLCtxt_2<t\esub{x}{u}>\esub{y}{\bangStratCtxt'_\indexOmega<t>}>$.
        Therefore $\bangStratCtxt_\indexOmega^{1'}<t>
        \mapstoR[\bangSymbBeta] \bangStratCtxt_\indexOmega^{2'}<t>$
        hence $\bangStratCtxt_\indexOmega^1<t>
        \bangArr_{S_\indexOmega}<dB> \bangStratCtxt_\indexOmega^2<t>$.
    \end{itemize}

\item[\bltI] $\rel = \bangSymbBang$: By definition, there exist three
    contexts $\bangStratCtxt_\indexOmega,
    \bangStratCtxt_\indexOmega^{1'}$ and
    $\bangStratCtxt_\indexOmega^{2'}$ such that
    $\bangStratCtxt_\indexOmega^1 =
    \bangStratCtxt_\indexOmega<\bangStratCtxt_\indexOmega^{1'}>$,
    $\bangStratCtxt_\indexOmega^2 =
    \bangStratCtxt_\indexOmega<\bangStratCtxt_\indexOmega^{2'}>$ and
    $\bangStratCtxt_\indexOmega^{1'} \mapstoR[\rel']
    \bangStratCtxt_\indexOmega^{2'}$ for some $\rel' \in
    \{\bangSymbBang_1, \bangSymbBang_2\}$.
    \begin{itemize}
    \item[\bltII] $\rel' = \bangSymbBang_1$: Then
        $\bangStratCtxt_\indexOmega^{1'} = \der{\bangLCtxt<\oc
        \bangStratCtxt'_\indexOmega>}$ and
        $\bangStratCtxt_\indexOmega^{2'} =
        \bangLCtxt<\bangStratCtxt'_\indexOmega>$. Thus
        $\bangStratCtxt_\indexOmega^{1'}<t> = \der{\bangLCtxt<\oc
        \bangStratCtxt'_\indexOmega<t>>}$ and
        $\bangStratCtxt_\indexOmega^{2'}<t> =
        \bangLCtxt<\bangStratCtxt'_\indexOmega<t>>$. Therefore
        $\bangStratCtxt_\indexOmega^{1'}<t> \mapstoR[\bangSymbBang]
        \bangStratCtxt_\indexOmega^{2'}<t>$ hence
        $\bangStratCtxt_\indexOmega^1<t> \bangArr_{S_\indexOmega}<dB>
        \bangStratCtxt_\indexOmega^2<t>$.

    \item[\bltII] $\rel' = \bangSymbBang_2$: Then
        $\bangStratCtxt_\indexOmega^{1'} =
        \der{\bangLCtxt_1<\bangLCtxt_2<\oc
        s>\esub{x}{\bangStratCtxt'_\indexOmega}>}$ and
        $\bangStratCtxt_\indexOmega^{2'} =
        \bangLCtxt_1<\bangLCtxt_2<s>\esub{x}{\bangStratCtxt'_\indexOmega}>$.
        Thus $\bangStratCtxt_\indexOmega^{1'}<t> =
        \der{\bangLCtxt_1<\bangLCtxt_2<\oc
        s>\esub{x}{\bangStratCtxt'_\indexOmega<t>}>}$ and
        $\bangStratCtxt_\indexOmega^{2'}<t> =
        \bangLCtxt_1<\bangLCtxt_2<s>\esub{x}{\bangStratCtxt'_\indexOmega<t>}>$.
        Therefore $\bangStratCtxt_\indexOmega^{1'}<t>
        \mapstoR[\bangSymbBang] \bangStratCtxt_\indexOmega^{2'}<t>$
        hence $\bangStratCtxt_\indexOmega^1<t>
        \bangArr_{S_\indexOmega}<dB> \bangStratCtxt_\indexOmega^2<t>$.
        \qedhere
    \end{itemize}
\end{itemize}
\end{proof}

==> 2_Proofs/Bang_Full_dB_d__Diamond.tex <==
\begin{proof}
Let $t, u_1, u_2 \in \bangSetTerms$ such that $u_1 \neq u_2$ with $t
\bangArr_{S_\indexOmega}<R_1> u_1$ and $t
\bangArr_{S_\indexOmega}<R_2> u_2$ for some $\rel_1, \rel_2 \in
\{\bangSymbBeta, \bangSymbBang\}$. Let us show that there exists $s
\in \bangSetTerms$ such that $u_1 \bangArr_{S_\indexOmega}<R_2> s$ and
$u_2 \bangArr_{S_\indexOmega}<R_1> s$. We distinguish two cases:
\begin{itemize}
\item[\bltI] $\rel_1 = \bangSymbBeta$: By definition, there exist
    $\bangStratCtxt_\indexOmega$, $\bangLCtxt$, $s_1, s_2 \in
    \bangSetTerms$ such that $t =
    \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>$
    and $u_1 =
    \bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>$. Since
    $u_1 \neq u_2$, then the step $t \bangArr_{S_\indexOmega}<R_2>
    u_2$ either happens in $\bangStratCtxt_\indexOmega$, $\bangLCtxt$,
    $s_1$ or $s_2$.
    \begin{itemize}
    \item[\bltII] $\bangStratCtxt_\indexOmega
        \bangArr_{S_\indexOmega}<R_2> \bangStratCtxt'_\indexOmega$
        with $u_2 =
        \bangStratCtxt'_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>$:
        We set $s :=
        \bangStratCtxt'_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>$
        which concludes this case since using
        \Cref{lem:Bang_Full_dB_d!_Context_Reduction_Lifted_to_Terms}:
        \begin{equation*}
            \begin{array}{ccc}
                \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>     &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>
            \\[0.1cm]
                \bangDownArr_{S_\indexOmega}<R_2>                                   &                               &\bangDownArr_{S_\indexOmega}<R_2>
            \\[0.1cm]
                \bangStratCtxt'_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>    &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt'_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>
            \end{array}
        \end{equation*}

    \item[\bltII] $\bangLCtxt_\indexOmega
        \bangArr_{S_\indexOmega}<R_2> \bangLCtxt'_\indexOmega$ with
        $u_2 =
        \bangStratCtxt_\indexOmega<\app{\bangLCtxt'<\abs{x}{s_1}>}{s_2}>$:
        We set $s :=
        \bangStratCtxt_\indexOmega<\bangLCtxt'<s_1\esub{x}{s_2}>>$
        which concludes this case since using
        \Cref{lem:Bang_Full_dB_d!_Context_Reduction_Lifted_to_Terms}:
        \begin{equation*}
            \begin{array}{ccc}
                \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>     &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>
            \\[0.1cm]
                \bangDownArr_{S_\indexOmega}<R_2>                                   &                               &\bangDownArr_{S_\indexOmega}<R_2>
            \\[0.1cm]
                \bangStratCtxt_\indexOmega<\app{\bangLCtxt'<\abs{x}{s_1}>}{s_2}>    &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt'<s_1\esub{x}{s_2}>>
            \end{array}
        \end{equation*}

    \item[\bltII] $s_1 \bangArr_{S_\indexOmega}<R_2> s'_1$ with $u_2 =
        \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s'_1}>}{s_2}>$:
        We set $s :=
        \bangStratCtxt_\indexOmega<\bangLCtxt<s'_1\esub{x}{s_2}>>$
        which concludes this case since:
        \begin{equation*}
            \begin{array}{ccc}
                \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>     &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>
            \\[0.1cm]
                \bangDownArr_{S_\indexOmega}<R_2>                                   &                               &\bangDownArr_{S_\indexOmega}<R_2>
            \\[0.1cm]
                \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s'_1}>}{s_2}>    &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s'_1\esub{x}{s_2}>>
            \end{array}
        \end{equation*}

    \item[\bltII] $s_2 \bangArr_{S_\indexOmega}<R_2> s'_2$ with $u_2 =
        \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s'_2}>$:
        We set $s :=
        \bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s'_2}>>$
        which concludes this case since:
        \begin{equation*}
            \begin{array}{ccc}
                \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>     &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>
            \\[0.1cm]
                \bangDownArr_{S_\indexOmega}<R_2>                                   &                               &\bangDownArr_{S_\indexOmega}<R_2>
            \\[0.1cm]
                \bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s'_2}>    &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s'_2}>>
            \end{array}
        \end{equation*}
    \end{itemize}

\item[\bltI] $\rel_1 = \bangSymbBang$: By definition, there exist
    $\bangStratCtxt_\indexOmega$, $\bangLCtxt$, $s \in \bangSetTerms$
    such that $t = \bangStratCtxt_\indexOmega<\der{\bangLCtxt<\oc
    s>}>$ and $u_1 = \bangStratCtxt_\indexOmega<\bangLCtxt<s>>$. Since
    $u_1 \neq u_2$, then the step $t \bangArr_{S_\indexOmega}<R_2>
    u_2$ either happens in $\bangStratCtxt_\indexOmega$, $\bangLCtxt$
    or $s$.
    \begin{itemize}
    \item[\bltII] $\bangStratCtxt_\indexOmega
        \bangArr_{S_\indexOmega}<R_2> \bangStratCtxt'_\indexOmega$
        with $u_2 = \bangStratCtxt'_\indexOmega<\der{\bangLCtxt<\oc
        s>}>$: We set $s :=
        \bangStratCtxt'_\indexOmega<\bangLCtxt<s>>$ which concludes
        this case since using
        \Cref{lem:Bang_Full_dB_d!_Context_Reduction_Lifted_to_Terms}:
        \begin{equation*}
            \begin{array}{ccc}
                \bangStratCtxt_\indexOmega<\der{\bangLCtxt<\oc s>}>     &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s>>
            \\[0.1cm]
                \bangDownArr_{S_\indexOmega}<R_2>                       &                               &\bangDownArr_{S_\indexOmega}<R_2>
            \\[0.1cm]
                \bangStratCtxt'_\indexOmega<\der{\bangLCtxt<\oc s>}>    &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt'_\indexOmega<\bangLCtxt<s>>
            \end{array}
        \end{equation*}

    \item[\bltII] $\bangLCtxt_\indexOmega
        \bangArr_{S_\indexOmega}<R_2> \bangLCtxt'_\indexOmega$ with
        $u_2 = \bangStratCtxt_\indexOmega<\der{\bangLCtxt'<\oc s>}>$:
        We set $s := \bangStratCtxt_\indexOmega<\bangLCtxt'<s>>$ which
        concludes this case since using
        \Cref{lem:Bang_Full_dB_d!_Context_Reduction_Lifted_to_Terms}:
        \begin{equation*}
            \begin{array}{ccc}
                \bangStratCtxt_\indexOmega<\der{\bangLCtxt<\oc s>}>     &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s>>
            \\[0.1cm]
                \bangDownArr_{S_\indexOmega}<R_2>                       &                               &\bangDownArr_{S_\indexOmega}<R_2>
            \\[0.1cm]
                \bangStratCtxt_\indexOmega<\der{\bangLCtxt'<\oc s>}>    &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt'<s>>
            \end{array}
        \end{equation*}

    \item[\bltII] $s \bangArr_{S_\indexOmega}<R_2> s'$ with $u_2 =
        \bangStratCtxt_\indexOmega<\der{\bangLCtxt<\oc s'>}>$: We set
        $s := \bangStratCtxt_\indexOmega<\bangLCtxt<s'>>$ which
        concludes this case since:
        \begin{equation*}
            \begin{array}{ccc}
                \bangStratCtxt_\indexOmega<\der{\bangLCtxt<\oc s>}>     &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s>>
            \\[0.1cm]
                \bangDownArr_{S_\indexOmega}<R_2>                       &                               &\bangDownArr_{S_\indexOmega}<R_2>
            \\[0.1cm]
                \bangStratCtxt_\indexOmega<\der{\bangLCtxt<\oc s'>}>    &\bangArr_{S_\indexOmega}<R_1>  &\bangStratCtxt_\indexOmega<\bangLCtxt<s'>>
            \end{array}
        \end{equation*}
    \end{itemize}
\end{itemize}
\end{proof}


==> 2_Proofs/Bang_Full_dB_d__Terminating.tex <==
\begin{proof}
Let $t, u \in \bangSetTerms$ such that $t \bangArr_{S_\indexOmega}<dB>
u$ (\resp $t \bangArr_{S_\indexOmega}<d!> u$).

By definition, there exist a context $\bangStratCtxt_\indexOmega$ and
terms $s_1, s_2$ such that $t =
\bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>$
(\resp $t = \bangStratCtxt_\indexOmega<\der{\bangLCtxt<\oc s_1>}>$)
and $u = \bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>$
(\resp $u = \bangStratCtxt_\indexOmega<\bangLCtxt<s_1>>$). Using
\Cref{lem:Bang_Term_Size_with_Context}, one has that:
\begin{equation*}
    \begin{array}{rcl}
        \termSize{t}
            &=& \termSize{\bangStratCtxt_\indexOmega<\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}>}
            = \termSize{\bangStratCtxt_\indexOmega} + \termSize{\app{\bangLCtxt<\abs{x}{s_1}>}{s_2}}
            = \termSize{\bangStratCtxt_\indexOmega} + 2 + \termSize{\bangLCtxt} + \termSize{s_1} + \termSize{s_2}
        \\
            &>& \termSize{\bangStratCtxt_\indexOmega} + 1 + \termSize{\bangLCtxt} + \termSize{s_1} + \termSize{s_2}
            = \termSize{\bangStratCtxt_\indexOmega} + \termSize{\bangLCtxt<s_1\esub{x}{s_2}>}
            = \termSize{\bangStratCtxt_\indexOmega<\bangLCtxt<s_1\esub{x}{s_2}>>}
            = \termSize{u}
    \\[0.2cm]
        (\resp\quad \termSize{t}
            &=& \termSize{\bangStratCtxt_\indexOmega<\bangLCtxt<\oc s_1>>}
            = \termSize{\bangStratCtxt_\indexOmega} + \termSize{\bangLCtxt<\oc s_1>}
            = \termSize{\bangStratCtxt_\indexOmega} + 2 + \termSize{\bangLCtxt} + \termSize{s_1}
        \\
            &>& \termSize{\bangStratCtxt_\indexOmega} + 1 + \termSize{\bangLCtxt} + \termSize{s_1}
            = \termSize{\bangStratCtxt_\indexOmega} + \termSize{\bangLCtxt<s_1>}
            = \termSize{\bangStratCtxt_\indexOmega<\bangLCtxt<s_1>>}
            = \termSize{u}\quad)
    \end{array}
\end{equation*}
One thus deduces that $\bangArr_{S_\indexOmega}<dB> \cup
\bangArr_{S_\indexOmega}<d!>$ is terminating.
\end{proof}

==> 2_Proofs/Bang_Full_s__Context_Reduction_Lifted_to_Terms.tex <==
\begin{proof}
By definition, there exist three contexts $\bangStratCtxt_\indexOmega,
\bangStratCtxt_\indexOmega^{1'}$ and $\bangStratCtxt_\indexOmega^{2'}$
such that $\bangStratCtxt_\indexOmega^1 =
\bangStratCtxt_\indexOmega<\bangStratCtxt_\indexOmega^{1'}>$,
$\bangStratCtxt_\indexOmega^2 =
\bangStratCtxt_\indexOmega<\bangStratCtxt_\indexOmega^{2'}>$ and
$\bangStratCtxt_\indexOmega^{1'} \mapstoR[\rel]
\bangStratCtxt_\indexOmega^{2'}$ for some $\rel \in \{\bangSymbSubs_1,
\bangSymbSubs_2\}$. We distinguish two cases:
\begin{itemize}
\item[\bltIII] $\rel = \bangSymbSubs_1$: Then
    $\bangStratCtxt_\indexOmega^{1'} =
    t\esub{x}{\bangLCtxt_1<\bangLCtxt_2<\oc
    u>\esub{y}{\bangStratCtxt_\indexOmega}>}$ and
    $\bangStratCtxt_\indexOmega^{2'} =
    \bangLCtxt_1<\bangLCtxt_2<t\isub{x}{u}>\esub{y}{\bangStratCtxt_\indexOmega}>$.
    Thus $\bangStratCtxt_\indexOmega^{1'}<t> =
    t\esub{x}{\bangLCtxt_1<\bangLCtxt_2<\oc
    u>\esub{y}{\bangStratCtxt_\indexOmega<t>}>}$ and
    $\bangStratCtxt_\indexOmega^{2'}<t> =
    \bangLCtxt_1<\bangLCtxt_2<t\isub{x}{u}>\esub{y}{\bangStratCtxt_\indexOmega<t>}>$.
    Therefore $\bangStratCtxt_\indexOmega^{1'}<t>
    \mapstoR[\bangSymbSubs] \bangStratCtxt_\indexOmega^{2'}<t>$ hence
    $\bangStratCtxt_\indexOmega^1<t> \bangArr_{S_\indexOmega}<s!>
    \bangStratCtxt_\indexOmega^2<t>$.

\item[\bltIII] $\rel = \bangSymbSubs_2$: Then
    $\bangStratCtxt_\indexOmega^{1'} =
    t\esub{x}{\bangLCtxt<\oc\bangStratCtxt_\indexOmega>}$ and
    $\bangStratCtxt_\indexOmega^{2'} =
    \bangLCtxt<t\isub{x}{\bangStratCtxt_\indexOmega}>$. Thus
    $\bangStratCtxt_\indexOmega^{1'}<t> =
    t\esub{x}{\bangLCtxt<\oc\bangStratCtxt_\indexOmega<t>>}$ and
    $\bangStratCtxt_\indexOmega^{2'}<t> =
    \bangLCtxt<t\isub{x}{\bangStratCtxt_\indexOmega<t>}>$. Therefore
    $\bangStratCtxt_\indexOmega^{1'}<t> \mapstoR[\bangSymbSubs]
    \bangStratCtxt_\indexOmega^{2'}<t>$ hence
    $\bangStratCtxt_\indexOmega^1<t> \bangArr_{S_\indexOmega}<s!>
    \bangStratCtxt_\indexOmega^2<t>$.
    \qedhere
\end{itemize}
\end{proof}

==> 2_Proofs/Bang_Full_s__Locally_Confluent.tex <==
\begin{proof}
Let $t, u_1, u_2 \in \bangSetTerms$ such that $t
\bangArr_{S_\indexOmega}<s!> u_1$, $t \bangArr_{S_\indexOmega}<s!>
u_2$ and $u_1 \neq u_2$. We reason by induction on $t$:
\begin{itemize}
\item[\bltI] $t = x$: Impossible since it contradicts $t
    \bangArr_{S_\indexOmega}<s!> u_1$.

\item[\bltI] $t = \abs{x}{t'}$: Since $t$ cannot be a
    $\bangSymbSubs$-redex, then necessarily
    $u_1 = \abs{x}{t'_1}$ and $u_2 = \abs{x}{t'_2}$ with $t'
    \bangArr_{S_\indexOmega}<s!> t'_1$ and $t'
    \bangArr_{S_\indexOmega}<s!> t'_2$. By \ih on $t'$, there exists
    $s' \in \bangSetTerms$ such that $t_1
    \bangArr*_{S_\indexOmega}<s!> s'$ and $t_2
    \bangArr*_{S_\indexOmega}<s!> s'$. We set $s := \abs{x}{s'}$
    concluding this case since by contextual closure:
    \begin{equation*}
        \begin{array}{lll}
            \abs{x}{t'}                             &\bangArr_{S_\indexOmega}<s!>   &\abs{x}{t'_1}
    \\[0.2cm]
            \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr*_{S_\indexOmega}<s!>
    \\[0.2cm]
            \abs{x}{t'_2}                           &\bangArr*_{S_\indexOmega}<s!>  &\abs{x}{s'}
        \end{array}
    \end{equation*}

\item[\bltI] $t = \app{t_1}{t_2}$: Since $t$ cannot be a
    $\bangSymbSubs$-redex, four different
    cases can be distinguished:
    \begin{itemize}
    \item[\bltII] $u_1 = \app{u'_1}{t_2}$, $u_2 = \app{u'_2}{t_2}$
        with $t_1 \bangArr_{S_\indexOmega}<s!> u'_1$ and $t_1
        \bangArr_{S_\indexOmega}<s!> u'_2$: By \ih on $t_1$, there
        exists $s_1 \in \bangSetTerms$ such that $u'_1
        \bangArr*_{S_\indexOmega}<s!> s_1$ and $u'_2
        \bangArr*_{S_\indexOmega}<s!> s_1$. We set $s :=
        \app{s_1}{t_2}$ concluding this case since by contextual
        closure:
        \begin{equation*}
            \begin{array}{lll}
                \app{t_1}{t_2}                          &\bangArr_{S_\indexOmega}<s!>   &\app{u'_1}{t_2}
        \\[0.2cm]
                \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr*_{S_\indexOmega}<s!>
        \\[0.2cm]
                \app{u'_2}{t_2}                         &\bangArr*_{S_\indexOmega}<s!>  &\app{s_1}{t_2}
            \end{array}
        \end{equation*}

    \item[\bltII] $u_1 = \app{u'_1}{t_2}$, $u_2 = \app{t_1}{u'_2}$
        with $t_1 \bangArr_{S_\indexOmega}<s!> u'_1$ and $t_2
        \bangArr_{S_\indexOmega}<s!> u'_2$: We set $s :=
        \app{u'_1}{u'_2}$ concluding this case since by contextual
        closure:
        \begin{equation*}
            \begin{array}{lll}
                \app{t_1}{t_2}                          &\bangArr_{S_\indexOmega}<s!>   &\app{u'_1}{t_2}
        \\[0.2cm]
                \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
        \\[0.2cm]
                \app{t_1}{u'_2}                         &\bangArr_{S_\indexOmega}<s!>   &\app{u'_1}{u'_2}
            \end{array}
        \end{equation*}

    \item[\bltII] $u_1 = \app{t_1}{u'_1}$, $u_2 = \app{u'_1}{t_2}$
        with $t_2 \bangArr_{S_\indexOmega}<s!> u'_1$ and $t_1
        \bangArr_{S_\indexOmega}<s!> u'_2$: We set $s :=
        \app{u'_1}{u'_2}$ concluding this case since by contextual
        closure:
        \begin{equation*}
            \begin{array}{lll}
                \app{t_1}{t_2}                          &\bangArr_{S_\indexOmega}<s!>   &\app{t_1}{u'_2}
        \\[0.2cm]
                \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr_{S_\indexOmega}<s!>
        \\[0.2cm]
                \app{u'_1}{t_2}                         &\bangArr_{S_\indexOmega}<s!>   &\app{u'_1}{u'_2}
            \end{array}
        \end{equation*}

    \item[\bltII] $u_1 = \app{t_1}{u'_1}$, $u_2 = \app{t_1}{u'_2}$
        with $t_2 \bangArr_{S_\indexOmega}<s!> u'_1$ and $t_2
        \bangArr_{S_\indexOmega}<s!> u'_2$: By \ih on $t_2$, there
        exists $s_2 \in \bangSetTerms$ such that $t_1
        \bangArr*_{S_\indexOmega}<s!> s_2$ and $t_2
        \bangArr*_{S_\indexOmega}<s!> s_2$. We set $s :=
        \app{t_1}{s_2}$ concluding this case since by contextual
        closure:
        \begin{equation*}
            \begin{array}{lll}
                \app{t_1}{t_2}                          &\bangArr_{S_\indexOmega}<s!>   &\app{t_1}{u'_1}
        \\[0.2cm]
                \;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\bangDownArr*_{S_\indexOmega}<s!>
        \\[0.2cm]
                \app{t_1}{u'_2}                         &\bangArr*_{S_\indexOmega}<s!>  &\app{t_1}{s'}
            \end{array}
        \end{equation*}
    \end{itemize}

\item[\bltI] $t = t_1\esub{x}{t_2}$: Notice that $t$ can be a
    $\bangSymbSubs$-redex but since $u_1
    \neq u_2$, three cases have to be distinguished:
    \begin{itemize}
    \item[\bltII] $t$ is the redex reduced in $t
        \bangArr_{S_\indexOmega}<s!> u_1$: Then $t_2 = \bangLCtxt<\oc
        t'_2>$ and $u_1 = \bangLCtxt<t_1\isub{x}{t'_2}>$. We
        distinguish two cases:
        \begin{itemize}
        \item[\bltIII] $u_2 = u'_1\esub{x}{t_2}$ and $t_1
            \bangArr_{S_\indexOmega}<s!> u'_1$: We set $s =
            \bangLCtxt<u'_1\isub{x}{t'_2}>$. By induction on $t_1$,
            one has that $t_1\isub{x}{t'_2}
            \bangArr_{S_\indexOmega}<s!> u'_1\isub{x}{t'_2}$ thus by
            contextual closure, one has that:
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{\bangLCtxt<\oc t'_2>}               &\bangArr_{S_\indexOmega}<s!>   &u'_1\esub{x}{\bangLCtxt<\oc t'_2>}
            \\[0.2cm]
                    \hspace{0.75cm}\bangDownArr_{S_\indexOmega}<s!> &                               &\hspace{0.75cm}\bangDownArr_{S_\indexOmega}<s!>
            \\[0.2cm]
                    \bangLCtxt<t_1\isub{x}{t'_2}>                   &\bangArr_{S_\indexOmega}<s!>   &\bangLCtxt<u'_1\isub{x}{t'_2}>
                \end{array}
            \end{equation*}
        \end{itemize}

        \item[\bltIII] $u_2 = t_1\esub{x}{u'_2}$ and $t_2
            \bangArr_{S_\indexOmega}<s!> u'_2$: Since $t_2 =
            \bangLCtxt<\oc t'_2>$, three cases can be distinguished:
            \begin{itemize}
            \item[\bltIV] $\bangLCtxt =
                \bangLCtxt_1<\bangLCtxt_3\esub{y}{\bangLCtxt_2<\oc
                t''_2>}>$ and $u'_2 =
                \bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3<\oc
                t'_2>\isub{y}{t''_2}>>$: We set $s' :=
                \bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t'_2}\bangCtxtPlug{t_1\isub{x}{t'_2\isub{y}{t''_2}}}>>$.
                By induction on $\bangLCtxt_3$, one has that
                $\bangLCtxt_3<t'_2>\isub{x}{t'_2} =
                \bangLCtxt_3\isub{x}{t'_2}\bangCtxtPlug{t_1\isub{x}{t'_2}}$.
                By \mbox{$\alpha$-conversion}, $y \notin
                \freeVar{t_1}$ and therefore, by induction on $t_1$,
                $t_1\isub{x}{t'_2}\isub{y}{t''_2} =
                t_1\isub{y}{t''_2}\isub{x}{t'_2\isub{y}{t''_2}}$ thus:
                \begin{equation*}
                    \begin{array}{lll}
                        t_1\esub{x}{\bangLCtxt_1<\bangLCtxt_3<\oc t'_2>\esub{y}{\bangLCtxt_2<\oc t''_2>}>}  &\bangArr_{S_\indexOmega}<s!>   &t_1\esub{x}{\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{y}{t''_2}\bangCtxtPlug{\oc t'_2\isub{y}{t''_2}}>>}
                \\[0.2cm]
                        \hspace{2cm}\bangDownArr_{S_\indexOmega}<s!>                                        &                               &\hspace{2cm}\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                        \bangLCtxt_1<\bangLCtxt_3<t_1\isub{x}{t'_2}>\esub{y}{\bangLCtxt_2<\oc t''_2>}>      &\bangArr_{S_\indexOmega}<s!>   &\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t'_2}\bangCtxtPlug{t_1\isub{x}{t'_2\isub{y}{t''_2}}}>>
                \\
                                                                                                            &                               &=\bangLCtxt_1<\bangLCtxt_2<\bangLCtxt_3\isub{x}{t'_2}\bangCtxtPlug{t_1\isub{y}{t''_2}\isub{x}{t'_2\isub{y}{t''_2}}}>>
                    \end{array}
                \end{equation*}

            \item[\bltIV] $u'_2 = \bangLCtxt'<\oc t'_2>$ and
                $\bangLCtxt \bangArr_{S_\indexOmega}<s!> \bangLCtxt'$:
                We set $s' := \bangLCtxt'<t_1\isub{x}{t'_2}>$ which
                concludes this case since using
                \Cref{lem:Bang_Full_s!_Context_Reduction_Lifted_to_Terms},
                one has:
                \begin{equation*}
                    \begin{array}{lll}
                        t_1\esub{x}{\bangLCtxt<\oc t'_2>}               &\bangArr_{S_\indexOmega}<s!>   &t_1\esub{x}{\bangLCtxt'<\oc t'_2>}
                \\[0.2cm]
                        \hspace{0.75cm}\bangDownArr_{S_\indexOmega}<s!> &                               &\hspace{0.75cm}\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                        \bangLCtxt<t_1\isub{x}{t'_2}>                   &\bangArr_{S_\indexOmega}<s!>   &\bangLCtxt'<t_1\isub{x}{t'_2}>
                    \end{array}
                \end{equation*}

            \item[\bltIV] $u'_2 = \bangLCtxt<\oc t''_2>$ and $t'_2
                \bangArr_{S_\indexOmega}<s!> t''_2$: We set $s' :=
                \bangLCtxt<t_1\isub{x}{t''_2}>$. By induction on
                $t_1$, one has that $t_1\isub{x}{t'_2}
                \bangArr*_{S_\indexOmega}<s!> t_1\isub{x}{t''_2}$
                thus:
                \begin{equation*}
                    \begin{array}{lll}
                        t_1\esub{x}{\bangLCtxt<\oc t'_2>}               &\bangArr_{S_\indexOmega}<s!>   &t_1\esub{x}{\bangLCtxt<\oc t''_2>}
                \\[0.2cm]
                        \hspace{0.75cm}\bangDownArr_{S_\indexOmega}<s!> &                               &\hspace{0.75cm}\bangDownArr_{S_\indexOmega}<s!>
                \\[0.2cm]
                        \bangLCtxt<t_1\isub{x}{t'_2}>                   &\bangArr*_{S_\indexOmega}<s!>  &\bangLCtxt<t_1\isub{x}{t''_2}>
                    \end{array}
                \end{equation*}
            \end{itemize}

    \item[\bltII] $t$ is the redex reduced in $t
        \bangArr_{S_\indexOmega}<s!> u_2$: Same as the previous case.

    \item[\bltII] $t$ is not the redex reduced in $t
        \bangArr_{S_\indexOmega}<s!> u_1$ nor $t
        \bangArr_{S_\indexOmega}<s!> u_2$: We distinguish four cases:
        \begin{itemize}
        \item[\bltIII] $u_1 = u'_1\esub{x}{t_2}$, $u_2 =
            u'_2\esub{x}{t_2}$ with $t_1 \bangArr_{S_\indexOmega}<s!>
            u'_1$ and $t_1 \bangArr_{S_\indexOmega}<s!> u'_2$: By \ih
            on $t_1$, there exists $s_1 \in \bangSetTerms$ such that
            $u'_1 \bangArr*_{S_\indexOmega}<s!> s_1$ and $u'_2
            \bangArr*_{S_\indexOmega}<s!> s_1$. We set $s :=
            s_1\esub{x}{t_2}$ concluding this case since by contextual
            closure:
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                            &\bangArr_{S_\indexOmega}<s!>   &u'_1\esub{x}{t_2}
            \\[0.2cm]
                    \;\;\;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\;\;\bangDownArr*_{S_\indexOmega}<s!>
            \\[0.2cm]
                    u'_2\esub{x}{t_2}                           &\bangArr*_{S_\indexOmega}<s!>  &s_1\esub{x}{t_2}
                \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = u'_1\esub{x}{t_2}$, $u_2 =
            t_1\esub{x}{u'_2}$ with $t_1 \bangArr_{S_\indexOmega}<s!>
            u'_1$ and $t_2 \bangArr_{S_\indexOmega}<s!> u'_2$: We set
            $s := u'_1\esub{x}{u'_2}$ concluding this case since by
            contextual closure:
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                            &\bangArr_{S_\indexOmega}<s!>   &u'_1\esub{x}{t_2}
            \\[0.2cm]
                    \;\;\;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\;\;\bangDownArr_{S_\indexOmega}<s!>
            \\[0.2cm]
                    t_1\esub{x}{u'_2}                           &\bangArr_{S_\indexOmega}<s!>   &u'_1\esub{x}{u'_2}
                \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = t_1\esub{x}{u'_1}$, $u_2 =
            u'_1\app{x}{t_2}$ with $t_2 \bangArr_{S_\indexOmega}<s!>
            u'_1$ and $t_1 \bangArr_{S_\indexOmega}<s!> u'_2$: We set
            $s := u'_1\esub{x}{u'_2}$ concluding this case since by
            contextual closure:
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                            &\bangArr_{S_\indexOmega}<s!>   &t_1\esub{x}{u'_2}
            \\[0.2cm]
                    \;\;\;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\;\;\bangDownArr_{S_\indexOmega}<s!>
            \\[0.2cm]
                    u'_1\esub{x}{t_2}                           &\bangArr_{S_\indexOmega}<s!>   &u'_1\esub{x}{u'_2}
                \end{array}
            \end{equation*}

        \item[\bltIII] $u_1 = t_1\esub{x}{u'_1}$, $u_2 =
            t_1\esub{x}{u'_2}$ with $t_2 \bangArr_{S_\indexOmega}<s!>
            u'_1$ and $t_2 \bangArr_{S_\indexOmega}<s!> u'_2$: By \ih
            on $t_2$, there exists $s_2 \in \bangSetTerms$ such that
            $t_1 \bangArr*_{S_\indexOmega}<s!> s_2$ and $t_2
            \bangArr*_{S_\indexOmega}<s!> s_2$. We set $s :=
            t_1\esub{x}{s_2}$ concluding this case since by contextual
            closure:
            \begin{equation*}
                \begin{array}{lll}
                    t_1\esub{x}{t_2}                            &\bangArr_{S_\indexOmega}<s!>   &t_1\esub{x}{u'_1}
            \\[0.2cm]
                    \;\;\;\;\bangDownArr_{S_\indexOmega}<s!>    &                               &\;\;\;\;\bangDownArr*_{S_\indexOmega}<s!>
            \\[0.2cm]
                    t_1\esub{x}{u'_2}                           &\bangArr*_{S_\indexOmega}<s!>  &t_1\esub{x}{s'}
                \end{array}
            \end{equation*}
        \end{itemize}
    \end{itemize}

\item[\bltI] $t = \der{t'}$: Since $t$ cannot be a
    $\bangSymbSubs$-redex, then necessarily
    $u_1 = \der{t'_1}$ and $u_2 = \der{t'_2}$ with $t'
    \bangArr_{S_\indexOmega}<s!> t'_1$ and $t'
    \bangArr_{S_\indexOmega}<s!> t'_2$. By \ih on $t'$, there exists
    $s' \in \bangSetTerms$ such that $t_1
    \bangArr*_{S_\indexOmega}<s!> s'$ and $t_2
    \bangArr*_{S_\indexOmega}<s!> s'$. We set $s := \der{s'}$
    concluding this case since by contextual closure:
    \begin{equation*}
        \begin{array}{lll}
            \der{t'}                                &\bangArr_{S_\indexOmega}<s!>   &\der{t'_1}
    \\[0.2cm]
            \;\;\;\bangDownArr_{S_\indexOmega}<s!>  &                               &\;\;\;\bangDownArr*_{S_\indexOmega}<s!>
    \\[0.2cm]
            \der{t'_2}                              &\bangArr*_{S_\indexOmega}<s!>  &\der{s'}
        \end{array}
    \end{equation*}

\item[\bltI] $t = \oc t'$: Since $t$ cannot be a
    $\bangSymbSubs$-redex, then necessarily
    $u_1 = \oc t'_1$ and $u_2 = \oc t'_2$ with $t'
    \bangArr_{S_\indexOmega}<s!> t'_1$ and $t'
    \bangArr_{S_\indexOmega}<s!> t'_2$. By \ih on $t'$, there exists
    $s' \in \bangSetTerms$ such that $t_1
    \bangArr*_{S_\indexOmega}<s!> s'$ and $t_2
    \bangArr*_{S_\indexOmega}<s!> s'$. We set $s := \oc s'$ concluding
    this case since by contextual closure:
    \begin{equation*}
        \begin{array}{lll}
            \oc t'                              &\bangArr_{S_\indexOmega}<s!>   &\oc t'_1
    \\[0.2cm]
            \bangDownArr_{S_\indexOmega}<s!>    &                               &\bangDownArr*_{S_\indexOmega}<s!>
    \\[0.2cm]
            \oc t'_2                            &\bangArr*_{S_\indexOmega}<s!>  &\oc s'
        \end{array}
    \end{equation*}
\end{itemize}
\end{proof}


==> 2_Proofs/Bang_Full_s__Terminating.tex <==
\begin{proof}
Let $t \in \bangSetTerms$. As the finite multisets over natural
numbers is well-ordered by $\prec$, we can proceed by induction on
$\multiSize{t}$. If $t$ is a $\bangSymbSubs$-normal form, then it is
trivially terminating. Otherwise, $t \bangArr_{S_\indexOmega}<s!> u$,
then $\multiSize{t} \succ \multiSize{u}$
(\Cref{lem:Bang_Full_MultiSize_decreases_Substitution}), and so $u$ is
strongly $\bangSymbSubs$-normalizing, by the \ih\ Therefore, $t$ is
strongly $\bangSymbSubs$-normalizing.
\end{proof}


==> 2_Proofs/Bang_Term_Size_with_Context.tex <==
\begin{proof}
Let $\bangStratCtxt_\indexOmega$ be a context and $t \in
\bangSetTerms$ be a term. By induction on
$\bangStratCtxt_\indexOmega$:
\begin{itemize}
\item[\bltI] $\bangStratCtxt_\indexOmega = \Hole$: Then
    $\termSize{\bangStratCtxt_\indexOmega<t>} = \termSize{t} = 0 +
    \termSize{t} = \termSize{\cdelia{\bangStratCtxt}{\bangStratCtxt_\indexOmega}} + \termSize{t}$.

\item[\bltI] $\bangStratCtxt_\indexOmega =
    \abs{x}{\bangStratCtxt'_\indexOmega}$: By \ih on
    $\bangStratCtxt'_\indexOmega$, one has that
    $\termSize{\bangStratCtxt'_\indexOmega<t>} =
    \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}$ thus:
    \begin{equation*}
        \termSize{\bangStratCtxt_\indexOmega<t>}
        = \termSize{\abs{x}{\bangStratCtxt'_\indexOmega<t>}}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega<t>}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}
        = \termSize{\abs{x}{\bangStratCtxt'_\indexOmega}} + \termSize{t}
        = \termSize{\bangStratCtxt_\indexOmega} + \termSize{t}
    \end{equation*}

\item[\bltI] $\bangStratCtxt_\indexOmega =
    \app{\bangStratCtxt'_\indexOmega}{u}$: By \ih on
    $\bangStratCtxt'_\indexOmega$, one has that
    $\termSize{\bangStratCtxt'_\indexOmega<t>} =
    \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}$ thus:
    \begin{equation*}
        \termSize{\bangStratCtxt_\indexOmega<t>}
        = \termSize{\app{\bangStratCtxt'_\indexOmega<t>}{u}}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega<t>} + \termSize{u}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t} + \termSize{u}
        = \termSize{\app{\bangStratCtxt'_\indexOmega}{u}} + \termSize{t}
        = \termSize{\bangStratCtxt_\indexOmega} + \termSize{t}
    \end{equation*}

\item[\bltI] $\bangStratCtxt_\indexOmega =
    \app[\,]{u}{\bangStratCtxt'_\indexOmega}$: By \ih on
    $\bangStratCtxt'_\indexOmega$, one has that
    $\termSize{\bangStratCtxt'_\indexOmega<t>} =
    \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}$ thus:
    \begin{equation*}
        \termSize{\bangStratCtxt_\indexOmega<t>}
        = \termSize{\app[\,]{u}{\bangStratCtxt'_\indexOmega<t>}}
        = 1 + \termSize{u} + \termSize{\bangStratCtxt'_\indexOmega<t>}
        = 1 + \termSize{u} + \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}
        = \termSize{\app[\,]{u}{\bangStratCtxt'_\indexOmega}} + \termSize{t}
        = \termSize{\bangStratCtxt_\indexOmega} + \termSize{t}
    \end{equation*}

\item[\bltI] $\bangStratCtxt_\indexOmega =
    \bangStratCtxt'_\indexOmega\esub{x}{u}$: By \ih on
    $\bangStratCtxt'_\indexOmega$, one has that
    $\termSize{\bangStratCtxt'_\indexOmega<t>} =
    \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}$ thus:
    \begin{equation*}
        \termSize{\bangStratCtxt_\indexOmega<t>}
        = \termSize{\bangStratCtxt'_\indexOmega<t>\esub{x}{u}}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega<t>} + \termSize{u}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t} + \termSize{u}
        = \termSize{\bangStratCtxt'_\indexOmega\esub{x}{u}} + \termSize{t}
        = \termSize{\bangStratCtxt_\indexOmega} + \termSize{t}
    \end{equation*}

\item[\bltI] $\bangStratCtxt_\indexOmega =
    u\esub{x}{\bangStratCtxt'_\indexOmega}$: By \ih on
    $\bangStratCtxt'_\indexOmega$, one has that
    $\termSize{\bangStratCtxt'_\indexOmega<t>} =
    \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}$ thus:
    \begin{equation*}
        \termSize{\bangStratCtxt_\indexOmega<t>}
        = \termSize{u\esub{x}{\bangStratCtxt'_\indexOmega<t>}}
        = 1 + \termSize{u} + \termSize{\bangStratCtxt'_\indexOmega<t>}
        = 1 + \termSize{u} + \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}
        = \termSize{u\esub{x}{\bangStratCtxt'_\indexOmega}} + \termSize{t}
        = \termSize{\bangStratCtxt_\indexOmega} + \termSize{t}
    \end{equation*}

\item[\bltI] $\bangStratCtxt_\indexOmega =
    \der{\bangStratCtxt'_\indexOmega}$: By \ih on
    $\bangStratCtxt'_\indexOmega$, one has that
    $\termSize{\bangStratCtxt'_\indexOmega<t>} =
    \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}$ thus:
    \begin{equation*}
        \termSize{\bangStratCtxt_\indexOmega<t>}
        = \termSize{\der{\bangStratCtxt'_\indexOmega<t>}}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega<t>}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}
        = \termSize{\der{\bangStratCtxt'_\indexOmega}} + \termSize{t}
        = \termSize{\bangStratCtxt_\indexOmega} + \termSize{t}
    \end{equation*}

\item[\bltI] $\bangStratCtxt_\indexOmega = \oc
    \bangStratCtxt'_\indexOmega$: By \ih on
    $\bangStratCtxt'_\indexOmega$, one has that
    $\termSize{\bangStratCtxt'_\indexOmega<t>} =
    \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}$ thus:
    \begin{equation*}
        \termSize{\bangStratCtxt_\indexOmega<t>}
        = \termSize{\oc \bangStratCtxt'_\indexOmega<t>}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega<t>}
        = 1 + \termSize{\bangStratCtxt'_\indexOmega} + \termSize{t}
        = \termSize{\oc \bangStratCtxt'_\indexOmega} + \termSize{t}
        = \termSize{\bangStratCtxt_\indexOmega} + \termSize{t}
    \end{equation*}
\end{itemize}
\end{proof}


==> 3_Proofs/BangAGKMean_Merging_Type_Derivations.tex <==
\begin{proof}
Let $(\Pi_i \bangAGKMeanTr \Gamma_i \vdash \oc t : \M_i)_{\iI}$ such
that $\bangBKRVInhPred{+_{i \in I} \Gamma_i}$. For each $i \in I$, $\Pi$
has the following form:
\begin{equation*}
    \begin{prooftree}
        \hypo{\Pi_i^j \bangAGKMeanTr \Gamma_i^j \vdash t : \sigma_i^j}
        \delims{\left(}{\right)_{j \in J_i}}
        \inferBangAGKMeanInh{+_{j \in J_i} \Gamma_i^j}
        \inferBangAGKMeanBg{+_{j \in J_i} \Gamma_i^j &\vdash \oc t : \mset{\sigma_i^j}_{j \in J_i}}
    \end{prooftree}
\end{equation*}
with $\Gamma_i = +_{j \in J_i} \Gamma_i^j$ and $\M_i =
\mset{\sigma_i^j}_{j \in J_i}$. By hypothesis $\bangBKRVInhPred{+_{i \in
I} \Gamma_i}$ thus $\bangBKRVInhPred{+_{j \in J_i, i \in I} \Gamma_i^j}$
and we let $\Pi$ be the following derivation:
\begin{equation*}
    \begin{prooftree}
        \hypo{\Pi_i^j \bangAGKMeanTr \Gamma_i^j \vdash t : \sigma_i^j}
        \delims{\left(}{\right)_{j \in J_i, i \in I}}
        \inferBangAGKMeanInh{+_{j \in J_i, i \in I} \Gamma_i^j}
        \inferBangAGKMeanBg{+_{j \in J_i, i \in I} \Gamma_i^j &\vdash \oc t : \mset{\sigma_i^j}_{j \in J_i, i \in I}}
    \end{prooftree}
\end{equation*}
\end{proof}


==> 3_Proofs/BangAGKMean_Reverse_Substitution.tex <==
\begin{proof}
Let $\Pi \bangAGKMeanTr \Gamma \vdash t\isub{x}{u} : \sigma$. We
reason by induction on $t$.
\begin{itemize}
\item[\bltI] $t = y$: We distinguish two cases:
    \begin{itemize}
    \item[\bltII] $y = x$: Then $t\isub{x}{u} = u$ and $\Pi
        \bangAGKMeanTr \Gamma \vdash u : \sigma$. Using
        \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(Gam)_and_inh(sig)},
        one has that $\bangBKRVInhPred{\Gamma}$ and
        $\bangBKRVInhPred{\bangArgs{\sigma}}$. By
        \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(sigma)}, one
        deduces that $\bangBKRVInhPred{\sigma}$ so that
        $\bangBKRVInhPred{\mset{\sigma}}$ also holds. We set $\M =
        \mset{\sigma}$, $\Gamma_1:=\emptyset $ and $\Gamma_2:=
        \Gamma$, so that $\Gamma = \Gamma_1 + \Gamma_2$. Then we set
        $\Pi_1$ and $\Pi_2$ as follows:
        \begin{equation*}
            \Pi_1 := \begin{prooftree}
                \inferBangAGKMeanInh{\mset{\sigma}}
                \inferBangAGKMeanInh{\bangArgs{\sigma}}
                \inferBangAGKMeanVar{x : \mset{\sigma} \vdash x : \sigma}
            \end{prooftree}
            \hspace{1.5cm}
            \Pi_2 := \begin{prooftree}
                \hypo{\Pi \bangAGKMeanTr \Gamma \vdash u : \sigma}
                \inferBangAGKMeanInh{\Gamma}
                \inferBangAGKMeanBg{\Gamma \vdash \oc u : \mset{\sigma}}
            \end{prooftree}
        \end{equation*}

      \item[\bltII] $y \neq x$: Then $t\isub{x}{u} = y = t$ and
        $\Gamma = y:\mset{\sigma}$. We set $\M := \emptymset$,
        $\Gamma_1 := \Gamma$, and $\Gamma_2:= \emptyset$, so that in
        particular $\Gamma_1 ; x:\emptymset = \Gamma_1$ and $\Gamma =
        \Gamma_1 + \Gamma_2$. We can then set $\Pi_1 := \Pi$ and
        $\Pi_2$ as follows:
        \begin{equation*}
            \begin{prooftree}
                \inferBangAGKMeanInh{\emptyset}
                \inferBangAGKMeanBg[1]{\emptyset \vdash \oc u : \emptymset}
            \end{prooftree}
        \end{equation*}
    \end{itemize}

\item[\bltI] $t = \abs{y}{t'}$: Then $t\isub{x}{u} =
    \abs{y}{(t'\isub{x}{u})}$ and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi \bangAGKMeanTr \Gamma; y : \N \vdash t'\isub{x}{u} : \sigma}
            \inferBangAGKMeanAbs{\Gamma \vdash \abs{y}{(t'\isub{x}{u})} : \N \typeArrow \sigma}
        \end{prooftree}
    \end{equation*}
    By \ih on $t'$, one obtains $\Pi'_1 \bangAGKMeanTr \Gamma'_1; x :
    \M \vdash t' : \sigma$ and $\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash
    \oc u : \M$ such that $\Gamma; y : \N = \Gamma'_1 + \Gamma_2$. By
    $\alpha$-conversion $y \notin \typeCtxtDom{\Gamma_2}$ so that
    $\Gamma'_1 = \Gamma_1; y : \N$ for some type context $\Gamma_1$.
    Finally, by $\alpha$-conversion, one has that $x \neq y$ thus
    $(\Gamma_1; y : \N); x : \M = (\Gamma_1; x : \M); y : \N$. We set
    $\Pi_1$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_1 \bangAGKMeanTr (\Gamma_1; x : \M); y : \N \vdash t' : \sigma}
            \inferBangAGKMeanAbs{\Gamma_1; x : \M \vdash \abs{y}{t'} : \N \typeArrow \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $t = \app{t_1}{t_2}$: Then $t\isub{x}{u} =
    \app{(t_1\isub{x}{u})}{(t_2\isub{x}{u})}$ and $\Pi$ has the
    following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1 \bangAGKMeanTr \Gamma_1 \vdash t_1\isub{x}{u} : \N \typeArrow \sigma}
            \hypo{\Phi_2 \bangAGKMeanTr \Gamma_2 \vdash t_2\isub{x}{u} : \N}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{(t_1\isub{x}{u})}{(t_2\isub{x}{u})} : \sigma}
        \end{prooftree}
    \end{equation*}
    where $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $t_1$ and $t_2$,
    one obtains $\Phi_1^1 \bangAGKMeanTr \Gamma_1^1; x : \M_1 \vdash
    t_1 : \N \typeArrow \sigma$ and $\Phi_2^1 \bangAGKMeanTr
    \Gamma_2^1; x : \M_2 \vdash t_2 : \N$, $\Phi_1^2 \bangAGKMeanTr
    \Gamma_1^2 \vdash \oc u : \M_1$ and $\Phi_2^2 \bangAGKMeanTr
    \Gamma_2^2 \vdash \oc u : \M_2$ such that $\Gamma_1 = \Gamma_1^1 +
    \Gamma_1^2$ and $\Gamma_2 = \Gamma_2^1 + \Gamma_2^2$. Since
    $\bangBKRVInhPred{\Gamma_1 + \Gamma_2}$ then
    $\bangBKRVInhPred{\Gamma_1^1 + \Gamma_2^1}$ and
    $\bangBKRVInhPred{\Gamma_1^2 + \Gamma_2^2}$. Using
    \Cref{lem:BangAGKMean_Merging_Type_Derivations}, one obtains
    $\Pi_2 \bangAGKMeanTr \Gamma_1^2 + \Gamma_2^2 \vdash \oc u : \M_1
    \uplus \M_2$. Moreover, using
    \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(sigma)}, one deduces
    that $\bangBKRVInhPred{\M_1 \uplus \M_2}$. Therefore
    $\bangBKRVInhPred{(\Gamma_1^1 + \Gamma_2^1); x : \M_1 \uplus
    \M_2}$. We set $\Pi_1$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1^1 \bangAGKMeanTr \Gamma_1^1; x : \M_1 \vdash t_1 : \N \typeArrow \sigma}
            \hypo{\Phi_2^1 \bangAGKMeanTr \Gamma_2^1; x : \M_2 \vdash t_2 : \N}
            \inferBangAGKMeanInh{(\Gamma_1^1 + \Gamma_2^1); x : \M_1 \uplus \M_2}
            \inferBangAGKMeanApp{(\Gamma_1^1 + \Gamma_2^1); x : \M_1 \uplus \M_2 \vdash \app{t_1}{t_2} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $t = t_1\esub{y}{t_2}$: Then $t\isub{x}{u} =
    t_1\isub{x}{u}\esub{y}{t_2\isub{x}{u}}$ and $\Pi$ has the
    following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1 \bangAGKMeanTr \Gamma_1; y : \N \vdash t_1\isub{x}{u} : \sigma}
            \hypo{\Phi_2 \bangAGKMeanTr \Gamma_2 \vdash t_2\isub{x}{u} : \N}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash t_1\isub{x}{u}\esub{y}{t_2\isub{x}{u}} : \sigma}
        \end{prooftree}
    \end{equation*}
    where $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $t_1$ and $t_2$,
    one obtains $\Phi_1^1 \bangAGKMeanTr \Gamma_1^1; x : \M_1 \vdash
    t_1 : \sigma$ and $\Phi_2^1 \bangAGKMeanTr \Gamma_2^1; x : \M_2
    \vdash t_2 : \N$, $\Phi_1^2 \bangAGKMeanTr \Gamma_1^2 \vdash \oc u
    : \M_1$ and $\Phi_2^2 \bangAGKMeanTr \Gamma_2^2 \vdash \oc u :
    \M_2$ such that $\Gamma_1; y : \N = \Gamma_1^1 + \Gamma_1^2$ and
    $\Gamma_2 = \Gamma_2^1 + \Gamma_2^2$. By $\alpha$-conversion, $y
    \notin \freeVar{u}$ so that $\Gamma_1^1 = \Delta_1^1; y : \N$ and
    $\Gamma_1 = \Delta_1^1 + \Gamma_1^2$. Since
    $\bangBKRVInhPred{\Gamma_1 + \Gamma_2}$ then
    $\bangBKRVInhPred{\Delta_1^1 + \Gamma_2^1}$ and
    $\bangBKRVInhPred{\Gamma_1^2 + \Gamma_2^2}$. Using
    \Cref{lem:BangAGKMean_Merging_Type_Derivations}, one obtains
    $\Pi_2 \bangAGKMeanTr \Gamma_1^2 + \Gamma_2^2 \vdash \oc u : \M_1
    \uplus \M_2$. Moreover, using
    \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(sigma)}, one deduces
    that $\bangBKRVInhPred{\M_1 \uplus \M_2}$ thus
    $\bangBKRVInhPred{(\Delta_1^1 + \Gamma_2^1); x : \M_1 \uplus
    \M_2}$. We set $\Pi_1$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1^1 \bangAGKMeanTr (\Delta_1^1; x : \M_1); y : \N \vdash t_1 : \sigma}
            \hypo{\Phi_2^1 \bangAGKMeanTr \Gamma_2^1; x : \M_2 \vdash t_2 : \N}
            \inferBangAGKMeanInh{(\Delta_1^1 + \Gamma_2^1); x : \M_1 \uplus \M_2}
            \inferBangAGKMeanEs{(\Delta_1^1 + \Gamma_2^1); x : \M_1 \uplus \M_2 \vdash t_1\esub{y}{t_2} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $t = \oc t'$: Then $t\isub{x}{u} = \oc (t'\isub{x}{u})$
    and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_i \bangAGKMeanTr \Gamma_i \vdash t'\isub{x}{u} : \sigma_i}
            \delims{\left(}{\right)_{i \in I}}
            \inferBangAGKMeanInh{+_{i \in I} \Gamma_i}
            \inferBangAGKMeanBg{+_{i \in I} \Gamma_i \vdash \oc (t'\isub{x}{u}) : \mset{\sigma_i}_{i \in I}}
        \end{prooftree}
    \end{equation*}
    For each $i \in I$, by \ih on $t'$, one obtains $\Phi_i^1
    \bangAGKMeanTr \Gamma_i^1; x : \M_i \vdash t' : \sigma_i$ and
    $\Phi_i^2 \bangAGKMeanTr \Gamma_i^2 \vdash \oc u : \M_i$ such that
    $\Gamma_i = \Gamma_i^1 + \Gamma_i^2$. Since $\bangBKRVInhPred{+_{i
    \in I} \Gamma_i}$ then $\bangBKRVInhPred{+_{i \in I} \Gamma_i^1}$
    and $\bangBKRVInhPred{+_{i \in I} \Gamma_i^2}$. Using
    \Cref{lem:BangAGKMean_Merging_Type_Derivations}, one obtains
    $\Pi_2 \bangAGKMeanTr +_{i \in I} \Gamma_i^2 \vdash \oc u :
    \uplus_{i \in I} \M_i$. Moreover, using
    \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(sigma)}, one deduces
    that $\bangBKRVInhPred{\uplus_{i \in I} \M_i}$ thus
    $\bangBKRVInhPred{+_{i \in I} \Gamma_i^1; x : \uplus_{i \in I}
    \M_i}$. We set $\Gamma_1 = +_{\iI} \Gamma_i^1$. Then we conclude
    with $\Pi_1$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_i^1 \bangAGKMeanTr \Gamma_i^1; x : \M_i \vdash t' : \sigma_i}
            \delims{\left(}{\right)_{i \in I}}
            \inferBangAGKMeanInh{+_{i \in I} \Gamma_i^1; x : \uplus_{i \in I} \M_i}
            \inferBangAGKMeanBg{+_{i \in I} \Gamma_i^1; x : \uplus_{i \in I} \M_i \vdash \oc t' : \mset{\sigma_i}_{i \in I}}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $t = \der{t'}$: Then $t\isub{x}{u} = \der{t'\isub{x}{u}}$
    and $\Pi$ has the followig form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi \bangAGKMeanTr \Gamma \vdash t'\isub{x}{u} : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma \vdash \der{t'\isub{x}{u}} : \sigma}
        \end{prooftree}
    \end{equation*}
    By \ih on $t'$, one obtains $\Phi_1 \bangAGKMeanTr \Gamma_1; x :
    \M \vdash t' : \mset{\sigma}$ and $\Pi_2 \bangAGKMeanTr \Gamma_2
    \vdash \oc u : \M$ such that $\Gamma = \Gamma_1 + \Gamma_2$. We
    set $\Pi_1$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi \bangAGKMeanTr \Gamma_1; x : \M \vdash t' : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma_1; x : \M \vdash \der{t'} : \sigma}
        \end{prooftree}
    \end{equation*}
\end{itemize}
\end{proof}


==> 3_Proofs/BangAGKMean_Splitting.tex <==
\begin{proof}
Let $\Pi \bangAGKMeanTr \Gamma \vdash \oc t : \M$ such that $\M =
\uplus_{i \in I} \N_i$. Then $\Pi$ is necessarily of the following
form:
\begin{equation*}
    \begin{prooftree}
        \hypo{\Phi_j \bangAGKMeanTr \Delta_j \vdash t : \sigma_j}
        \delims{\left(}{\right)_{j \in J}}
        \inferBangAGKMeanInh{+_{j \in J} \Delta_j}
        \inferBangAGKMeanBg{+_{j \in J} \Delta_j &\vdash \oc t : \mset{\sigma_j}_{j \in J}}
    \end{prooftree}
\end{equation*}
where $\Gamma = +_{j \in J} \Delta_j$ and $\M = \mset{\sigma_j}_{j \in
J}$. Since $\M = \uplus_{i \in I} \N_i$, then there exists $(J_i)_{i
\in I} \subset \nat$ such that $\mset{\sigma_j}_{j \in J_i} = \N_i$.
Since $\bangBKRVInhPred{+_{i \in I} \Delta_i}$ then in particular
$\bangBKRVInhPred{+_{i \in J_i} \Delta_i}$. We set $\Gamma_i = +_{j
\in J_i} \Delta_j$ and $\Pi_i$ as the following derivation:
\begin{equation*}
    \begin{prooftree}
        \hypo{\Phi_j \bangAGKMeanTr \Delta_j \vdash t : \sigma_j}
        \delims{\left(}{\right)_{j \in J_i}}
        \inferBangAGKMeanInh{+_{j \in J_i} \Delta_j}
        \inferBangAGKMeanBg{+_{j \in J_i} \Delta_j &\vdash \oc t : \mset{\sigma_j}_{j \in J_i}}
    \end{prooftree}
\end{equation*}
which concludes this case since $\Gamma_i = +_{j \in J_i} \Delta_j$
and $\mset{\sigma_j}_{j \in J_i} = \N_i$
\end{proof}

==> 3_Proofs/BangAGKMean_Substitution.tex <==
\begin{proof}
Let $\Pi \bangAGKMeanTr \Gamma \vdash t\isub{x}{u} : \sigma$. We
reason by induction on $t$.
\begin{itemize}
\item[\bltI] $t = y$: We distinguish two cases:
    \begin{itemize}
    \item[\bltII] $y = x$: Then $t\isub{x}{u} = u$ and $\Pi_1$ and
        $\Pi_2$ have the following form:
        \begin{equation*}
            \Pi_1 := \begin{prooftree}
                \inferBangAGKMeanInh{\mset{\sigma}}
                \inferBangAGKMeanInh{\bangArgs{\sigma}}
                \inferBangAGKMeanVar{x : \mset{\sigma} \vdash x : \sigma}
            \end{prooftree}
            \hspace{1.5cm}
            \Pi_2 := \begin{prooftree}
                \hypo{\Pi' \bangAGKMeanTr \Gamma_2 \vdash u : \sigma}
                \inferBangAGKMeanInh{\Gamma}
                \inferBangAGKMeanBg{\Gamma_2 \vdash \oc u : \mset{\sigma}}
            \end{prooftree}
        \end{equation*}
        with $\Gamma_1 = \emptyset$ and $\M = \mset{\sigma}$. We set
        $\Pi := \Pi'$ concluding this case since $\Gamma_1 + \Gamma_2
        = \emptyset + \Gamma_2 = \Gamma_2$.

      \item[\bltII] $y \neq x$: Then $t\isub{x}{u} = y$ and $\Pi_1$
        and $\Pi_2$ has the following form:
        \begin{equation*}
            \Pi_1 := \begin{prooftree}
                \inferBangAGKMeanInh{\mset{\sigma}}
                \inferBangAGKMeanInh{\bangArgs{\sigma}}
                \inferBangAGKMeanVar{y : \mset{\sigma} \vdash y : \sigma}
            \end{prooftree}
            \hspace{1.5cm}
            \Pi_2 := \begin{prooftree}
                \inferBangAGKMeanInh{\emptyset}
                \inferBangAGKMeanBg[1]{\emptyset \vdash \oc u : \emptymset}
            \end{prooftree}
        \end{equation*}
        with $\Gamma = y : \mset{\sigma}$, $\Gamma_2 = \emptyset$ and
        $\M = \emptymset$. We set $\Pi := \Pi_1$ which concludes this
        case since $\Gamma_1 + \Gamma_2 = (y : \mset{\sigma}) +
        \emptyset = y : \mset{\sigma}$.
    \end{itemize}

\item[\bltI] $t = \abs{y}{t'}$: Then $t\isub{x}{u} =
    \abs{y}{(t'\isub{x}{u})}$ and $\Pi_1$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1 \bangAGKMeanTr (\Gamma_1; x : \M); y : \N \vdash t' : \tau}
            \inferBangAGKMeanAbs{\Gamma_1; x : \M \vdash \abs{y}{t'} : \N \typeArrow \tau}
        \end{prooftree}
    \end{equation*}
    with $\sigma = \N \typeArrow \tau$. By $\alpha$-conversion, $x
    \neq y$ thus $(\Gamma_1; x : \M); y : \N = (\Gamma_1; y : \N); x :
    \M$. By \ih on $t'$, one obtains $\Phi'_1 \bangAGKMeanTr
    (\Gamma_1; y : \N) + \Gamma_2 \vdash t'\isub{x}{y} : \tau$. By
    $\alpha$-conversion again, one has that $y \notin \freeVar{u}$ so
    that $(\Gamma_1; y : \N) + \Gamma_2 = (\Gamma_1 + \Gamma_2); y :
    \N$. We set $\Pi$ as the following derivation:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi'_1 \bangAGKMeanTr (\Gamma_1 + \Gamma_2); y : \N \vdash t'\isub{x}{y} : \tau}
            \inferBangAGKMeanAbs{\Gamma_1 + \Gamma_2 \vdash \abs{y}{(t'\isub{x}{u})} : \N \typeArrow \tau}
        \end{prooftree}
    \end{equation*}
    which concludes this case since $\sigma = \N \typeArrow \tau$.

\item[\bltI] $t = \app{t_1}{t_2}$: Then $t\isub{x}{u} =
    \app{(t_1\isub{x}{u})}{(t_2\isub{x}{u})}$ and $\Pi$ has the
    following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1 \bangAGKMeanTr \Delta_1 \vdash t_1 : \N \typeArrow \sigma}
            \hypo{\Phi_2 \bangAGKMeanTr \Delta_2 \vdash t_2 : \N}
            \inferBangAGKMeanInh{\Delta_1 + \Delta_2}
            \inferBangAGKMeanApp{\Delta_1 + \Delta_2 \vdash \app{t_1}{t_2} : \sigma}
        \end{prooftree}
    \end{equation*}
    with $\Gamma_1; x : \M = \Delta_1 + \Delta_2$. Let $\Delta_1 =
    \Gamma_1^1; x : \M_1$, $\Delta_2 = \Gamma_1^2; x : \M_2$ and
    $\Gamma_1 = \Gamma_1^1 + \Gamma_1^2$ for some contexts
    $\Gamma_1^1, \Gamma_1^2$ and some multitypes $\M_1, \M_2$. Using
    \victorTodo[Splitting Lemma], there exists $\Pi_2^1 \bangAGKMeanTr
    \Gamma_2^1 \vdash u : \M_1$ and $\Pi_2^2 \bangAGKMeanTr \Gamma_2^2
    \vdash u : \M_2$ such that $\Gamma_2^1 + \Gamma_2^2 = \Gamma_2$.
    By \ih on $t_1$ and $t_2$, there exist $\Phi'_1 \bangAGKMeanTr
    \Gamma_1^1 + \Gamma_2^1 \vdash t_1\isub{x}{u} : \N \typeArrow
    \sigma$ and $\Phi'_2 \bangAGKMeanTr \Gamma_1^2 + \Gamma_2^2 \vdash
    t_2\isub{x}{u} : \N$. Since $\bangBKRVInhPred{\Gamma_1}$ then
    $\bangBKRVInhPred{\Gamma_1^1 + \Gamma_1^2}$. Moreover, from
    $\Pi_2$ and
    \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(Gam)_and_inh(sig)},
    one deduces that $\bangBKRVInhPred{\Gamma_2^1 + \Gamma_2^2}$ so
    that $\bangBKRVInhPred{\Gamma_1^1 + \Gamma_2^1 + \Gamma_1^2 +
    \Gamma_2^2}$. We set $\Pi$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi'_1 \bangAGKMeanTr \Gamma_1^1 + \Gamma_2^1 \vdash t_1\isub{x}{u} : \N \typeArrow \sigma}
            \hypo{\Phi'_2 \bangAGKMeanTr \Gamma_1^2 + \Gamma_2^2 \vdash t_2\isub{x}{u} : \N}
            \inferBangAGKMeanInh{\Gamma_1^1 + \Gamma_2^1 + \Gamma_1^2 + \Gamma_2^2}
            \inferBangAGKMeanApp{\Gamma_1^1 + \Gamma_2^1 + \Gamma_1^2 + \Gamma_2^2 \vdash \app{(t_1\isub{x}{u})}{(t_2\isub{x}{u})} : \sigma}
        \end{prooftree}
    \end{equation*}
    which concludes this case since $\Gamma_1 + \Gamma_2 = (\Gamma_1^1
    + \Gamma_1^2) + (\Gamma_2^1 + \Gamma_2^2) = \Gamma_1^1 +
    \Gamma_2^1 + \Gamma_1^2 + \Gamma_2^2$.

\item[\bltI] $t = t_1\esub{y}{t_2}$: Then $t\isub{x}{u} =
    t_1\isub{x}{u}\esub{y}{t_2\isub{x}{u}}$ and $\Pi$ has the
    following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1 \bangAGKMeanTr \Delta_1; y : \N \vdash t_1 : \sigma}
            \hypo{\Phi_2 \bangAGKMeanTr \Delta_2 \vdash t_2 : \N}
            \inferBangAGKMeanInh{\Delta_1 + \Delta_2}
            \inferBangAGKMeanEs{\Delta_1 + \Delta_2 \vdash t_1\esub{y}{t_2} : \sigma}
        \end{prooftree}
    \end{equation*}
    with $\Gamma_1; x : \M = \Delta_1 + \Delta_2$. Let $\Delta_1 =
    \Gamma_1^1; x : \M_1$, $\Delta_2 = \Gamma_1^2; x : \M_2$ and
    $\Gamma_1 = \Gamma_1^1 + \Gamma_1^2$ for some contexts
    $\Gamma_1^1, \Gamma_1^2$ and some multitypes $\M_1, \M_2$. Using
    \victorTodo[Splitting Lemma], there exists $\Pi_2^1 \bangAGKMeanTr
    \Gamma_2^1 \vdash u : \M_1$ and $\Pi_2^2 \bangAGKMeanTr \Gamma_2^2
    \vdash u : \M_2$ such that $\Gamma_2^1 + \Gamma_2^2 = \Gamma_2$.
    By \ih on $t_1$ and $t_2$, there exist $\Phi'_1 \bangAGKMeanTr
    (\Gamma_1^1; y : \N) + \Gamma_2^1 \vdash t_1\isub{x}{u} : \N
    \typeArrow \sigma$ and $\Phi'_2 \bangAGKMeanTr \Gamma_1^2 +
    \Gamma_2^2 \vdash t_2\isub{x}{u} : \N$. By $\alpha$-conversion,
    one has that $y \notin \freeVar{u}$ so that $(\Gamma_1^1; y : \N)
    + \Gamma_2^1 = (\Gamma_1^1 + \Gamma_2^1); y : \N$. Since
    $\bangBKRVInhPred{\Gamma_1}$ then $\bangBKRVInhPred{\Gamma_1^1 +
    \Gamma_1^2}$. Moreover, from $\Pi_2$ and
    \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(Gam)_and_inh(sig)},
    one deduces that $\bangBKRVInhPred{\Gamma_2^1 + \Gamma_2^2}$ so
    that $\bangBKRVInhPred{\Gamma_1^1 + \Gamma_2^1 + \Gamma_1^2 +
    \Gamma_2^2}$. We set $\Pi$ as follows:
    \begin{equation*} \hspace{-0.5cm}
        \begin{prooftree}
            \hypo{\Phi'_1 \bangAGKMeanTr (\Gamma_1^1 + \Gamma_2^1); y : \N \vdash t_1\isub{x}{u} : \N \typeArrow \sigma}
            \hypo{\Phi'_2 \bangAGKMeanTr \Gamma_1^2 + \Gamma_2^2 \vdash t_2\isub{x}{u} : \N}
            \inferBangAGKMeanInh{\Gamma_1^1 + \Gamma_2^1 + \Gamma_1^2 + \Gamma_2^2}
            \inferBangAGKMeanEs{\Gamma_1^1 + \Gamma_2^1 + \Gamma_1^2 + \Gamma_2^2 \vdash \app{(t_1\isub{x}{u})}{(t_2\isub{x}{u})} : \sigma}
        \end{prooftree}
    \end{equation*}
    which concludes this case since $\Gamma_1 + \Gamma_2 = (\Gamma_1^1
    + \Gamma_1^2) + (\Gamma_2^1 + \Gamma_2^2) = \Gamma_1^1 +
    \Gamma_2^1 + \Gamma_1^2 + \Gamma_2^2$.

\item[\bltI] $t = \oc t'$: Then $t\isub{x}{u} = \oc (t'\isub{x}{u})$
    and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_i \bangAGKMeanTr \Delta_i \vdash t' : \tau_i}
            \delims{\left(}{\right)_{i \in I}}
            \inferBangAGKMeanInh{+_{i \in I} \Delta_i}
            \inferBangAGKMeanBg{+_{i \in I} \Delta_i \vdash \oc t' : \mset{\tau_i}_{i \in I}}
        \end{prooftree}
    \end{equation*}
    where $+_{i \in I} \Delta_i = \Gamma; x : \M$ and $\sigma =
    \mset{\tau_i}_{i \in I}$. For all $i \in I$, let $\Delta_i =
    \Gamma_1^i; x : \M_i$ such that $\Gamma_1 = +_{i \in I}
    \Gamma_1^i$ for some contexts $\Gamma_1^i$ and some multitypes
    $\M_i$. Using \victorTodo[Splitting Lemma], for all $i \in I$,
    there exists $\Pi_2^i \bangAGKMeanTr \Gamma_2^i \vdash u : \M_i$
    such that $\Gamma_2 = +_{i \in I} \Gamma_2^i$. By \ih on $t'$,
    there exist $\Phi'_i \bangAGKMeanTr \Gamma_1^i + \Gamma_2^i \vdash
    t'\isub{x}{u} : \tau_i$. Since $\bangBKRVInhPred{+_{i \in I}
    \Delta_i}$ then $\bangBKRVInhPred{+_{i \in I} \Gamma_1^i}$.
    Moreover, using
    \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(Gam)_and_inh(sig)},
    one deduces that $\bangBKRVInhPred{\Gamma_2}$ thus
    $\bangBKRVInhPred{+_{i \in I} \Gamma_2^i}$ and therefore
    $\bangBKRVInhPred{+_{i \in I} (\Gamma_1^i + \Gamma_2^i)}$. We set
    $\Pi$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi'_i \bangAGKMeanTr \Gamma_1^i + \Gamma_2^i \vdash t'\isub{x}{u} : \tau_i}
            \delims{\left(}{\right)_{i \in I}}
            \inferBangAGKMeanInh{+_{i \in I} (\Gamma_1^i + \Gamma_2^i)}
            \inferBangAGKMeanBg{+_{i \in I} (\Gamma_1^i + \Gamma_2^i) \vdash \oc(t'\isub{x}{u}) : \mset{\tau_i}_{i \in I}}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $t = \der{t'}$: Then $t\isub{x}{u} = \der{t'\isub{x}{u}}$
    and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi \bangAGKMeanTr \Gamma_1; x : \M \vdash t' : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma_1; x : \M \vdash \der{t'} : \sigma}
        \end{prooftree}
    \end{equation*}
    By \ih on $t'$, one obtains $\Phi' \bangAGKMeanTr \Gamma_1 +
    \Gamma_2 \vdash t'\isub{x}{u} : \mset{\sigma}$. We set $\Pi$ as
    follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi' \bangAGKMeanTr \Gamma_1 + \Gamma_2 \vdash t'\isub{x}{u} : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma_1 + \Gamma_2 \vdash \der{t'\isub{x}{u}} : \sigma}
        \end{prooftree}
    \end{equation*}
\end{itemize}
\end{proof}


==> 3_Proofs/BangAGKMean_Surface_Subject_Expansion.tex <==
\begin{proof}
Let $\Pi \bangAGKMeanTr \Gamma \vdash u : \sigma$ and $t
\bangArr_{S} u$. By definition, there exists a context
$\bangStratCtxt$ and terms $t', u' \in \bangSetTerms$ such that $t =
\bangStratCtxt<t'>$, $u = \bangStratCtxt<u'>$ and $t' \mapstoR u'$
for some $\rel \in \{\bangSymbBeta, \bangSymbSubs, \bangSymbBang\}$.
By induction on $\bangStratCtxt$. Cases:
\begin{itemize}
\item[\bltI] $\bangStratCtxt = \Hole$: Then $t = t'$ and $u = u'$.
    We distinguish three cases:
    \begin{itemize}
    \item[\bltII] $\rel = \bangSymbBeta$: Then $t' =
        \app{\bangLCtxt<\abs{x}{s_1}>}{s_2}$ and $u' =
        \bangLCtxt<s_1\esub{x}{s_2}>$ for some context $\bangLCtxt$
        and some terms $s_1, s_2 \in \bangSetTerms$. By induction on
        $\bangLCtxt$. Cases:
        \begin{itemize}
        \item[\bltI] $\bangLCtxt = \Hole$: Then $\Pi$ has the
        following form:
        \begin{equation*}
            \begin{prooftree}
                \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s_1 : \sigma}
                \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s_2 : \M}
                \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s_1\esub{x}{s_2} : \sigma}
            \end{prooftree}
        \end{equation*}
        We set $\Pi'$ as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s_1 : \sigma}
                \inferBangAGKMeanAbs{\Gamma_1 \vdash \abs{x}{s_1} : \M \typeArrow \sigma}
                \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s_2 : \M}
                \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{(\abs{x}{s_1})}{s_2} : \sigma}
            \end{prooftree}
        \end{equation*}

        \item[\bltI] $\bangLCtxt = \bangLCtxt'\esub{y}{s'}$: Then
            $\Pi$ has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<s_1\esub{x}{s_2}> : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangLCtxt'<s_1\esub{x}{s_2}>\esub{y}{s'} : \sigma}
                \end{prooftree}
            \end{equation*}
            with $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\Pi_1$,
            one obtains $\Phi \bangAGKMeanTr \Gamma_1; y : \M \vdash
            \app{\bangLCtxt'<\abs{x}{s_1}>}{s_2} : \sigma$. By
            construction, $\Phi$ necessarily has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Phi_1 \bangAGKMeanTr \Delta_1 \vdash \bangLCtxt'<\abs{x}{s_1}> : \N \typeArrow \sigma}
                    \hypo{\Phi_2 \bangAGKMeanTr \Delta_2 \vdash s_2 : \N}
                    \inferBangAGKMeanInh{\Delta_1 + \Delta_2}
                    \inferBangAGKMeanApp{\Delta_1 + \Delta_2 \vdash \app{\bangLCtxt'<\abs{x}{s_1}>}{s_2} : \sigma}
                \end{prooftree}
            \end{equation*}
            for some type $\N$ and some type context $\Delta_1,
            \Delta_2$ such that $\Gamma_1; y : \M = \Delta_1 +
            \Delta_2$. By $\alpha$-conversion, $y \notin
            \freeVar{s_2}$ thus $\Delta_1 = \Delta'_1; y : \M$ and
            $\Gamma_1 = \Delta'_1 + \Delta_2$. By hypothesis
            $\bangBKRVInhPred{\Gamma}$ but since $\Gamma = \Gamma_1 +
            \Gamma_2 = \Delta'_1 + \Delta_2 + \Gamma_2$ then
            $\bangBKRVInhPred{\Delta'_1 + \Gamma_2 + \Delta_2}$ and
            $\bangBKRVInhPred{\Delta'_1 + \Gamma_2}$. We set $\Pi'$ as
            follows
            \begin{equation*}\hspace{-3.5cm}
                \begin{prooftree}
                    \hypo{\Phi_1 \bangAGKMeanTr \Delta'_1; y : \M \vdash \bangLCtxt'<\abs{x}{s_1}> : \N \typeArrow \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Delta'_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Delta'_1 + \Gamma_2 \vdash \bangLCtxt'<\abs{x}{s_1}>\esub{y}{s'} : \N \typeArrow \sigma}
                    \hypo{\Phi_2 \bangAGKMeanTr \Delta_2 \vdash s_2 : \N}
                    \inferBangAGKMeanInh{\Delta'_1 + \Gamma_2 + \Delta_2}
                    \inferBangAGKMeanApp{\Delta'_1 + \Gamma_2 + \Delta_2 \vdash \app{\bangLCtxt<\abs{x}{s_1}>}{s_2} : \sigma}
                \end{prooftree}
            \end{equation*}
        \end{itemize}
        We conclude since $\Delta'_1 + \Gamma_2  + \Delta_2  =
        \Gamma$.
    \item[\bltII] $\rel = \bangSymbSubs$: Then $t' =
        s_1\esub{x}{\bangLCtxt<\oc s_2>}$ and $u' =
        \bangLCtxt<s_1\isub{x}{s_2}>$ for some context $\bangLCtxt$
        and some terms $s_1, s_2 \in \bangSetTerms$. By induction on
        $\bangLCtxt$. Cases:
        \begin{itemize}
        \item[\bltI] $\bangLCtxt = \Hole$: Then $t =
            s_1\isub{x}{s_2}$, $u = s_1\esub{x}{s_2}$ and $\Pi
            \bangAGKMeanTr \Gamma \vdash s_1\isub{x}{s_2} : s_2$.
            Using \Cref{lem:BangAGKMean_Reverse_Substitution}, one
            obtains $\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s_1
            : \sigma$ and $\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash \oc
            s_2 : \M$ such that $\Gamma = \Gamma_1 + \Gamma_2$. Using,
            \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(Gam)_and_inh(sig)},
            one has that $\bangBKRVInhPred{\Gamma}$ thus
            $\bangBKRVInhPred{\Gamma_1 + \Gamma_2}$. We set $\Pi'$ as
            follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s_1 : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash \oc s_2 : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s_1\esub{x}{\oc s_2} : \sigma}
                \end{prooftree}
            \end{equation*}

        \item[\bltI] $\bangLCtxt = \bangLCtxt'\esub{y}{s'}$: Then
            $\Pi$ has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<s_1\isub{x}{s_2}> : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangLCtxt'<s_1\isub{x}{s_2}>\esub{y}{s'} : \sigma}
                \end{prooftree}
            \end{equation*}
            with $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\Pi_1$,
            one obtains $\Phi \bangAGKMeanTr \Gamma_1; y : \M \vdash
            s_1\esub{x}{\bangLCtxt'<\oc s_2>} : \sigma$. By
            construction, $\Phi$ necessarily has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Phi_1 \bangAGKMeanTr \Delta_1; x : \N \vdash s_1 : \sigma}
                    \hypo{\Phi_2 \bangAGKMeanTr \Delta_2 \vdash \bangLCtxt'<\oc s_2> : \N}
                    \inferBangAGKMeanInh{\Delta_1 + \Delta_2}
                    \inferBangAGKMeanEs{\Delta_1 + \Delta_2 \vdash s_1\esub{x}{\bangLCtxt'<\oc s_2>} : \sigma}
                \end{prooftree}
            \end{equation*}
            for some type $\N$ and some type context $\Delta_1,
            \Delta_2$ such that $\Gamma_1; y : \M = \Delta_1 +
            \Delta_2$. By $\alpha$-conversion, $y \notin
            \freeVar{s_1}$ thus $\Delta_2 = \Delta'_2; y : \M$ and
            $\Gamma_1 = \Delta_1 + \Delta'_2$. By hypothesis
            $\bangBKRVInhPred{\Gamma}$ but since $\Gamma = \Gamma_1 +
            \Gamma_2 = \Delta_1 + \Delta'_2 + \Gamma_2$ then
            $\bangBKRVInhPred{\Delta_1 + \Delta'_2 + \Gamma_2}$ and
            $\bangBKRVInhPred{\Delta'_2 + \Gamma_2}$. We set $\Pi'$ as
            follows
            \begin{equation*}\hspace{-2.5cm}
                \begin{prooftree}
                    \hypo{\Phi_1 \bangAGKMeanTr \Delta_1; x : \N \vdash s_1 : \sigma}
                    \hypo{\Phi_2 \bangAGKMeanTr \Delta'_2; y : \M \vdash \bangLCtxt'<\oc s_2> : \N}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Delta'_2 + \Gamma_2}
                    \inferBangAGKMeanEs{\Delta'_2 + \Gamma_2 \vdash \bangLCtxt'<\oc s_2>\esub{y}{s'} : \N}
                    \inferBangAGKMeanInh{\Delta_1 + \Delta'_2 + \Gamma_2}
                    \inferBangAGKMeanEs{\Delta_1 + \Delta'_2 + \Gamma_2 \vdash s_1\esub{x}{\bangLCtxt'<\oc s_2>\esub{y}{s'}} : \sigma}
                \end{prooftree}
            \end{equation*}
        \end{itemize}
        We conclude since $\Delta_1 + \Delta'_2 + \Gamma_2  = \Gamma$.
    \item[\bltII] $\rel = \bangSymbBang$: Then $t' =
        \der{\bangLCtxt<\oc s>}$ and $u' = \bangLCtxt<s>$ for some
        context $\bangLCtxt$ and some term $s \in \bangSetTerms$. By
        induction on $\bangLCtxt$. Cases:
        \begin{itemize}
        \item[\bltI] $\bangLCtxt = \Hole$: Then $t = \der{\oc u}$, $u
            = s$ and $\Pi \bangAGKMeanTr \Gamma \vdash s : \sigma$.
            Using
            \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(Gam)_and_inh(sig)},
            one deduces that $\bangBKRVInhPred{\Gamma}$ and
            $\bangBKRVInhPred{\bangArgs{\sigma}}$. We set $\Pi'$ as
            follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi \bangAGKMeanTr \Gamma \vdash s : \sigma}
                    \inferBangAGKMeanInh{\Gamma}
                    \inferBangAGKMeanBg{\Gamma \vdash \oc s : \mset{\sigma}}
                    \inferBangAGKMeanInh{\bangArgs{\sigma}}
                    \inferBangAGKMeanDer{\Gamma \vdash \der{\oc u} : \sigma}
                \end{prooftree}
            \end{equation*}

        \item[\bltI] $\bangLCtxt = \bangLCtxt'\esub{y}{s'}$: Then
            $\Pi$ has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<s> : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangLCtxt'<s>\esub{y}{s'} : \sigma}
                \end{prooftree}
            \end{equation*}
            with $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\Pi_1$,
            one obtains $\Phi \bangAGKMeanTr \Gamma_1; y : \M \vdash
            \der{\bangLCtxt'<\oc s>} : \sigma$. By construction,
            $\Phi$ necessarily has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Phi' \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<\oc s> : \mset{\sigma}}
                    \inferBangAGKMeanInh{\bangArgs{\sigma}}
                    \inferBangAGKMeanDer{\Gamma_1; y : \M \vdash \der{\bangLCtxt'<\oc u>} : \sigma}
                \end{prooftree}
            \end{equation*}
            We set $\Pi'$ as follows
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Phi' \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<\oc s> : \mset{\sigma}}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangLCtxt'<\oc s>\esub{y}{s'} : \mset{\sigma}}
                    \inferBangAGKMeanInh{\bangArgs{\sigma}}
                    \inferBangAGKMeanDer{\Gamma \vdash \der{\bangLCtxt'<\oc s>\esub{y}{s'}} : \sigma}
                \end{prooftree}
            \end{equation*}
        \end{itemize}
    \end{itemize}

\item[\bltI] $\bangStratCtxt = \abs{x}{\bangStratCtxt'}$: Then $t
    = \abs{x}{\bangStratCtxt'<t'>}$, $u =
    \abs{x}{\bangStratCtxt'<u'>}$ and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi \bangAGKMeanTr \Gamma; x : \M \vdash \bangStratCtxt'<u'> : \sigma}
            \inferBangAGKMeanAbs{\Gamma \vdash \abs{x}{\bangStratCtxt'<u'>} : \M \typeArrow \sigma}
        \end{prooftree}
    \end{equation*}
    By \ih on $\bangStratCtxt'$, there exists $\Phi' \bangAGKMeanTr
    \Gamma; x : \M \vdash \bangStratCtxt'<t'> : \sigma$. We set
    $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi' \bangAGKMeanTr \Gamma; x : \M \vdash \bangStratCtxt'<t'> : \sigma}
            \inferBangAGKMeanAbs{\Gamma \vdash \abs{x}{\bangStratCtxt'<t'>} : \M \typeArrow \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \app{\bangStratCtxt'}{s}$: Then $t
    = \app{\bangStratCtxt'<t'>}{s}$, $u =
    \app{\bangStratCtxt'<u'>}{s}$ and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash \bangStratCtxt'<u'> : \M \typeArrow \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{\bangStratCtxt'<u'>}{s} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on
    $\bangStratCtxt'$, there exists $\Pi'_1 \bangAGKMeanTr \Gamma_1
    \vdash \bangStratCtxt'<t'> : \M \typeArrow \sigma$. We set
    $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_1 \bangAGKMeanTr \Gamma_1 \vdash \bangStratCtxt'<t'> : \M \typeArrow \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{\bangStratCtxt'<t'>}{s} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \app[\,]{s}{\bangStratCtxt'}$: Then
    $t = \app[\,]{s}{\bangStratCtxt'<t'>}$, $u =
    \app[\,]{s}{\bangStratCtxt'<u'>}$ and $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash s : \M \typeArrow \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<u'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app[\,]{s}{\bangStratCtxt'<u'>} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on
    $\bangStratCtxt'$, there exists $\Pi'_2 \bangAGKMeanTr \Gamma_2
    \vdash \bangStratCtxt'<t'> : \M$. We set $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash s : \M \typeArrow \sigma}
            \hypo{\Pi'_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<t'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app[\,]{s}{\bangStratCtxt'<t'>} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \bangStratCtxt'\esub{x}{s}$: Then
    $t = \bangStratCtxt'<t'>\esub{x}{s}$, $u =
    \bangStratCtxt'<u'>\esub{x}{s}$ and $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash \bangStratCtxt'<u'> : \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangStratCtxt'<u'>\esub{x}{s} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on
    $\bangStratCtxt'$, there exists $\Pi'_1 \bangAGKMeanTr \Gamma_1;
    x : \M \vdash \bangStratCtxt'<t'> : \sigma$. We set $\Pi'$ as
    follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash \bangStratCtxt'<t'> : \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangStratCtxt'<t'>\esub{x}{s} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = s\esub{x}{\bangStratCtxt'}$: Then
    $t = s\esub{x}{\bangStratCtxt'<t'>}$, $u =
    s\esub{x}{\bangStratCtxt'<u'>}$ and $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s : \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<u'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s\esub{x}{\bangStratCtxt'<u'>} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on
    $\bangStratCtxt'$, there exists $\Pi'_2 \bangAGKMeanTr \Gamma_2
    \vdash \bangStratCtxt'<t'> : \M$. We set $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s : \sigma}
            \hypo{\Pi'_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<t'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s\esub{x}{\bangStratCtxt'<t'>} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \der{\bangStratCtxt'}$: Then $t =
    \der{\bangStratCtxt'<t'>}$, $u = \der{\bangStratCtxt'<u'>}$
    and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi \bangAGKMeanTr \Gamma \vdash \bangStratCtxt'<u'> : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma \vdash \der{\bangStratCtxt'<u'>} : \sigma}
        \end{prooftree}
    \end{equation*}
    By \ih on $\bangStratCtxt'$, there exists $\Phi' \bangAGKMeanTr
    \Gamma \vdash \bangStratCtxt'<t'> : \mset{\sigma}$. We set
    $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi' \bangAGKMeanTr \Gamma \vdash \bangStratCtxt'<t'> : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma \vdash \der{\bangStratCtxt'<t'>} : \sigma}
        \end{prooftree}
    \end{equation*}

% \item[\bltI] $\bangStratCtxt = \oc\bangStratCtxt$: Then $t =
%     \oc\bangStratCtxt<t'>$ and $u = \oc\bangStratCtxt<u'>$ and
%     $\Pi$ has the following form:
%     \begin{equation*}
%         \begin{prooftree}
%             \hypo{\Phi_i \bangAGKMeanTr \Gamma_i \vdash \bangStratCtxt'<u'> : \sigma_i}
%             \delims{\left(}{\right)_{i \in I}}
%             \inferBangAGKMeanInh{\bangArgs{+_{i \in I} \Gamma_i}}
%             \inferBangAGKMeanBg{+_{i \in I} \Gamma_i \vdash \oc\bangStratCtxt'<u'> : \mset{\sigma_i}_{i \in I}}
%         \end{prooftree}
%     \end{equation*}
%     For every $i \in I$, by \ih on $\bangStratCtxt'$, there exists
%     $\Phi'_i \bangAGKMeanTr \Gamma_i \vdash \bangStratCtxt'<t'> :
%     \sigma_i$. We set $\Pi'$ as follows:
%     \begin{equation*}
%         \begin{prooftree}
%             \hypo{\Phi'_i \bangAGKMeanTr \Gamma_i \vdash \bangStratCtxt'<t'> : \sigma_i}
%             \delims{\left(}{\right)_{i \in I}}
%             \inferBangAGKMeanInh{\bangArgs{+_{i \in I} \Gamma_i}}
%             \inferBangAGKMeanBg{+_{i \in I} \Gamma_i \vdash \oc\bangStratCtxt'<t'> : \mset{\sigma_i}_{i \in I}}
%         \end{prooftree}
%     \end{equation*}
\end{itemize}
\end{proof}

==> 3_Proofs/BangAGKMean_Surface_Subject_Reduction.tex <==
\begin{proof}
Let $\Pi \bangAGKMeanTr \Gamma \vdash t : \sigma$ and $t \bangArr_{S}
u$. By definition, there exists a context $\bangStratCtxt$ and terms
$t', u' \in \bangSetTerms$ such that $t = \bangStratCtxt<t'>$, $u =
\bangStratCtxt<u'>$ and $t' \mapstoR u'$ for some $\rel \in
\{\bangSymbBeta, \bangSymbSubs, \bangSymbBang\}$. By induction on
$\bangStratCtxt$. Cases:
\begin{itemize}
\item[\bltI] $\bangStratCtxt = \Hole$: Then $t = t'$ and $u = u'$. We
    distinguish three cases:
    \begin{itemize}
    \item[\bltII] $\rel = \bangSymbBeta$: Then $t' =
        \app{\bangLCtxt<\abs{x}{s_1}>}{s_2}$ and $u' =
        \bangLCtxt<s_1\esub{x}{s_2}>$ for some context $\bangLCtxt$
        and some terms $s_1, s_2 \in \bangSetTerms$. By induction on
        $\bangLCtxt$. Cases:
        \begin{itemize}
        \item[\bltI] $\bangLCtxt = \Hole$: Then $\Pi$ has the
        following form:
        \begin{equation*}
            \begin{prooftree}
                \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s_1 : \sigma}
                \inferBangAGKMeanAbs{\Gamma_1 \vdash \abs{x}{s_1} : \M \typeArrow \sigma}
                \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s_2 : \M}
                \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{(\abs{x}{s_1})}{s_2} : \sigma}
            \end{prooftree}
        \end{equation*}
        with $\Gamma = \Gamma_1 + \Gamma_2$. We set $\Pi'$ as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s_1 : \sigma}
                \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s_2 : \M}
                \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s_1\esub{x}{s_2} : \sigma}
            \end{prooftree}
        \end{equation*}

        \item[\bltI] $\bangLCtxt = \bangLCtxt'\esub{y}{s'}$: Then
            $\Pi$ has the following form:
            \begin{equation*}\hspace{-3.5cm}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<\abs{x}{s_1}> : \N \typeArrow \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangLCtxt'<\abs{x}{s_1}>\esub{y}{s'} : \N \typeArrow \sigma}
                    \hypo{\Pi_3 \bangAGKMeanTr \Gamma_3 \vdash s_2 : \N}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2 + \Gamma_3}
                    \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 + \Gamma_3 \vdash \app{\bangLCtxt<\abs{x}{s_1}>}{s_2} : \sigma}
                \end{prooftree}
            \end{equation*}
            with $\Gamma = \Gamma_1 + \Gamma_2 + \Gamma_3$. From
            $\bangBKRVInhPred{\Gamma}$ one deduces
            $\bangBKRVInhPred{\Gamma_1}$, $\bangBKRVInhPred{\Gamma_2}$
            and $\bangBKRVInhPred{\Gamma_3}$. Thus, using
            \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(sigma)} with
            $\Pi_2$, one deduces that $\bangBKRVInhPred{\M}$ so that
            $\bangBKRVInhPred{(\Gamma_1; y : \M) + \Gamma_3}$. Let
            $\Phi$ be the following derivation:
            \begin{equation*} \hspace{1cm}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<\abs{x}{s_1}> : \N \typeArrow \sigma}
                    \hypo{\Pi_3 \bangAGKMeanTr \Gamma_3 \vdash s_2 : \N}
                    \inferBangAGKMeanInh{(\Gamma_1; y : \M) + \Gamma_3}
                    \inferBangAGKMeanApp{(\Gamma_1; y : \M) + \Gamma_3 \vdash \app{\bangLCtxt'<\abs{x}{s_1}>}{s_2} : \sigma}
                \end{prooftree}
            \end{equation*}
            By \ih on $\bangLCtxt'$, there exist $\Phi' \bangAGKMeanTr
            (\Gamma_1; y : \M) + \Gamma_3 \vdash
            \bangLCtxt'<s_1\esub{x}{s_2}> : \sigma$. By
            $\alpha$-conversion, one has that $y \notin \freeVar{s'}$
            so that $(\Gamma_1; y : \M) + \Gamma_3 = (\Gamma_1 +
            \Gamma_3); y : \M$. We set $\Pi'$ as follows:
            \begin{equation*}\hspace{1.25cm}
                \begin{prooftree}
                    \hypo{\Phi' \bangAGKMeanTr (\Gamma_1 + \Gamma_3); y : \M \vdash \bangLCtxt'<s_1\esub{x}{s_2}> : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_3 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_3 + \Gamma_2 \vdash \bangLCtxt<s_1\esub{x}{s_2}> : \sigma}
                \end{prooftree}
            \end{equation*}
            which concludes this case since $\Gamma = \Gamma_1 +
            \Gamma_3 + \Gamma_2$.
        \end{itemize}

    \item[\bltII] $\rel = \bangSymbSubs$: Then $t' =
        s_1\esub{x}{\bangLCtxt<\oc s_2>}$ and $u' =
        \bangLCtxt<s_1\isub{x}{s_2}>$ for some context $\bangLCtxt$
        and some terms $s_1, s_2 \in \bangSetTerms$. By induction on
        $\bangLCtxt$. Cases:
        \begin{itemize}
        \item[\bltI] $\bangLCtxt = \Hole$: Then $\Pi$ has the
            following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s_1 : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash \oc s_2 : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s_1\esub{x}{\oc s_2} : \sigma}
                \end{prooftree}
            \end{equation*}
            One concludes this case using \victorTodo[Substitution
            Lemma] with $\Pi_1$ and $\Pi_2$.

        \item[\bltI] $\bangLCtxt = \bangLCtxt'\esub{y}{s'}$: Then
            $\Pi$ has the following form:
            \begin{equation*}\hspace{-2.5cm}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \N \vdash s_1 : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2; y : \M \vdash \bangLCtxt'<\oc s_2> : \N}
                    \hypo{\Pi_3 \bangAGKMeanTr \Gamma_3 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_2 + \Gamma_3}
                    \inferBangAGKMeanEs{\Gamma_2 + \Gamma_3 \vdash \bangLCtxt'<\oc s_2>\esub{y}{s'} : \N}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2 + \Gamma_3}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 + \Gamma_3 \vdash s_1\esub{x}{\bangLCtxt'<\oc s_2>\esub{y}{s'}} : \sigma}
                \end{prooftree}
            \end{equation*}
            with $\Gamma = \Gamma_1 + \Gamma_2 + \Gamma_3$. From
            $\bangBKRVInhPred{\Gamma}$ one deduces that
            $\bangBKRVInhPred{\Gamma_1}$, $\bangBKRVInhPred{\Gamma_2}$
            and $\bangBKRVInhPred{\Gamma_3}$. Thus, using
            \Cref{lem:bangAGKMean_Gam_|-_t_:_sig_==>_inh(sigma)} with
            $\Pi_3$, one deduces that $\bangBKRVInhPred{\M}$ so that
            $\bangBKRVInhPred{\Gamma_1 + (\Gamma_2; y : \M)}$. Let
            $\Phi$ be the following derivation:
            \begin{equation*} \hspace{1cm}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \N \vdash s_1 : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2; y : \M \vdash \bangLCtxt'<\oc s_2> : \N}
                    \inferBangAGKMeanInh{\Gamma_1 + (\Gamma_2; y : \M)}
                    \inferBangAGKMeanEs{\Gamma_1 + (\Gamma_2; y : \M) \vdash s_1\esub{x}{\bangLCtxt'<\oc s_2>} : \sigma}
                \end{prooftree}
            \end{equation*}
            By \ih on $\bangLCtxt'$, there exists $\Phi'
            \bangAGKMeanTr \Gamma_1 + (\Gamma_2; y : \M) \vdash
            \bangLCtxt'<s_1\isub{x}{s_2}> : \sigma$. By
            $\alpha$-conversion, one has that $y \notin \freeVar{s_1}$
            so that $\Gamma_1 + (\Gamma_2; y : \M) = (\Gamma_1 +
            \Gamma_2); y : \M$. We set $\Pi'$ as follows:
            \begin{equation*} \hspace{1cm}
                \begin{prooftree}
                    \hypo{\Phi' \bangAGKMeanTr (\Gamma_1 + \Gamma_2); y : \M \vdash \bangLCtxt'<s_1\isub{x}{s_2}> : \sigma}
                    \hypo{\Pi_3 \bangAGKMeanTr \Gamma_3 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2 + \Gamma_3}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 + \Gamma_3 \vdash s_1\esub{x}{\bangLCtxt<\oc s_2>} : \sigma}
                \end{prooftree}
            \end{equation*}
            which concludes this case since $\Gamma = \Gamma_1 +
            \Gamma_2 + \Gamma_3$.
        \end{itemize}

    \item[\bltII] $\rel = \bangSymbBang$: Then $t' =
        \der{\bangLCtxt<\oc s>}$ and $u' = \bangLCtxt<s>$ for some
        context $\bangLCtxt$ and some term $s \in \bangSetTerms$. By
        induction on $\bangLCtxt$. Cases:
        \begin{itemize}
        \item[\bltI] $\bangLCtxt = \Hole$: Then $t = \der{\oc u}$, $u
            = s$ and $\Pi$ has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Phi \bangAGKMeanTr \Gamma \vdash s : \sigma}
                    \inferBangAGKMeanInh{\Gamma}
                    \inferBangAGKMeanBg{\Gamma \vdash \oc s : \mset{\sigma}}
                    \inferBangAGKMeanInh{\bangArgs{\sigma}}
                    \inferBangAGKMeanDer{\Gamma \vdash \der{\oc u} : \sigma}
                \end{prooftree}
            \end{equation*}
            We set $\Pi' := \Phi$ concluding this case.

        \item[\bltI] $\bangLCtxt = \bangLCtxt'\esub{y}{s'}$: Then
            $\Pi$ has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<\oc s> : \mset{\sigma}}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangLCtxt'<\oc s>\esub{y}{s'} : \mset{\sigma}}
                    \inferBangAGKMeanInh{\bangArgs{\sigma}}
                    \inferBangAGKMeanDer{\Gamma_1 + \Gamma_2 \vdash \der{\bangLCtxt'<\oc s>\esub{y}{s'}} : \sigma}
                \end{prooftree}
            \end{equation*}
            Let $\Phi$ be the following derivation:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; y : \M \vdash \bangLCtxt'<\oc s> : \mset{\sigma}}
                    \inferBangAGKMeanInh{\bangArgs{\sigma}}
                    \inferBangAGKMeanDer{\Gamma_1, y : \M \vdash \der{\bangLCtxt'<\oc s>} : \sigma}
                \end{prooftree}
            \end{equation*}
            By \ih on $\bangLCtxt'$, there exists $\Phi'
            \bangAGKMeanTr \Gamma_1, y : \M \vdash \bangLCtxt'<s> :
            \sigma$. We set $\Pi'$ as follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypo{\Phi' \bangAGKMeanTr \Gamma_1, y : \M \vdash \bangLCtxt'<s> : \sigma}
                    \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s' : \M}
                    \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                    \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangLCtxt'<s>\esub{y}{s'} : \sigma}
                \end{prooftree}
            \end{equation*}
            concluding this case since $\Gamma = \Gamma_1 + \Gamma_2$.
        \end{itemize}
    \end{itemize}

\item[\bltI] $\bangStratCtxt = \abs{x}{\bangStratCtxt'}$: Then $t =
    \abs{x}{\bangStratCtxt'<t'>}$, $u = \abs{x}{\bangStratCtxt'<u'>}$
    and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi \bangAGKMeanTr \Gamma; x : \M \vdash \bangStratCtxt'<t'> : \sigma}
            \inferBangAGKMeanAbs{\Gamma \vdash \abs{x}{\bangStratCtxt'<t'>} : \M \typeArrow \sigma}
        \end{prooftree}
    \end{equation*}
    By \ih on $\bangStratCtxt'$, there exists $\Phi' \bangAGKMeanTr
    \Gamma; x : \M \vdash \bangStratCtxt'<u'> : \sigma$. We set $\Pi'$
    as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi' \bangAGKMeanTr \Gamma; x : \M \vdash \bangStratCtxt'<u'> : \sigma}
            \inferBangAGKMeanAbs{\Gamma \vdash \abs{x}{\bangStratCtxt'<u'>} : \M \typeArrow \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \app{\bangStratCtxt'}{s}$: Then $t =
    \app{\bangStratCtxt'<t'>}{s}$, $u = \app{\bangStratCtxt'<u'>}{s}$
    and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash \bangStratCtxt'<t'> : \M \typeArrow \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{\bangStratCtxt'<t'>}{s} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\bangStratCtxt'$,
    there exists $\Pi'_1 \bangAGKMeanTr \Gamma_1 \vdash
    \bangStratCtxt'<u'> : \M \typeArrow \sigma$. We set $\Pi'$ as
    follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_1 \bangAGKMeanTr \Gamma_1 \vdash \bangStratCtxt'<u'> : \M \typeArrow \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{\bangStratCtxt'<u'>}{s} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \app[\,]{s}{\bangStratCtxt'}$: Then $t
    = \app[\,]{s}{\bangStratCtxt'<t'>}$, $u =
    \app[\,]{s}{\bangStratCtxt'<u'>}$ and $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash s : \M \typeArrow \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<t'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app[\,]{s}{\bangStratCtxt'<t'>} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\bangStratCtxt'$,
    there exists $\Pi'_2 \bangAGKMeanTr \Gamma_2 \vdash
    \bangStratCtxt'<u'> : \M$. We set $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash s : \M \typeArrow \sigma}
            \hypo{\Pi'_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<u'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app[\,]{s}{\bangStratCtxt'<u'>} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \bangStratCtxt'\esub{x}{s}$: Then $t =
    \bangStratCtxt'<t'>\esub{x}{s}$, $u =
    \bangStratCtxt'<u'>\esub{x}{s}$ and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash \bangStratCtxt'<t'> : \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangStratCtxt'<t'>\esub{x}{s} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\bangStratCtxt'$,
    there exists $\Pi'_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash
    \bangStratCtxt'<u'> : \sigma$. We set $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi'_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash \bangStratCtxt'<u'> : \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash s : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash \bangStratCtxt'<u'>\esub{x}{s} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = s\esub{x}{\bangStratCtxt'}$: Then
    $t = s\esub{x}{\bangStratCtxt'<t'>}$, $u =
    s\esub{x}{\bangStratCtxt'<u'>}$ and $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s : \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<t'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s\esub{x}{\bangStratCtxt'<t'>} : \sigma}
        \end{prooftree}
    \end{equation*}
    for some type $\M$ and some type context $\Gamma_1, \Gamma_2$ such
    that $\Gamma = \Gamma_1 + \Gamma_2$. By \ih on $\bangStratCtxt'$,
    there exists $\Pi'_2 \bangAGKMeanTr \Gamma_2 \vdash
    \bangStratCtxt'<u'> : \M$. We set $\Pi'$ as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash s : \sigma}
            \hypo{\Pi'_2 \bangAGKMeanTr \Gamma_2 \vdash \bangStratCtxt'<u'> : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash s\esub{x}{\bangStratCtxt'<u'>} : \sigma}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\bangStratCtxt = \der{\bangStratCtxt'}$: Then $t =
    \der{\bangStratCtxt'<t'>}$, $u = \der{\bangStratCtxt'<u'>}$ and
    $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi \bangAGKMeanTr \Gamma \vdash \bangStratCtxt'<t'> : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma \vdash \der{\bangStratCtxt'<t'>} : \sigma}
        \end{prooftree}
    \end{equation*}
    By \ih on $\bangStratCtxt'$, there exists $\Phi' \bangAGKMeanTr
    \Gamma \vdash \bangStratCtxt'<u'> : \mset{\sigma}$. We set $\Pi'$
    as follows:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi' \bangAGKMeanTr \Gamma \vdash \bangStratCtxt'<u'> : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma \vdash \der{\bangStratCtxt'<u'>} : \sigma}
        \end{prooftree}
    \end{equation*}

% \item[\bltI] $\bangStratCtxt = \oc\bangStratCtxt$: Then $t =
%     \oc\bangStratCtxt<t'>$ and $u = \oc\bangStratCtxt<u'>$ and
%     $\Pi$ has the following form:
%     \begin{equation*}
%         \begin{prooftree}
%             \hypo{\Phi_i \bangAGKMeanTr \Gamma_i \vdash \bangStratCtxt'<t'> : \sigma_i}
%             \delims{\left(}{\right)_{i \in I}}
%             \inferBangAGKMeanInh{\bangArgs{+_{i \in I} \Gamma_i}}
%             \inferBangAGKMeanBg{+_{i \in I} \Gamma_i \vdash \oc\bangStratCtxt'<t'> : \mset{\sigma_i}_{i \in I}}
%         \end{prooftree}
%     \end{equation*}
%     For every $i \in I$, by \ih on $\bangStratCtxt'$, there exists
%     $\Phi'_i \bangAGKMeanTr \Gamma_i \vdash \bangStratCtxt'<u'> :
%     \sigma_i$. We set $\Pi'$ as follows:
%     \begin{equation*}
%         \begin{prooftree}
%             \hypo{\Phi'_i \bangAGKMeanTr \Gamma_i \vdash \bangStratCtxt'<u'> : \sigma_i}
%             \delims{\left(}{\right)_{i \in I}}
%             \inferBangAGKMeanInh{\bangArgs{+_{i \in I} \Gamma_i}}
%             \inferBangAGKMeanBg{+_{i \in I} \Gamma_i \vdash \oc\bangStratCtxt'<u'> : \mset{\sigma_i}_{i \in I}}
%         \end{prooftree}
%     \end{equation*}
\end{itemize}
\end{proof}

==> 3_Proofs/BangAGKMean_Typability_Testing_Contexts.tex <==
\begin{proof}
Let $\Pi \bangAGKMeanTr \bangTCtxt<t>$. By induction on $\bangTCtxt$.
Cases:
\begin{itemize}
\item[\bltI] $\bangTCtxt = \Hole$: Then $\bangTCtxt<t> = t$ and $\Pi
    \bangAGKMeanTr t$ holds by hypothesis, which concludes this case.

\item[\bltI] $\bangTCtxt = \app[\,]{(\abs{x}{\bangTCtxt'})}{u}$: Then
    $\bangTCtxt<t> = \app[\,]{(\abs{x}{\bangTCtxt'<t>})}{u}$ and $\Pi$
    has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash \bangTCtxt'<t> : \sigma}
            \inferBangAGKMeanAbs{\Gamma_1 \vdash \abs{x}{\bangTCtxt'<t>} : \M \typeArrow \sigma}

            \hypo{\Phi_2 \bangAGKMeanTr \Gamma_2 \vdash u : \M}

            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}

            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{(\abs{x}{\bangTCtxt'<t>})}{u} : \sigma}
        \end{prooftree}
    \end{equation*}
    By the \ih on $\Phi_1$, one concludes that $\Pi' \bangAGKMeanTr
    t$.

\item[\bltI] $\bangTCtxt = \app{\bangTCtxt'}{u}$: Then $t =
    \app{\bangTCtxt'<t>}{u}$ and $\Pi$ has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Phi_1 \bangAGKMeanTr \Gamma_1 \vdash \bangTCtxt'<t> : \M \typeArrow \sigma}

            \hypo{\Phi_2 \bangAGKMeanTr \Gamma_2 \vdash u : \M}

            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}

            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{\bangTCtxt'<t>}{u} : \sigma}
        \end{prooftree}
    \end{equation*}
    By the \ih on $\Phi_1$, one concludes that $\Pi' \bangAGKMeanTr
    t$.
\end{itemize}
\end{proof}


==> 3_Proofs/BangAGKMean_Typability_implies_Ctxt_and_Args_Inhabitated.tex <==
\begin{proof}
Let $\Pi \bangAGKMeanTr \Gamma \vdash t : \sigma$. By induction on
$\Pi$. Cases:
\begin{itemize}
\item[\bltI] $(\bangAGKMeanVarRuleName)$: Then $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \inferBangAGKMeanInh{\mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanVar{x : \mset{\sigma} \vdash x : \sigma}
        \end{prooftree}
    \end{equation*}
    where $\Gamma = x : \mset{\sigma}$, so that by hypothesis,
    $\bangBKRVInhPred{\Gamma}$ and $\bangBKRVInhPred{\bangArgs{\sigma}}$.

\item[\bltI] $(\bangAGKMeanAbsRuleName)$: Then $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi' \bangAGKMeanTr \Gamma; x : \M \vdash t : \tau}
            \inferBangAGKMeanAbs{\Gamma \vdash \abs{x}{t} : \M \typeArrow \tau}
        \end{prooftree}
    \end{equation*}
    where $\sigma = \M \typeArrow \tau$. By the \ih on $\Pi'$, one
    deduces $\bangBKRVInhPred{\Gamma; x : \M}$ and
    $\bangBKRVInhPred{\bangArgs{\tau}}$. Thus $\bangBKRVInhPred{\Gamma}$ and
    $\bangBKRVInhPred{\M}$,  hence $\bangBKRVInhPred{\bangArgs{\M \typeArrow
    \tau}}$ which concludes this case.

\item[\bltI] $(\bangAGKMeanAppRuleName)$: Then $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash t : \M \typeArrow \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash u : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{t}{u} : \sigma}
        \end{prooftree}
    \end{equation*}
    where $\Gamma = \Gamma_1 + \Gamma_2$. By the \ih on $\Pi_1$, one
    deduces $\bangBKRVInhPred{\bangArgs{\M \typeArrow \sigma}}$ hence in
    particular $\bangBKRVInhPred{\bangArgs{\sigma}}$. Since
    $\bangBKRVInhPred{\Gamma}$ holds by hypothesis, then this concludes
    this case.

\item[\bltI] $(\bangAGKMeanEsRuleName)$: Then $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1; x : \M \vdash t : \sigma}
            \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash u : \M}
            \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
            \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash t\esub{x}{u} : \sigma}
        \end{prooftree}
    \end{equation*}
    where $\Gamma = \Gamma_1 + \Gamma_2$. By the \ih on $\Pi_1$, one
    deduces $\bangBKRVInhPred{\bangArgs{\sigma}}$. Since
    $\bangBKRVInhPred{\Gamma}$ holds by hypothesis, then this concludes
    this case.

\item[\bltI] $(\bangAGKMeanDerRuleName)$: Then $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi' \bangAGKMeanTr \Gamma \vdash t : \mset{\sigma}}
            \inferBangAGKMeanInh{\bangArgs{\sigma}}
            \inferBangAGKMeanDer{\Gamma \vdash \der{t} : \sigma}
        \end{prooftree}
    \end{equation*}
    By the \ih on $\Pi'$, one deduces $\bangBKRVInhPred{\Gamma}$. This
    concludes this case since $\bangBKRVInhPred{\bangArgs{\sigma}}$ holds
    by hypothesis.

\item[\bltI] $(\bangAGKMeanBgRuleName)$: Then $\Pi$ has the following
    form:
    \begin{equation*}
        \begin{prooftree}
            \hypo{\Pi_i \bangAGKMeanTr \Gamma_i \vdash u : \tau_i}
            \delims{\left(}{\right)_{i \in I}}
            \inferBangAGKMeanInh{+_{i \in I} \Gamma_i}
            \inferBangAGKMeanBg{+_{i \in I} \Gamma_i &\vdash \oc t : \mset{\tau_i}_{i \in I}}
        \end{prooftree}
    \end{equation*}
    where $\Gamma = +_{i \in I} \Gamma_i$ and $\sigma =
    \mset{\tau_i}_{i \in I}$. Then trivially
    $\bangBKRVInhPred{\bangArgs{\sigma}} = \bangBKRVInhPred{\emul} $. This
    concludes this case since $\bangBKRVInhPred{\Gamma}$ holds by
    hypothesis.
\end{itemize}
\end{proof}


==> 3_Proofs/Bang_MA_L_t___=_MA_L__MA_t__.tex <==
\begin{proof} \deliaLu%
By induction on $\bangLCtxt$:
\begin{itemize}
\item[\bltI] $\bangLCtxt = \Hole$: Then
    $\bangMeaningfulApprox{\bangLCtxt<t>} = \bangMeaningfulApprox{t} =
    \Hole\bangCtxtPlug{\bangMeaningfulApprox{t}} =
    \bangMeaningfulApprox{\Hole}\bangCtxtPlug{\bangMeaningfulApprox{t}}$.

\item[\bltI] $\bangLCtxt = \bangLCtxt'\esub{x}{u}$: Then
    $\bangLCtxt<t> = \bangLCtxt'<t>\esub{x}{u}$ is meaningful so that
    using
    \Cref{lem:bang_solvability_on_app_and_es}.(\ref{lem:bang_meaningful_on_esub}),
    one has that $\bangLCtxt'<t>$ is meaningful. By \ih on
    $\bangLCtxt'$, one obtains that
    $\bangMeaningfulApprox{\bangLCtxt'<t>} =
    \bangMeaningfulApprox{\bangLCtxt'}\bangCtxtPlug{\bangMeaningfulApprox{t}}$
    thus:
    \begin{equation*}
        \begin{array}{r cl cl}
            \bangMeaningfulApprox{\bangLCtxt<t>}
                &=& \bangMeaningfulApprox{\bangLCtxt'<t>\esub{x}{u}}
        \\
                &=& \bangMeaningfulApprox{\bangLCtxt'<t>}\esub{x}{\bangMeaningfulApprox{u}}
        \\
                &\eqih& \bangMeaningfulApprox{\bangLCtxt'}\bangCtxtPlug{\bangMeaningfulApprox{t}}\esub{x}{\bangMeaningfulApprox{u}}
        \\
                &=& \bangMeaningfulApprox{\bangLCtxt'}\esub{x}{\bangMeaningfulApprox{u}}\bangCtxtPlug{\bangMeaningfulApprox{t}}
        \\
                &=& \bangMeaningfulApprox{\bangLCtxt'\esub{x}{u}}\bangCtxtPlug{\bangMeaningfulApprox{t}}
                &=& \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\bangMeaningfulApprox{t}}
        \end{array}
    \end{equation*}
\end{itemize}
\end{proof}

==> 3_Proofs/Bang_MA_t___=_t.tex <==
\begin{proof} \label{prf:Bang_MA(t)_<=_t}%
We distinguish two cases:
\begin{itemize}
\item[\bltI] $t$ meaningless: Then $\bangMeaningfulApprox{t} =
    \bangAprxBot \bangAprxLeq t$.

\item[\bltI] $t$ meaningful: By cases on $t$:
    \begin{itemize}
    \item[\bltII] $t = x$: Then $\bangMeaningfulApprox{t} = x
        \bangAprxLeq x = t$.

    \item[\bltII] $t = \abs{x}{t'}$: By \ih on $t'$, one has that
        $\bangMeaningfulApprox{t'} \bangAprxLeq t'$ thus
        $\bangMeaningfulApprox{t} = \abs{x}{\bangMeaningfulApprox{t'}}
        \bangAprxLeq \abs{x}{t'} = t$.

    \item[\bltII] $t = \app{t_1}{t_2}$: By \ih on $t_1$ and $t_2$, one
        has that $\bangMeaningfulApprox{t_1} \bangAprxLeq t_1$ and
        $\bangMeaningfulApprox{t_2} \bangAprxLeq t_2$ so that
        $\bangMeaningfulApprox{t} =
        \app{\bangMeaningfulApprox{t_1}}{\bangMeaningfulApprox{t_2}}
        \bangAprxLeq \app{t_1}{t_2} = t$.

    \item[\bltII] $t = t_1\esub{x}{t_2}$: By \ih on $t_1$ and $t_2$,
        one has that $\bangMeaningfulApprox{t_1} \bangAprxLeq t_1$ and
        $\bangMeaningfulApprox{t_2} \bangAprxLeq t_2$ so that
        $\bangMeaningfulApprox{t} =
        \bangMeaningfulApprox{t_1}\esub{x}{\bangMeaningfulApprox{t_2}}
        \bangAprxLeq t_1\esub{x}{t_2} = t$.

    \item[\bltI] $t = \oc t'$: By \ih on $t'$, one has that
        $\bangMeaningfulApprox{t'} \bangAprxLeq t'$ thus
        $\bangMeaningfulApprox{t} = \oc\bangMeaningfulApprox{t'}
        \bangAprxLeq \oc t' = t$.

    \item[\bltI] $t = \der{t'}$: By \ih on $t'$, one has that
        $\bangMeaningfulApprox{t'} \bangAprxLeq t'$ thus
        $\bangMeaningfulApprox{t} = \der{\bangMeaningfulApprox{t'}}
        \bangAprxLeq \der{t'} = t$.
        \qedhere
    \end{itemize}
\end{itemize} 
\end{proof}

==> 3_Proofs/Bang_MA_t_x-=u___=_MA_t__x-=MA_u__.tex <==
\begin{proof} \deliaLu%
We distinguish two cases:
\begin{itemize}
\item[\bltI] $t\isub{x}{u}$ meaningless: Then
    $\bangMeaningfulApprox{t\isub{x}{u}} = \bangAprxBot \bangAprxLeq
    \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}$.

\item[\bltI] $t\isub{x}{u}$ meaningful:
    Using~\Cref{lem:Bang_meaningful_subterms}.(\ref{lem:Bang_meaningful_on_isub}),
    one deduces that $t$ is meaningful. By induction on $t$:
    \begin{itemize}
    \item[\bltII] $t = y$: Then $\bangMeaningfulApprox{t} = y$ and we
        distinguish two cases:
        \begin{itemize}
        \item[\bltIII] $y = x$: Then
            $\bangMeaningfulApprox{t\isub{x}{u}} =
            \bangMeaningfulApprox{u} =
            x\isub{x}{\bangMeaningfulApprox{u}} =
            \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}$.

        \item[\bltIII] $y \neq x$: Then
            $\bangMeaningfulApprox{t\isub{x}{u}} =
            \bangMeaningfulApprox{y} = y =
            y\isub{x}{\bangMeaningfulApprox{u}} =
            \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}$.
        \end{itemize}

    \item[\bltII] $t = \abs{y}{t'}$: Then $\bangMeaningfulApprox{t} =
        \abs{y}{\bangMeaningfulApprox{t'}}$ and \ih on $t'$, one has
        that $\bangMeaningfulApprox{t'\isub{x}{u}} \bangAprxLeq
        \bangMeaningfulApprox{t'}\isub{x}{\bangMeaningfulApprox{u}}$.
        Thus:
        \begin{equation*}
            \begin{array}{r cl cl}
                \bangMeaningfulApprox{t\isub{x}{u}}
                &=& \bangMeaningfulApprox{\abs{y}{(t'\isub{x}{u})}}
            \\
                &=& \abs{y}{\bangMeaningfulApprox{t'\isub{x}{u}}}
            \\
                &\bangAprxLeqIh& \abs{y}{\bangMeaningfulApprox{t'}\isub{x}{\bangMeaningfulApprox{u}}}
            \\
                &=& (\abs{y}{\bangMeaningfulApprox{t'}})\isub{x}{\bangMeaningfulApprox{u}}
            \\
                &=& \bangMeaningfulApprox{\abs{y}{t'}}\isub{x}{\bangMeaningfulApprox{u}}
                &=& \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}
            \end{array}
        \end{equation*}

    \item[\bltII] $t = \app{t_1}{t_2}$: Then $\bangMeaningfulApprox{t}
        =
        \app{\bangMeaningfulApprox{t_1}}{\bangMeaningfulApprox{t_2}}$
        and by \ih on $t_1$ and $t_2$, one has that
        $\bangMeaningfulApprox{t_1\isub{x}{u}} \bangAprxLeq
        \bangMeaningfulApprox{t_1}\isub{x}{\bangMeaningfulApprox{u}}$
        and $\bangMeaningfulApprox{t_2\isub{x}{u}} \bangAprxLeq
        \bangMeaningfulApprox{t_2}\isub{x}{\bangMeaningfulApprox{u}}$.
        Thus:
        \begin{equation*}
            \begin{array}{r cl cl}
                \bangMeaningfulApprox{t\isub{x}{u}}
                &=& \bangMeaningfulApprox{\app{t_1\isub{x}{u}}{t_2\isub{x}{u}}}
            \\
                &=& \app{\bangMeaningfulApprox{t_1\isub{x}{u}}}{\bangMeaningfulApprox{t_2\isub{x}{u}}}
            \\
                &\bangAprxLeqIh& \app{(\bangMeaningfulApprox{t_1}\isub{x}{\bangMeaningfulApprox{u}})}{(\bangMeaningfulApprox{t_2}\isub{x}{\bangMeaningfulApprox{u}})}
            \\
                &=& (\app{\bangMeaningfulApprox{t_1}}{\bangMeaningfulApprox{t_2}})\isub{x}{\bangMeaningfulApprox{u}}
            \\
                &=& \bangMeaningfulApprox{\app{t_1}{t_2}}\isub{x}{\bangMeaningfulApprox{u}}
                &=& \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}
            \end{array}
        \end{equation*}

    \item[\bltII] $t = t_1\esub{y}{t_2}$: Thus
        $\bangMeaningfulApprox{t} =
        \bangMeaningfulApprox{t_1}\esub{y}{\bangMeaningfulApprox{t_2}}$
        and by \ih on $t_1$ and $t_2$, one has that
        $\bangMeaningfulApprox{t_1\isub{x}{u}} \bangAprxLeq
        \bangMeaningfulApprox{t_1}\isub{x}{\bangMeaningfulApprox{u}}$
        and $\bangMeaningfulApprox{t_2\isub{x}{u}} \bangAprxLeq
        \bangMeaningfulApprox{t_2}\isub{x}{\bangMeaningfulApprox{u}}$.
        Thus:
        \begin{equation*}
            \begin{array}{r cl cl}
                \bangMeaningfulApprox{t\isub{x}{u}}
                &=& \bangMeaningfulApprox{t_1\isub{x}{u}\esub{y}{t_2\isub{x}{u}}}
            \\
                &=& \bangMeaningfulApprox{t_1\isub{x}{u}}\esub{y}{\bangMeaningfulApprox{t_2\isub{x}{u}}}
            \\
                &\bangAprxLeqIh& (\bangMeaningfulApprox{t_1}\isub{x}{\bangMeaningfulApprox{u}})\esub{y}{\bangMeaningfulApprox{t_2}\isub{x}{\bangMeaningfulApprox{u}}}
            \\
                &=& (\bangMeaningfulApprox{t_1}\esub{y}{\bangMeaningfulApprox{t_2}})\isub{x}{\bangMeaningfulApprox{u}}
            \\
                &=& \bangMeaningfulApprox{t_1\esub{y}{t_2}}\isub{x}{\bangMeaningfulApprox{u}}
                &=& \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}
            \end{array}
        \end{equation*}

    \item[\bltII] $t = \der{t'}$: Then $\bangMeaningfulApprox{t} =
        \der{\bangMeaningfulApprox{t'}}$ and by \ih on $t'$, one has
        that $\bangMeaningfulApprox{t'\isub{x}{u}} =
        \bangMeaningfulApprox{t'}\isub{x}{\bangMeaningfulApprox{u}}$.
        Thus:
        \begin{equation*}
            \begin{array}{r cl cl}
                \bangMeaningfulApprox{t\isub{x}{u}}
                    &=& \bangMeaningfulApprox{\der{t'\isub{x}{u}}}
                \\
                    &=& \der{\bangMeaningfulApprox{t'\isub{x}{u}}}
                \\
                    &\eqih& \der{\bangMeaningfulApprox{t'}\isub{x}{\bangMeaningfulApprox{u}}}
                \\
                    &=& \der{\bangMeaningfulApprox{t'}}\isub{x}{\bangMeaningfulApprox{u}}
                    &=& \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}
            \end{array}
        \end{equation*}
    
    \item[\bltII] $t = \oc t'$: Then $\bangMeaningfulApprox{t} = \oc
        \bangMeaningfulApprox{t'}$ and by \ih on $t'$, one has that
        $\bangMeaningfulApprox{t'\isub{x}{u}} =
        \bangMeaningfulApprox{t'}\isub{x}{\bangMeaningfulApprox{u}}$.
        Thus:
        \begin{equation*}
            \begin{array}{r cl cl}
                \bangMeaningfulApprox{t\isub{x}{u}}
                    &=& \bangMeaningfulApprox{\oc(t'\isub{x}{u})}
                \\
                    &=& \oc \bangMeaningfulApprox{t'\isub{x}{u}}
                \\
                    &\eqih& \oc(\bangMeaningfulApprox{t'}\isub{x}{\bangMeaningfulApprox{u}})
                \\
                    &=& (\oc\bangMeaningfulApprox{t'})\isub{x}{\bangMeaningfulApprox{u}}
                    &=& \bangMeaningfulApprox{t}\isub{x}{\bangMeaningfulApprox{u}}
            \end{array}
        \end{equation*}
        \qedhere
    \end{itemize}
\end{itemize}
\end{proof}

==> 3_Proofs/Bang_SnNF_t__=__MA_t__in_bnoSn.tex <==
\begin{proof}
We strengthen the induction hypothesis:

Let $t \in \setBangTerms$ be meaningful and $n \in \setOrdinals$.
Then:
\begin{enumerate}
\item If $t \in \bangNeS_n$ then $\bangMeaningfulApprox{t} \in
    \bangAprxBneS_n$;
\item If $t \in \bangNaS_n$ then $\bangMeaningfulApprox{t} \in
    \bangAprxBnaS_n$;
\item If $t \in \bangNbS_n$ then $\bangMeaningfulApprox{t} \in
    \bangAprxBnbS_n$;
\item If $t \in \bangNoS_n$ then $\bangMeaningfulApprox{t} \in
    \bangAprxBnoS_n$.
\end{enumerate}

Let $t \in \setBangTerms$ be meaningful. By mutual induction on $t \in
\bangNeS_n$, $t \in \bangNaS_n$, $t \in \bangNbS_n$ and $t \in
\bangNoS_n$ with $n \in \setOrdinals$. Cases:
\begin{enumerate}
\item If $t \in \bangNeS_n$: Cases:
    \begin{itemize}
    \item $t = x$: Then $\bangMeaningfulApprox{t} = x \in
        \bangAprxBneS_n$

    \item $t = \app{t_1}{t_2}$ with $t_1 \in \bangAprxBneS_n$ and $t_2
        \in \bangAprxBnaS_n$: Using
        \Cref{lem:Bang_meaningful_subterms}.\ref{lem:Bang_meaningful_on_app},
        one has that $t_1$ and $t_2$ are meaningful thus by \ih on
        $t_1$ and $t_2$, one deduces that $\bangMeaningfulApprox{t_1}
        \in \bangAprxBneS_n$ and $\bangMeaningfulApprox{t_2} \in
        \bangAprxBnaS_n$. We conclude that \victorTodo

    \item $t = \der{t'}$ with $t' \in \bangAprxBneS_n$: Using
        \Cref{lem:Bang_meaningful_subterms}.\ref{lem:Bang_meaningful_on_der},
        one has that $t'$ is meaningful thus by \ih on $t'$, one
        deduces that $\bangMeaningfulApprox{t'} \in \bangAprxBneS_n$

    \item $t = t_1\esub{x}{t_2}$ with $t_1, t_2 \in \bangAprxBneS_n$:

    \end{itemize}

\item If $t \in \bangNaS_n$: Cases:
    \begin{itemize}
    \item 
    \end{itemize}

\item If $t \in \bangNbS_n$: Cases:
    \begin{itemize}
    \item 
    \end{itemize}

\item If $t \in \bangNoS_n$: Cases:
    \begin{itemize}
    \item 
    \end{itemize}

\end{enumerate}
% Since $\cbnPredSNF_n{t}$, then in particular $\cbnPredSNF{t}$, so that
% $t$ is meaninful. We reason by induction on $t \in \setBangTerms$:
% \begin{itemize}
% \item[\bltI] $t = x$: Then $\neg\cbnAbsPred{t}$ and $\bangMeaningfulApprox{t} =
%     x \in \cbnAprxAneS_n$.

% \item[\bltI] $t = \abs{x}{t'}$: Then $\cbnPredSNF_n{t'}$ and
%     $\cbnAbsPred{t}$ thus by \ih on $t'$, one has $\bangMeaningfulApprox{t'} \in
%     \cbnAprxAnoS_n$.

% \item[\bltI] $t = \app{t_1}{t_2}$: Then $\neg\cbnAbsPred{t}$,
%     $\cbnPredSNF_n{t_1}$ and $\neg\cbnAbsPred{t_1}$. By \ih on $t_1$,
%     one has that $\bangMeaningfulApprox{t_1} \in \cbnAprxAneS_n$. We distinguish
%     two cases:
%     \begin{itemize}
%     \item $n = 0$: Then $\bangMeaningfulApprox{t} =
%         \app{\bangMeaningfulApprox{t_1}}{\bangMeaningfulApprox{t_2}} \in
%         \app{\cbnAprxAneS_0}{\aprxT} \subseteq \cbnAprxAnoS_0$.

%     \item $n > 0$ (\resp $n = \omega$): Then $\cbnPredSNF_m{t_2}$ with
%         $m = n - 1$ (\resp $m = \omega$). By \ih on $t_2$, one has
%         that $\bangMeaningfulApprox{t_2} \in \cbnAprxAnoS_m$ thus
%         $\bangMeaningfulApprox{t} = \app{\bangMeaningfulApprox{t_1}}{\bangMeaningfulApprox{t_2}} \in
%         \app{\cbnAprxAneS_n}{\cbnAprxAnoS_m} \subseteq
%         \cbnAprxAneS_n$.
%     \end{itemize}

% \item[\bltI] $t = t_1\esub{x}{t_2}$: Impossible since
%     $\cbnPredSNF_n{t}$.
% \end{itemize}
\end{proof}

==> 3_Proofs/Bang_t1__=_t2_and_u1__=_u2_==__t1_x-=u1___=_t2_x-=u2_.tex <==
\begin{proof}
By induction on $\aprxT_1$:
\begin{itemize}
\item[\bltI] $\aprxT_1 = \bangAprxBot$: Then
	$\aprxT_1\isub{x}{\aprxU_1} = \bangAprxBot \bangAprxLeq
	\aprxT_2\isub{x}{\aprxU_2}$.

\item[\bltI] $\aprxT_1 = y$: Then $\aprxT_2 = y$ and we distinguish
    two cases:
    \begin{itemize}
    \item[\bltII] $x = y$: Thus $\aprxT_1\isub{x}{\aprxU_1} = \aprxU_1
        \bangAprxLeq \aprxU_2 = \aprxT_2\isub{x}{\aprxU_2}$.

    \item[\bltII] $x \neq y$: Thus $\aprxT_1\isub{x}{\aprxU_1} = y =
        \aprxT_2\isub{x}{\aprxU_2}$, thus $\aprxT_1\isub{x}{\aprxU_1}
        \bangAprxLeq \aprxT_2\isub{x}{\aprxU_2}$ by reflexivity of
        $\bangAprxLeq$.
    \end{itemize}

\item[\bltI] $\aprxT_1 = \abs{y}{\aprxT'_1}$: Then
	$\aprxT_1\isub{x}{\aprxU_1} =
	\abs{y}{\aprxT'_1\isub{x}{\aprxU_1}}$ (by supposing $y \notin
	\freeVar{\aprxU_1} \cup \freeVar{\aprxU_2}$ without loss of
	generality) and necessarily $\aprxT_2 = \abs{y}{\aprxT'_2}$ with
	$\aprxT'_1 \bangAprxLeq \aprxT'_2$ thus
	$\aprxT_2\isub{x}{\aprxU_2} =
	\abs{y}{\aprxT'_2\isub{y}{\aprxU_2}}$. By \ih on $\aprxT'_1$, one
	has that $\aprxT'_1\isub{x}{\aprxU_1} \bangAprxLeq
	\aprxT'_2\isub{x}{\aprxU_2}$ hence $\aprxT_1\isub{x}{\aprxU_1} =
	\abs{y}{\aprxT'_1\isub{x}{\aprxU_1}} \bangAprxLeq
	\abs{y}{\aprxT'_2\isub{x}{\aprxU_2}} = \aprxT_2\isub{x}{\aprxU_2}$
	by contextual closure.

\item[\bltI] $\aprxT_1 = \app{\aprxT_1^1}{\aprxT_1^2}$: Then
	$\aprxT_1\isub{x}{\aprxU_1} =
	\app{(\aprxT_1^1\isub{x}{\aprxU_1})}{(\aprxT_1^2\isub{x}{\aprxU_1})}$
	and necessarily $\aprxT_2 = \app[\,]{\aprxT_2^1}{\aprxT_2^2}$ with
	$\aprxT_1^1 \bangAprxLeq \aprxT_2^1$ and $\aprxT_1^2 \bangAprxLeq
	\aprxT_2^2$, thus $\aprxT_2\isub{y}{\aprxU_2} =
	\app{(\aprxT_2^1\isub{x}{\aprxU_2})}{(\aprxT_2^2\isub{x}{\aprxU_2})}$.
	By \ih on $\aprxT_1^1$ and $\aprxT_1^2$, one obtains that
	$\aprxT_1^1\isub{x}{\aprxU_1} \bangAprxLeq
	\aprxT_2^1\isub{x}{\aprxU_2}$ and $\aprxT_1^2\isub{x}{\aprxU_1}
	\bangAprxLeq \aprxT_2^2\isub{x}{\aprxU_2}$, hence
	$\aprxT_1\isub{x}{\aprxU_1} =
	\app{(\aprxT_1^1\isub{x}{\aprxU_1})}{(\aprxT_1^2\isub{x}{\aprxU_1})}
	\bangAprxLeq
	\app{(\aprxT_2^1\isub{x}{\aprxU_2})}{(\aprxT_2^2\isub{x}{\aprxU_2})}
	= \aprxT_2\isub{x}{\aprxU_2}$ by contextual closure.

\item[\bltI] $\aprxT_1 = \aprxT_1^1\esub{y}{\aprxT_1^2}$: Then
	$\aprxT_1\isub{x}{\aprxU_1} =
	\aprxT_1^1\isub{x}{\aprxU_1}\esub{y}{\aprxT_1^2\isub{x}{\aprxU_1}}$
	and necessarily $\aprxT_2 = \aprxT_2^1\esub{y}{\aprxT_2^2}$ with
	$\aprxT_1^1 \bangAprxLeq \aprxT_2^1$ and $\aprxT_1^2 \bangAprxLeq
	\aprxT_2^2$, thus $\aprxT_2\isub{y}{\aprxU_2} =
	\aprxT_2^1\isub{x}{\aprxU_2}\esub{y}{\aprxT_2^2\isub{x}{\aprxU_2}}$.
	By \ih on $\aprxT_1^1$ and $\aprxT_1^2$, one has
	$\aprxT_1^1\isub{x}{\aprxU_1} \bangAprxLeq
	\aprxT_2^1\isub{x}{\aprxU_2}$ and $\aprxT_1^2\isub{x}{\aprxU_1}
	\bangAprxLeq \aprxT_2^2\isub{x}{\aprxU_2}$, so by contextual
	closure $\aprxT_1\isub{x}{\aprxU_1} =
	\aprxT_1^1\isub{x}{\aprxU_1}\esub{y}{\aprxT_1^2\isub{x}{\aprxU_1}}
	\bangAprxLeq
	\aprxT_2^1\isub{x}{\aprxU_2}\esub{y}{\aprxT_2^2\isub{x}{\aprxU_2}}
	= \aprxT_2\isub{x}{\aprxU_2}$.

\item[\bltI] $\aprxT_1 = \der{\aprxT'_1}$: Then
    $\aprxT_1\isub{x}{\aprxU_1} = \der{\aprxT_1\isub{x}{\aprxU_1}}$
    and $\aprxT_2 = \der{\aprxT'_2}$ with $\aprxT'_1 \bangAprxLeq
    \aprxT'_2$ thus $\aprxT_2\isub{x}{\aprxU_2} =
    \der{\aprxT'_2\isub{x}{\aprxU_2}}$. By \ih on $\aprxT'_1$, one has
    that $\aprxT'_1\isub{x}{\aprxU_1} \bangAprxLeq
    \aprxT'_2\isub{x}{\aprxU_2}$, so by contextual closure
    $\aprxT_1\isub{x}{\aprxU_1} = \der{\aprxT'_1\isub{x}{\aprxU_1}}
    \bangAprxLeq \der{\aprxT'_2\isub{x}{\aprxU_2}} =
    \aprxT_2\isub{x}{\aprxU_2}$

\item[\bltI] $\aprxT_1 = \oc \aprxT'_1$: Then
    $\aprxT_1\isub{x}{\aprxU_1} = \oc (\aprxT_1\isub{x}{\aprxU_1})$
    and $\aprxT_2 = \oc \aprxT'_2$ with $\aprxT'_1 \bangAprxLeq
    \aprxT'_2$ thus $\aprxT_2\isub{x}{\aprxU_2} = \oc
    (\aprxT'_2\isub{x}{\aprxU_2})$. By \ih on $\aprxT'_1$, one has
    that $\aprxT'_1\isub{x}{\aprxU_1} \bangAprxLeq
    \aprxT'_2\isub{x}{\aprxU_2}$, so by contextual closure
    $\aprxT_1\isub{x}{\aprxU_1} = \oc (\aprxT'_1\isub{x}{\aprxU_1})
    \bangAprxLeq \oc (\aprxT'_2\isub{x}{\aprxU_2}) =
    \aprxT_2\isub{x}{\aprxU_2}$
	\qedhere
\end{itemize}
\end{proof}

==> 3_Proofs/Bang_t_-_Sn_u_=__MA_t__-__Sn_s__=_MA_u_.tex <==
\begin{proof}
%  \deliaLu

Let $t, u \in \setBangTerms$ such that $t \bangArr_{S_n} u$. We
distinguish two cases:
\begin{itemize}
\item[\bltI] $t$ meaningless: Then $u$ is meaningful
    using~\Cref{lem:Bang_t_meaningful_and_t_->Sn_u_=>_u_meaningful}
    thus $\bangMeaningfulApprox{t} = \bangAprxBot$ and
    $\bangMeaningfulApprox{u} = \bangAprxBot$. We set $\aprxU :=
    \bangMeaningfulApprox{u}$ therefore by reflexivity of both
    relations, $\bangMeaningfulApprox{t} \bangAprxArr*_{S_n} \aprxU
    \bangAprxGeq \bangMeaningfulApprox{u}$.

\item[\bltI] $t$ meaningful: Then $u$ is meaningful
    using~\Cref{lem:Bang_t_meaningful_and_t_->Sn_u_=>_u_meaningful}.
    By definition, there exist a context $\bangSCtxt_n$ and terms $t',
    u' \in \setBangTerms$ such that $t = \bangSCtxt_n<t'>$, $u =
    \bangSCtxt_n<u'>$ and $t' \mapstoR u'$ for some $\rel \in
    \{\bangSymbBeta, \bangSymbSubs, \bangSymbBang\}$. We reason by
    induction on $\bangSCtxt_n$:
    \begin{itemize}
    \item[\bltII] $\bangSCtxt_n = \Hole$: Then $t = t'$ and $u = u'$.
        We distinguish three cases:
        \begin{itemize}
        \item[\bltIII] \victor{[Non-modifié]} $\rel = \bangSymbBeta$:
            Then $t' = \app{\bangLCtxt<\abs{x}{s_1}>}{s_2}$ and $u' =
            \bangLCtxt<s_1\esub{x}{s_2}>$ for some context
            $\bangLCtxt$ and some terms $s_1, s_2 \in \setBangTerms$.
            Since $t'$ is meaningful, then using
            \Cref{lem:Bang_meaningful_subterms}.(\ref{lem:Bang_meaningful_on_app}),
            one deduces in particular that $\bangLCtxt<\abs{x}{s_1}>$
            is meaningful. Since $u'$ is meaningful, then using
            \Cref{lem:Bang_meaningful_subterms}.(\ref{lem:Bang_meaningful_on_esub}),
            one deduces in particular that $s_1\esub{x}{s_2}$ is
            meaningful. Thus, using
            \Cref{lem:Bang_MA(L<t>)_=_MA(L)<MA(t)>}, one has that
            $\bangMeaningfulApprox{t'} =
            \app{\bangMeaningfulApprox{\bangLCtxt<\abs{x}{s_1}>}}{\bangMeaningfulApprox{s_2}}
            =
            \app{\bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\abs{x}{\bangMeaningfulApprox{s_1}}}}{\bangMeaningfulApprox{s_2}}$
            and $\bangMeaningfulApprox{u'} =
            \bangMeaningfulApprox{\bangLCtxt<s_1\esub{x}{s_2}>} =
            \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{
            \bangMeaningfulApprox{s_1\esub{x}{s_2}}} =
            \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\bangMeaningfulApprox{s_1}\esub{x}{\bangMeaningfulApprox{s_2}}}$.
            Thus $\bangMeaningfulApprox{t} = \bangMeaningfulApprox{t'}
            \mapstoR[\bangSymbBeta] \bangMeaningfulApprox{u'} =
            \bangMeaningfulApprox{u}$. We set $\aprxU :=
            \bangMeaningfulApprox{u}$, therefore by reflexivity
            $\bangMeaningfulApprox{t} \bangAprxArr_{S_n} \aprxU
            \bangAprxGeq \bangMeaningfulApprox{u}$.

        \item[\bltIII] $\rel = \bangSymbSubs$: Then $t' =
            s_1\esub{x}{\bangLCtxt<\oc s_2>}$ and $u' =
            \bangLCtxt<s_1\isub{x}{s_2}>$ for some context
            $\bangLCtxt$ and some terms $s_1, s_2 \in \setBangTerms$.
            Since $t'$ is meaningful, then using
            \Cref{lem:Bang_meaningful_subterms}.(\ref{lem:Bang_meaningful_on_esub}),
            one deduces that $\bangLCtxt<\oc s_2>$ is meaningful thus
            $\bangMeaningfulApprox{t'} =
            \bangMeaningfulApprox{s_1}\esub{x}{\bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\oc\bangMeaningfulApprox{s_2}}}$
            using \Cref{lem:Bang_MA(L<t>)_=_MA(L)<MA(t)>}. Since $u'$
            is meaningful, one has that $\bangMeaningfulApprox{u'} =
            \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\bangMeaningfulApprox{s_1\isub{x}{s_2}}}$
            using \Cref{lem:Bang_MA(L<t>)_=_MA(L)<MA(t)>}. Using
            \Cref{lem:Bang_MA(t{x:=u})_=_MA(t){x:=MA(u)}}, one has
            that $\bangMeaningfulApprox{s_1\isub{x}{s_2}} \bangAprxLeq
            \bangMeaningfulApprox{s_1}\isub{x}{\bangMeaningfulApprox{s_2}}$.
            Thus, $\bangMeaningfulApprox{t'} \mapstoR[\bangSymbSubs]
            \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\bangMeaningfulApprox{s_1}\isub{x}{\bangMeaningfulApprox{s_2}}}
            \bangAprxGeq \bangMeaningfulApprox{u'}$. We set $\aprxU :=
            \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\bangMeaningfulApprox{s_1}\isub{x}{\bangMeaningfulApprox{s_2}}}$,
            therefore $\bangMeaningfulApprox{t} \bangAprxArr_{S_n}
            \aprxU \bangAprxGeq \bangMeaningfulApprox{u}$.

        \item[\bltIII] $\rel = \bangSymbBang$: Then $t' =
            \der{\bangLCtxt<\oc s>}$ and $u' = \bangLCtxt<s>$ for some
            context $\bangLCtxt$ and some term $s \in \setBangTerms$.
            Since $t'$ is meaningful, then using
            \Cref{lem:Bang_meaningful_subterms}.\ref{lem:Bang_meaningful_on_der},
            one deduces that $\bangLCtxt<\oc s>$ is meaningful thus
            that $\bangMeaningfulApprox{\bangLCtxt<\oc s>} =
            \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\oc
            \bangMeaningfulApprox{s}}$ using
            \Cref{lem:Bang_MA(L<t>)_=_MA(L)<MA(t)>}. Since $u'$ is
            meaningful, then $\bangMeaningfulApprox{\bangLCtxt<s>} =
            \bangMeaningfulApprox{\bangLCtxt}\bangCtxtPlug{\bangMeaningfulApprox{s}}$
            using \Cref{lem:Bang_MA(L<t>)_=_MA(L)<MA(t)>} thus
            $\bangMeaningfulApprox{t} = \bangMeaningfulApprox{t'}
            \mapstoR[\bangSymbBang] \bangMeaningfulApprox{u'} =
            \bangMeaningfulApprox{u}$. We set $\aprxU =
            \bangMeaningfulApprox{u}$, therefore by reflexivity
            $\bangMeaningfulApprox{t} \bangAprxArr_{S_n} \aprxU
            \bangAprxGeq \bangMeaningfulApprox{u}$.
        \end{itemize}

    \item[\bltII] \victor{[Non-modifié]} $\bangSCtxt_n =
        \abs{x}{\bangSCtxt'_n}$: By \ih on $\bangSCtxt'_n$, one has
        $\aprxU'$ such that $\bangMeaningfulApprox{\bangSCtxt'_n<t'>}
        \bangAprxArr*_{S_n} \aprxU' \bangAprxGeq
        \bangMeaningfulApprox{\bangSCtxt'_n<u'>}$. We set $\aprxU :=
        \abs{x}{\aprxU'}$, therefore
        $\bangMeaningfulApprox{\bangSCtxt_n<t'>} =
        \abs{x}{\bangMeaningfulApprox{\bangSCtxt'_n<t'>}}
        \bangAprxArr*_{S_n} \aprxU \bangAprxGeq
        \abs{x}{\bangMeaningfulApprox{\bangSCtxt'_n<u'>}} =
        \bangMeaningfulApprox{\bangSCtxt_n<u'>}$.
        

    \item[\bltII] \victor{[Non-modifié]} $\bangSCtxt_n =
        \app[\,]{\bangSCtxt'_n}{s}$: By \ih on $\bangSCtxt'_n$, one
        has $\aprxU'$ such that
        $\bangMeaningfulApprox{\bangSCtxt'_n<t'>} \bangAprxArr*_{S_n}
        \aprxU' \bangAprxGeq
        \bangMeaningfulApprox{\bangSCtxt'_n<u'>}$. We set $\aprxU :=
        \app{\aprxU'}{\bangMeaningfulApprox{s}}$, therefore
        $\bangMeaningfulApprox{\bangSCtxt_n<t'>} =
        \app{\bangMeaningfulApprox{\bangSCtxt'_n<t'>}}{\bangMeaningfulApprox{s}}
        \bangAprxArr*_{S_n} \aprxU \bangAprxGeq
        \app{\bangMeaningfulApprox{\bangSCtxt'_n<u'>}}{\bangMeaningfulApprox{s}}
        = \bangMeaningfulApprox{\bangSCtxt_n<u'>}$.

    \item[\bltII] $\bangSCtxt_n = \app[\,]{s}{\bangSCtxt'_n}$: By \ih
        on $\bangSCtxt'_m$, one has $\aprxU'$ such that
        $\bangMeaningfulApprox{\bangSCtxt'_n<t'>} \bangAprxArr*_{S_n}
        \aprxU' \bangAprxGeq
        \bangMeaningfulApprox{\bangSCtxt'_n<u'>}$. We set $\aprxU :=
        \app{\bangMeaningfulApprox{s}}{\aprxU'}$, therefore
        $\bangMeaningfulApprox{\bangSCtxt_n<t'>} =
        \app{\bangMeaningfulApprox{s}}{\bangMeaningfulApprox{\bangSCtxt'_n<t'>}}
        \bangAprxArr*_{S_n} \aprxU \bangAprxGeq
        \app{\bangMeaningfulApprox{s}}{\bangMeaningfulApprox{\bangSCtxt'_n<u'>}}
        = \bangMeaningfulApprox{\bangSCtxt_n<u'>}$.

    \item[\bltII] \victor{[Non-modifié]} $\bangSCtxt_n =
        \bangSCtxt'_n\esub{x}{s}$: By \ih on $\bangSCtxt'_n$, one has
        $\aprxU'$ such that $\bangMeaningfulApprox{\bangSCtxt'_n<t'>}
        \bangAprxArr*_{S_n} \aprxU' \bangAprxGeq
        \bangMeaningfulApprox{\bangSCtxt'_n<u'>}$. We set $\aprxU :=
        \aprxU'\esub{x}{\bangMeaningfulApprox{s}}$, therefore
        $\bangMeaningfulApprox{\bangSCtxt_n<t'>} =
        \aprxU'\esub{x}{\bangMeaningfulApprox{s}} \bangAprxArr*_{S_n}
        \aprxU \bangAprxGeq
        \bangMeaningfulApprox{\bangSCtxt'_n<u'>}\esub{x}{\bangMeaningfulApprox{s}}
        = \bangMeaningfulApprox{\bangSCtxt_n<u'>}$.

    \item[\bltII] $\bangSCtxt_n = s\esub{x}{\bangSCtxt'_n}$: By \ih on
        $\bangSCtxt_m$, one has $\aprxU'$ such that
        $\bangMeaningfulApprox{\bangSCtxt'_n<t'>} \bangAprxArr*_{S_n}
        \aprxU' \bangAprxGeq
        \bangMeaningfulApprox{\bangSCtxt'_n<u'>}$. We set $\aprxU :=
        \bangMeaningfulApprox{s}\esub{x}{\aprxU'}$, therefore
        $\bangMeaningfulApprox{\bangSCtxt_n<t'>} =
        \bangMeaningfulApprox{s}\esub{x}{\bangMeaningfulApprox{\bangSCtxt'_n<t'>}}
        \bangAprxArr*_{S_n} \aprxU \bangAprxGeq
        \bangMeaningfulApprox{s}\esub{x}{\bangMeaningfulApprox{\bangSCtxt'_n<u'>}}
        = \bangMeaningfulApprox{\bangSCtxt_n<u'>}$.

    \item[\bltII] $\bangSCtxt_n = \der{\bangSCtxt'_n}$: By \ih on
        $\bangSCtxt'_n$, one has $\aprxU'$ such that
        $\bangMeaningfulApprox{\bangSCtxt'_n<t'>} \bangAprxArr*_{S_n}
        \aprxU' \bangAprxGeq
        \bangMeaningfulApprox{\bangSCtxt'_n<u'>}$. We set $\aprxU :=
        \der{\aprxU'}$, therefore
        $\bangMeaningfulApprox{\bangSCtxt_n<t'>} =
        \der{\bangMeaningfulApprox{\bangSCtxt'_n<t'>}}
        \bangAprxArr*_{S_n} \aprxU \bangAprxGeq
        \der{\bangMeaningfulApprox{\bangSCtxt'_n<u'>}} =
        \bangMeaningfulApprox{\bangSCtxt_n<u'>}$.
    
    \item[\bltII] $\bangSCtxt_n = \oc \bangSCtxt'_m$ with either $n =
        m = \omega$, or $n = m + 1$ and $m \geq 0$: By \ih on
        $\bangSCtxt'_m$, one has $\aprxU'$ such that
        $\bangMeaningfulApprox{\bangSCtxt'_m<t'>} \bangAprxArr*_{S_m}
        \bangMeaningfulApprox{\bangSCtxt'_m<u'>}$. We set $\aprxU =
        \oc\aprxU'$, therefore
        $\bangMeaningfulApprox{\bangSCtxt_n<t'>} =
        \bangMeaningfulApprox{\bangSCtxt'_m<t'>} \bangAprxArr*_{S_n}
        \bangMeaningfulApprox{\bangSCtxt'_m<u'>} =
        \bangMeaningfulApprox{\bangSCtxt_n<u'>}$.
        \qedhere
    \end{itemize}
\end{itemize}
\end{proof}




==> 3_Proofs/Bang_t_-__u_and_t__=_t__==__t__-__u__and_u__=_u_.tex <==
\begin{proof}
\label{prf:Bang_t_->_u_and_t_<=_t'_==>_t'_->_u'_and_u_<=_u'}%
Let $\aprxT, \aprxU, \aprxT' \in \setBangAprxTerms$ such that $\aprxT
\bangAprxLeq \aprxT'$ and $\aprxT \bangAprxArr_{S_n} \aprxU$. Then
$\aprxT = \bangAprxSCtxt_n<\aprxT_r>$ and $\aprxU =
\bangAprxSCtxt_n<\aprxU_r>$ with $\aprxT_r \mapstoR \aprxU_r$ for some
$\aprxT_r, \aprxU_r \in \setBangAprxTerms$ and $\rel \in
\{\bangSymbBeta, \bangSymbSubs, \bangSymbBang\}$. Let us proceed by
induction on $\bangAprxSCtxt_n$:
\begin{itemize}
\item[\bltI] $\bangAprxSCtxt_n = \Hole$: Then $\aprxT = \aprxT_r$ and
    $\aprxU = \aprxU_r$. We distinguish three cases:
    \begin{itemize}
    \item[\bltII] $\rel = \bangAprxSymbBeta$: Then $\aprxT =
        \app{\bangAprxLCtxt<\abs{x}{\aprxS_1}>}{\aprxS_2}$ and $\aprxU
        = \bangAprxLCtxt<\aprxS_1\esub{x}{\aprxS_2}>$ for some context
        $\bangAprxLCtxt$ and some partial terms $\aprxS_1, \aprxS_2
        \in \setBangAprxTerms$. Since $\aprxT \bangAprxLeq \aprxT'$,
        by induction on $\bangAprxLCtxt$, one has that $\aprxT =
        \app{\bangAprxLCtxt'<\abs{x}{\aprxS'_1}>}{\aprxS'_2}$ with
        $\bangAprxLCtxt \bangAprxLeq \bangAprxLCtxt'$, $\aprxS_1
        \bangAprxLeq \aprxS'_1$ and $\aprxS_2 \bangAprxLeq \aprxS'_2$
        for some context $\bangAprxLCtxt'$ and partial terms
        $\aprxS'_1, \aprxS'_2 \in \setBangAprxTerms$. Taking $\aprxU'
        = \bangAprxLCtxt'<\aprxS'_1\esub{x}{\aprxS'_2}>$ concludes
        this case since $\aprxT' =
        \app{\bangAprxLCtxt'<\abs{x}{\aprxS'_1}>}{\aprxS'_2}
        \bangAprxArr_{S_n}
        \bangAprxLCtxt'<\aprxS'_1\esub{x}{\aprxS'_2}> = \aprxU'$ and
        by transitivity $\aprxS_1\esub{x}{\aprxS_2} \bangAprxLeq
        \aprxS'_1\esub{x}{\aprxS'_2}$ thus
        $\bangAprxLCtxt<\aprxS_1\esub{x}{\aprxS_2}> \bangAprxLeq
        \bangAprxLCtxt'<\aprxS'_1\esub{x}{\aprxS'_2}> = \aprxU'$ using
        \Cref{lem:Bang_L1_<=_L2_and_t1_<=_t2_==>_L1<t1>_<=_L2<t2>}.

    \item[\bltII] $\rel = \bangAprxSymbSubs$: Then $\aprxT =
        \aprxS_1\esub{x}{\bangAprxLCtxt<\oc\aprxS_2>}$ and $\aprxU =
        \bangAprxLCtxt<\aprxS_1\isub{x}{\aprxS_2}>$ for some partial
        terms $\aprxS_1, \aprxS_2 \in \setBangAprxTerms$ and some
        partial context $\bangAprxLCtxt$. Since $\aprxT \bangAprxLeq
        \aprxT'$, one has that $\aprxT' =
        \aprxS'_1\esub{x}{\bangAprxLCtxt'<\oc\aprxS'_2>}$ with
        $\aprxS_1 \bangAprxLeq \aprxS'_1$ and $\aprxS_2 \bangAprxLeq
        \aprxS'_2$ and $\bangAprxLCtxt \bangAprxLeq \bangAprxLCtxt'$
        for some some partial terms $\aprxS'_1, \aprxS'_2 \in
        \setBangAprxTerms$ and some partial context $\bangAprxLCtxt'$.
        Taking $\aprxU' =
        \bangAprxLCtxt<\aprxS'_1\isub{x}{\aprxS'_2}>$ concludes this
        case since $\aprxT' =
        \aprxS'_1\esub{x}{\bangAprxLCtxt<\oc\aprxS'_2>}
        \bangAprxArr_{S_n}
        \bangAprxLCtxt<\aprxS'_1\isub{x}{\aprxS'_2}>$ and using
        \Cref{lem:Bang_t1_<=_t2_and_u1_<=_u2_==>_t1{x:=u1}_<=_t2{x:=u2},lem:Bang_L1_<=_L2_and_t1_<=_t2_==>_L1<t1>_<=_L2<t2>},
        one has that $\bangAprxLCtxt<\aprxS_1\isub{x}{\aprxS_2}>
        \bangAprxLeq \bangAprxLCtxt'<\aprxS'_1\isub{x}{\aprxS'_2}>$.

    \item[\bltII] $\rel = \bangAprxSymbBang$: Then $\aprxT =
        \der{\bangAprxLCtxt<\oc\aprxS>}$ and $\aprxU =
        \bangAprxLCtxt<\aprxS>$ for some partial term $\aprxS \in
        \setBangAprxTerms$ and some partial context $\bangAprxLCtxt$.
        Since $\aprxT \bangAprxLeq \aprxT'$, one has that $\aprxT' =
        \der{\bangAprxLCtxt'<\oc\aprxS'>}$ for some partial term
        $\aprxS' \in \setBangAprxTerms$ and some partial context
        $\bangAprxLCtxt'$ such that $\bangAprxLCtxt \bangAprxLeq
        \bangAprxLCtxt'$ and $\aprxS \bangAprxLeq \aprxS'$. Taking
        $\aprxU' = \bangAprxLCtxt'<\aprxS'>$ concludes this case since
        $\aprxT' = \der{\bangAprxLCtxt'<\oc\aprxS'>}
        \bangAprxArr_{S_n} \bangAprxLCtxt'<\aprxS'>$ and $\aprxU =
        \bangAprxLCtxt<\aprxS> \bangAprxLeq \bangAprxLCtxt'<\aprxS'>$
        using
        \Cref{lem:Bang_L1_<=_L2_and_t1_<=_t2_==>_L1<t1>_<=_L2<t2>}.
    \end{itemize}

\item[\bltI] $\bangAprxSCtxt_n = \abs{x}{\bangAprxSCtxt'_n}$: Then
    $\aprxT = \abs{x}{\bangAprxSCtxt'_n<\aprxT_r>}$ and $\aprxU =
    \abs{x}{\bangAprxSCtxt'_n<\aprxU_r>}$ thus $\aprxT' =
    \abs{x}{\aprxT'_1}$ for some partial term $\aprxT'_1$ such that
    $\bangAprxSCtxt'_n<\aprxT_r> \bangAprxLeq \aprxT'_1$. Since
    $\bangAprxSCtxt'_n<\aprxT_r> \bangAprxArr_{S_n}
    \bangAprxSCtxt'_n<\aprxU_r>$, by \ih on $\bangAprxSCtxt'_n$, one
    obtains $\aprxU'_1 \in \setBangAprxTerms$ such that $\aprxT'_1
    \bangAprxArr_{S_n} \aprxU'_1$ and $\bangAprxSCtxt'_n<\aprxU_r>
    \bangAprxLeq \aprxU'_1$. Taking $\aprxU' = \abs{x}{\aprxU'_1}$
    concludes this case since $\aprxT' = \abs{x}{\aprxT'_1}
    \bangAprxArr_{S_n} \abs{x}{\aprxU'_1} = \aprxU'$ and $\aprxU =
    \abs{x}{\bangAprxSCtxt'_n<\aprxU_r>} \bangAprxLeq
    \abs{x}{\aprxU'_1} = \aprxU'$.

\item[\bltI] $\bangAprxSCtxt_n = \app[\,]{\bangAprxSCtxt'_n}{\aprxS}$:
    Then $\aprxT = \app{\bangAprxSCtxt'_n<\aprxT_r>}{\aprxS}$ and
    $\aprxU = \app{\bangAprxSCtxt'_n<\aprxU_r>}{\aprxS}$ thus $\aprxT'
    = \app[\,]{\aprxT'_1}{\aprxS'}$ for some partial term $\aprxT'_1,
    \aprxS \in \setBangAprxTerms$ such that
    $\bangAprxSCtxt'_n<\aprxT_r> \bangAprxLeq \aprxT'_1$ and $\aprxS
    \bangAprxLeq \aprxS'$. Since $\bangAprxSCtxt'_n<\aprxT_r>
    \bangAprxArr_{S_n} \bangAprxSCtxt'_n<\aprxU_r>$, by \ih on
    $\bangAprxSCtxt'_n$, one obtains $\aprxU'_1 \in \setBangAprxTerms$
    such that $\aprxT'_1 \bangAprxArr_{S_n} \aprxU'_1$ and
    $\bangAprxSCtxt'_n<\aprxU_r> \bangAprxLeq \aprxU'_1$. Taking
    $\aprxU' = \app{\aprxU'_1}{\aprxS'}$ concludes this case since
    $\aprxT' = \app{\aprxT'_1}{\aprxS'} \bangAprxArr_{S_n}
    \app{\aprxU'_1}{\aprxS'} = \aprxU'$ and $\aprxU =
    \app{\bangAprxSCtxt'_n<\aprxU_r>}{\aprxS} \bangAprxLeq
    \app{\aprxU'_1}{\aprxS'} = \aprxU'$ by transitivity.

\item[\bltI] $\bangAprxSCtxt_n = \app[\,]{\aprxS}{\bangAprxSCtxt'_n}$:
    Then $\aprxT = \app[\,]{\aprxS}{\bangAprxSCtxt'_n<\aprxT_r>}$ and
    $\aprxU = \app[\,]{\aprxS}{\bangAprxSCtxt'_n<\aprxU_r>}$ thus
    $\aprxT' = \app[\,]{\aprxS'}{\aprxT'_1}$ for some partial term
    $\aprxS, \aprxT'_1 \in \setBangAprxTerms$ such that $\aprxS
    \bangAprxLeq \aprxS'$ and $\bangAprxSCtxt'_n<\aprxT_r>
    \bangAprxLeq \aprxT'_1$. Since $\bangAprxSCtxt'_n<\aprxT_r>
    \bangAprxArr_{S_n} \bangAprxSCtxt'_n<\aprxU_r>$, by \ih on
    $\bangAprxSCtxt'_n$, one obtains $\aprxU'_1 \in \setBangAprxTerms$
    such that $\aprxT'_1 \bangAprxArr_{S_n} \aprxU'_1$ and
    $\bangAprxSCtxt'_n<\aprxU_r> \bangAprxLeq \aprxU'_1$. Taking
    $\aprxU' = \app{\aprxS'}{\aprxU'_1}$ concludes this case since
    $\aprxT' = \app{\aprxS'}{\aprxT'_1} \bangAprxArr_{S_n}
    \app{\aprxS'}{\aprxU'_1} = \aprxU'$ and $\aprxU =
    \app[\,]{\aprxS}{\bangAprxSCtxt'_n<\aprxU_r>} \bangAprxLeq
    \app{\aprxS'}{\aprxU'_1} = \aprxU'$ by transitivity.

\item[\bltI] $\bangAprxSCtxt_n = \bangAprxSCtxt'_n\esub{x}{\aprxS}$:
    Then $\aprxT = \bangAprxSCtxt'_n<\aprxT_r>\esub{x}{\aprxS}$ and
    $\aprxU = \bangAprxSCtxt'_n<\aprxU_r>\esub{x}{\aprxS}$ thus
    $\aprxT' = \aprxT'_1\esub{x}{\aprxS'}$ for some partial term
    $\aprxT'_1, \aprxS \in \setBangAprxTerms$ such that
    $\bangAprxSCtxt'_n<\aprxT_r> \bangAprxLeq \aprxT'_1$ and $\aprxS
    \bangAprxLeq \aprxS'$. Since $\bangAprxSCtxt'_n<\aprxT_r>
    \bangAprxArr_{S_n} \bangAprxSCtxt'_n<\aprxU_r>$, by \ih on
    $\bangAprxSCtxt'_n$, one obtains $\aprxU'_1 \in \setBangAprxTerms$
    such that $\aprxT'_1 \bangAprxArr_{S_n} \aprxU'_1$ and
    $\bangAprxSCtxt'_n<\aprxU_r> \bangAprxLeq \aprxU'_1$. Taking
    $\aprxU' = \aprxU'_1\esub{x}{\aprxS'}$ concludes this case since
    $\aprxT' = \aprxT'_1\esub{x}{\aprxS'} \bangAprxArr_{S_n}
    \aprxU'_1\esub{x}{\aprxS'} = \aprxU'$ and $\aprxU =
    \bangAprxSCtxt'_n<\aprxU_r>\esub{x}{\aprxS} \bangAprxLeq
    \aprxU'_1\esub{x}{\aprxS'} = \aprxU'$ by transitivity.

\item[\bltI] $\bangAprxSCtxt_n = \aprxS\esub{x}{\bangAprxSCtxt'_n}$:
    Then $\aprxT = \aprxS\esub{x}{\bangAprxSCtxt'_n<\aprxT_r>}$ and
    $\aprxU = \aprxS\esub{x}{\bangAprxSCtxt'_n<\aprxU_r>}$ thus
    $\aprxT' = \aprxS'\esub{x}{\aprxT'_1}$ for some partial term
    $\aprxS, \aprxT'_1 \in \setBangAprxTerms$ such that $\aprxS
    \bangAprxLeq \aprxS'$ and $\bangAprxSCtxt'_n<\aprxT_r>
    \bangAprxLeq \aprxT'_1$. Since $\bangAprxSCtxt'_m<\aprxT_r>
    \bangAprxArr_{S_n} \bangAprxSCtxt'_n<\aprxU_r>$, by \ih on
    $\bangAprxSCtxt'_n$, one obtains $\aprxU'_1 \in \setBangAprxTerms$
    such that $\aprxT'_1 \bangAprxArr_{S_n} \aprxU'_1$ and
    $\bangAprxSCtxt'_n<\aprxU_r> \bangAprxLeq \aprxU'_1$. Taking
    $\aprxU' = \aprxS'\esub{x}{\aprxU'_1}$ concludes this case since
    $\aprxT' = \aprxS'\esub{x}{\aprxT'_1} \bangAprxArr_{S_n}
    \aprxS'\esub{x}{\aprxU'_1} = \aprxU'$ and $\aprxU =
    \aprxS\esub{x}{\bangAprxSCtxt'_n<\aprxU_r>} \bangAprxLeq
    \aprxS'\esub{x}{\aprxU'_1} = \aprxU'$ by transitivity.

\item[\bltI] $\bangAprxSCtxt = \oc\bangAprxSCtxt'_m$ with either $n >
    0$ and $m = n-1$ or $n = m = \omega$: Then $\aprxT = \oc
    \bangAprxSCtxt'_m<\aprxT_r>$ and $\aprxU = \oc
    \bangAprxSCtxt'_m<\aprxU_r>$ thus $\aprxT' = \oc\aprxT'_1$ for
    some partial term $\aprxT'_1 \in \setBangAprxTerms$ such that
    $\bangAprxSCtxt'_m<\aprxT_r> \bangAprxLeq \aprxT'_1$. Since
    $\bangAprxSCtxt'_m<\aprxT_r> \bangAprxArr_{S_m}
    \bangAprxSCtxt'_m<\aprxU_r>$, by \ih on $\bangAprxSCtxt'_m$, one
    obtains $\aprxU'_1 \in \setBangAprxTerms$ such that $\aprxT'_1
    \bangAprxArr_{S_m} \aprxU'_1$ and $\bangAprxSCtxt'_m<\aprxU_r>
    \bangAprxLeq \aprxU'_1$. Taking $\aprxU' = \oc\aprxU'_1$ concludes
    this case since $\aprxT' = \oc\aprxT'_1 \bangAprxArr_{S_n}
    \oc\aprxU'_1 = \aprxU'$ and $\aprxU =
    \oc\bangAprxSCtxt'_n<\aprxU_r> \bangAprxLeq \oc\aprxU'_1 =
    \aprxU'$ by transitivity.

\item[\bltI] $\bangAprxSCtxt_n = \der{\bangAprxSCtxt'_n}$: Then
    $\aprxT = \der{\bangAprxSCtxt'_n<\aprxT_r>}$ and $\aprxU =
    \der{\bangAprxSCtxt'_n<\aprxU_r>}$ thus $\aprxT' =
    \der{\aprxT'_1}$ for some partial term $\aprxT'_1$ such that
    $\bangAprxSCtxt'_n<\aprxT_r> \bangAprxLeq \aprxT'_1$. Since
    $\bangAprxSCtxt'_n<\aprxT_r> \bangAprxArr_{S_n}
    \bangAprxSCtxt'_n<\aprxU_r>$, by \ih on $\bangAprxSCtxt'_n$, one
    obtains $\aprxU'_1 \in \setBangAprxTerms$ such that $\aprxT'_1
    \bangAprxArr_{S_n} \aprxU'_1$ and $\bangAprxSCtxt'_n<\aprxU_r>
    \bangAprxLeq \aprxU'_1$. Taking $\aprxU' = \der{\aprxU'_1}$
    concludes this case since $\aprxT' = \der{\aprxT'_1}
    \bangAprxArr_{S_n} \der{\aprxU'_1} = \aprxU'$ and $\aprxU =
    \der{\bangAprxSCtxt'_n<\aprxU_r>} \bangAprxLeq \der{\aprxU'_1} =
    \aprxU'$.
    \qedhere
\end{itemize}
\end{proof}

==> 3_Proofs/Bang_t_meaningless_=__MA_F_t____=_MA_F_u__.tex <==
\begin{proof}
\label{prf:Bang_t_meaningless_=>_MA(F<t>)_<=_MA(F<u>)}%
We distinguish two cases:
\begin{itemize}
\item[\bltI] $\bangFCtxt<t>$ meaningless: Then
    $\bangMeaningfulApprox{\bangFCtxt<t>} = \bangAprxBot \bangAprxLeq
    \bangMeaningfulApprox{\bangFCtxt<u>}$.

\item[\bltI] $\bangFCtxt<t>$ meaningful: Then by
    \Cref{lem:Bang_Qualitative_Surface_Genericity}, one deduces that
    $\bangFCtxt<u>$ is also meaningful. By induction on $\bangFCtxt$.
    Cases:
    \begin{itemize}
    \item[\bltII] $\bangFCtxt = \Hole$: Then $\bangFCtxt<t> = t$ which
        contradicts the hypothesis $t$ is meaningless.

    \item[\bltII] $\bangFCtxt = \abs{x}{\bangFCtxt'}$: By \ih on
        $\bangFCtxt'$, one has that
        $\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}$ thus
        $\bangMeaningfulApprox{\bangFCtxt<t>} =
        \abs{x}{\bangMeaningfulApprox{\bangFCtxt'<t>}} \bangAprxLeq
        \abs{x}{\bangMeaningfulApprox{\bangFCtxt'<u>}} =
        \bangMeaningfulApprox{\bangFCtxt<u>}$.

    \item[\bltII] $\bangFCtxt = \app{\bangFCtxt'}{s}$: By \ih on
        $\bangFCtxt'$, one has that
        $\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}$ thus
        $\bangMeaningfulApprox{\bangFCtxt<t>} =
        \app{\bangMeaningfulApprox{\bangFCtxt'<t>}}{s} \bangAprxLeq
        \app{\bangMeaningfulApprox{\bangFCtxt'<u>}}{s} =
        \bangMeaningfulApprox{\bangFCtxt<u>}$.

    \item[\bltII] $\bangFCtxt = \app{s}{\bangFCtxt'}$: By \ih on
        $\bangFCtxt'$, one has that
        $\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}$ thus
        $\bangMeaningfulApprox{\bangFCtxt<t>} =
        \app[\,]{s}{\bangMeaningfulApprox{\bangFCtxt'<t>}}
        \bangAprxLeq
        \app[\,]{s}{\bangMeaningfulApprox{\bangFCtxt'<u>}} =
        \bangMeaningfulApprox{\bangFCtxt<u>}$.

    \item[\bltII] $\bangFCtxt = \bangFCtxt'\esub{x}{s}$: By \ih on
        $\bangFCtxt'$, one has that
        $\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}$ thus
        $\bangMeaningfulApprox{\bangFCtxt<t>} =
        \bangMeaningfulApprox{\bangFCtxt'<t>}\esub{x}{s} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}\esub{x}{s} =
        \bangMeaningfulApprox{\bangFCtxt<u>}$.

    \item[\bltII] $\bangFCtxt = s\esub{x}{\bangFCtxt'}$: By \ih on
        $\bangFCtxt'$, one has that
        $\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}$ thus
        $\bangMeaningfulApprox{\bangFCtxt<t>} =
        s\esub{x}{\bangMeaningfulApprox{\bangFCtxt'<t>}} \bangAprxLeq
        s\esub{x}{\bangMeaningfulApprox{\bangFCtxt'<u>}} =
        \bangMeaningfulApprox{\bangFCtxt<u>}$.

    \item[\bltII] $\bangFCtxt = \der{\bangFCtxt'}$: By \ih on
        $\bangFCtxt'$, one has that
        $\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}$ thus
        $\bangMeaningfulApprox{\bangFCtxt<t>} =
        \der{\bangMeaningfulApprox{\bangFCtxt'<t>}} \bangAprxLeq
        \der{\bangMeaningfulApprox{\bangFCtxt'<u>}} =
        \bangMeaningfulApprox{\bangFCtxt<u>}$.

    \item[\bltII] $\bangFCtxt = \oc \bangFCtxt'$:  By \ih on
        $\bangFCtxt'$, one has that
        $\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \bangMeaningfulApprox{\bangFCtxt'<u>}$ thus
        $\bangMeaningfulApprox{\bangFCtxt<t>} =
        \oc\bangMeaningfulApprox{\bangFCtxt'<t>} \bangAprxLeq
        \oc\bangMeaningfulApprox{\bangFCtxt'<u>} =
        \bangMeaningfulApprox{\bangFCtxt<u>}$.
    \end{itemize}
\end{itemize}
\end{proof}

==> fig_Type_System_Bm.tex <==
\begin{figure}[t]
%    \ovalbox{
        $\hspace{-1.25cm}\begin{array}{c}
            \begin{prooftree}
                \inferBangAGKMeanInh{\mset{\sigma}}
                \inferBangAGKMeanInh{\bangArgs{\sigma}}
                \inferBangAGKMeanVar{x : \mset{\sigma} \vdash x : \sigma}
            \end{prooftree}
        \qquad
            \begin{prooftree}
                \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1 \vdash t : \M \typeArrow \sigma}
                \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash u : \M}
                \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                \inferBangAGKMeanApp{\Gamma_1 + \Gamma_2 \vdash \app{t}{u} : \sigma}
            \end{prooftree}
    \\[12pt]
            \begin{prooftree}
                \hypo{\Pi \bangAGKMeanTr \Gamma, x : \M \vdash t : \sigma}
                \inferBangAGKMeanAbs{\Gamma \vdash \abs{x}{t} : \M \typeArrow \sigma}
            \end{prooftree}
        \qquad
            \begin{prooftree}
                \hypo{\Pi_1 \bangAGKMeanTr \Gamma_1, x : \M \vdash t : \sigma}
                \hypo{\Pi_2 \bangAGKMeanTr \Gamma_2 \vdash u : \M}
                \inferBangAGKMeanInh{\Gamma_1 + \Gamma_2}
                \inferBangAGKMeanEs{\Gamma_1 + \Gamma_2 \vdash t\esub{x}{u} : \sigma}
            \end{prooftree}
    \\[12pt]
            \begin{prooftree}
                \hypo{(\Pi_i \bangAGKMeanTr \Gamma_i \vdash t :
                \sigma_i)_{i \in I}} \inferBangAGKMeanInh{+_{i \in I}
                \Gamma_i} \inferBangAGKMeanBg{+_{i \in I} \Gamma_i
                &\vdash \oc t : \mset{\sigma_i}_{i \in I}}
            \end{prooftree}
        \qquad
            \begin{prooftree}
                \hypo{\Pi \bangAGKMeanTr \Gamma \vdash t : \mset{\sigma}}
                \inferBangAGKMeanInh{\bangArgs{\sigma}}
                \inferBangAGKMeanDer{\Gamma \vdash \der{t} : \sigma}
            \end{prooftree}
        \end{array}$
%    }
    \caption{Type System $\bangAGKMeanTypeSys$ for the \bangCalculusSymb-calculus.}
    \label{fig:BangAGKMean_Typing_System_Rules}%
\end{figure}










